Distribution functions for a family of general-relativistic Hypervirial models in collisionless regime

By considering the Einstein-Vlasov system for static spherically symmetric distributions of matter, we show that configurations with constant anisotropy parameter $\beta$ have, necessarily, a distribution function (DF) of the form $F=l^{-2\beta}\xi(\varepsilon)$, where $\varepsilon=E/m$ and $l=L/m$ are the relativistic energy and angular momentum per unit rest mass, respectively. We exploit this result to obtain DFs for the general relativistic extension of the Hypervirial family introduced by Nguyen and Lingam (2013), which Newtonian potential is given by $\phi(r)=-\phi_o /[1+(r/a)^{n}]^{1/n}$ ($a$ and $\phi_o$ are positive free parameters, $n=1,2,...$). Such DFs can be written in the form $F_{n}=l^{n-2}\xi_{n}(\varepsilon)$. For odd $n$, we find that $\xi_n$ is a polynomial of order $2n+1$ in $\varepsilon$, as in the case of the Hernquist model ($n=1$), for which $F_1\propto l^{-1}\left(2\varepsilon-1\right)\left(\varepsilon-1\right)^2$. For even $n$, we can write $\xi_n$ in terms of incomplete beta functions (Plummer model, $n=2$, is an example). Since we demand that $F\geq 0$ throughout the phase space, the particular form of each $\xi_n$ leads to restrictions for the values of $\phi_o$. For example, for the Hernquist model we find that $0\leq \phi_o \leq2/3$, i.e. an upper bounding value less than the one obtained for Nguyen and Lingam ($0\leq \phi_o \leq1$), based on energy conditions.

==> stabgr_refs <==
% Encoding: UTF-8




%% Organizado pelo nome do primeiro autor e ano

%% ============================================================
%% ====== Abramowicz MA et al. ======
%% ============================================================

% 1990MNRAS.245..733A,
@ARTICLE{abramowicz1990MNRAS,
   author = {{Abramowicz}, M. A.},
    title = "{Centrifugal Force - a Few Surprises}",
  journal = {\mnras},
     year = 1990,
    month = aug,
   volume = 245,
    pages = {733},
   adsurl = {http://adsabs.harvard.edu/abs/1990MNRAS.245..733A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% Abramowicz & Fragile 2013, LRR, Foundations of Black Hole Accretion Disk Theory
% %%2013LRR....16....1A,
@ARTICLE{abramowiczFragileLRR,
   author = {{Abramowicz}, M.A. and {Fragile}, P.C.},
    title = "{Foundations of Black Hole Accretion Disk Theory}",
  journal = {Living Reviews in Relativity},
archivePrefix = "arXiv",
   eprint = {1104.5499},
 primaryClass = "astro-ph.HE",
 keywords = {black hole accretion disks},
     year = 2013,
    month = jan,
   volume = 16,
    pages = {1},
      doi = {10.12942/lrr-2013-1},
   adsurl = {http://adsabs.harvard.edu/abs/2013LRR....16....1A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% Abramowicz & Kluzniak 2005, Ap\&SS, Epicyclic Frequencies Derived From The Effective Potential: Simple And Practical Formulae
%%2005Ap&SS.300..127A,
@ARTICLE{abramowiczKluzniak2005ApSS,
   author = {{Abramowicz}, M.A. and {Klu{\'z}niak}, W.},
    title = "{Epicyclic Frequencies Derived From The Effective Potential: Simple And Practical Formulae}",
  journal = {\apss},
   eprint = {astro-ph/0411709},
 keywords = {black holes, neutron stars, orbital motion, epicyclic frequencies},
     year = 2005,
    month = nov,
   volume = 300,
    pages = {127-136},
      doi = {10.1007/s10509-005-1173-z},
   adsurl = {http://adsabs.harvard.edu/abs/2005Ap\%26SS.300..127A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Allen C et al. ======
%% ============================================================

% 1991RMxAA..22..255A,
@ARTICLE{allenSantillan1991RMxAA,
   author = {{Allen}, C. and {Santillan}, A.},
    title = "{An improved model of the galactic mass distribution for orbit computations}",
  journal = {\rmxaa},
 keywords = {Astronomical Models, Galactic Mass, Mass Distribution, Milky Way Galaxy, Stellar Motions, Dynamic Models, Galactic Rotation, Galactic Structure, Mathematical Models},
     year = 1991,
    month = oct,
   volume = 22,
    pages = {255-263},
   adsurl = {http://adsabs.harvard.edu/abs/1991RMxAA..22..255A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Ansorg M et al. ======
%% ============================================================

%
%%1998JMP....39.5984A,
@ARTICLE{ansorg1998JMP,
   author = {{Ansorg}, M.},
    title = "{Timelike geodesic motions within the general relativistic gravitational field of the rigidly rotating disk of dust}",
  journal = {Journal of Mathematical Physics},
 keywords = {Exact solutions, Einstein-Maxwell spacetimes spacetimes with fluids radiation or classical fields},
     year = 1998,
    month = nov,
   volume = 39,
    pages = {5984-6000},
      doi = {10.1063/1.532609},
   adsurl = {http://adsabs.harvard.edu/abs/1998JMP....39.5984A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Arnold VI et al. ======
%% ============================================================

%
@book{arnoldMmcm,
  author = {V. I. Arnol'd}, edition = {Second},
  title  = {Mathematical Methods of Classical Mechanics},
  publisher = {Springer-Verlag},
  year = {1989}, series = {Graduate Texts in Mathematics},  volume = 60,
  address = {New York, NY}	
}



%\bibitem[\protect\citeauthoryear{Arnold}{1978}]{arnold}
%Arnold V. I., 1978, Mathematical Methods of Classical
%Mechanics. Springer-Verlag, New York, NY

%% ============================================================
%% ====== Bardeen JM et al. ======
%% ============================================================


%%1970ApJ...161..103B,
@ARTICLE{bardeen1970ApJ,
   author = {{Bardeen}, J. M.},
    title = "{Stability of Circular Orbits in Stationary, Axisymmetric Space-Times}",
  journal = {\apj},
     year = 1970,
    month = jul,
   volume = 161,
    pages = {103},
      doi = {10.1086/150515},
   adsurl = {http://adsabs.harvard.edu/abs/1970ApJ...161..103B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== BarrabÃ¨s C et al. ======
%% ============================================================

%1989CQGra...6..581B,
@ARTICLE{barrabes1989CQGra,
   author = {{Barrab{\`e}s}, C.},
    title = "{Singular hypersurfaces in general relativity - A unified description}",
  journal = {Classical and Quantum Gravity},
 keywords = {Cosmology, Hyperspaces, Relativity, Shock Waves, Einstein Equations, Stress Tensors},
     year = 1989,
    month = may,
   volume = 6,
    pages = {581-588},
      doi = {10.1088/0264-9381/6/5/003},
   adsurl = {http://adsabs.harvard.edu/abs/1989CQGra...6..581B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Batsleer P et al. ======
%% ============================================================

% 1994A&A...287...43B,
@ARTICLE{batsleerDejonghe1994AA,
   author = {{Batsleer}, P. and {Dejonghe}, H.},
    title = "{The generation of Stackel potentials for galactic dynamical modeling}",
  journal = {\aap},
 keywords = {Astronomical Models, Dynamic Models, Galactic Structure, Milky Way Galaxy, Potential, Rotation, Galactic Halos, Measure And Integration, Rotating Disks},
     year = 1994,
    month = jul,
   volume = 287,
    pages = {43-54},
   adsurl = {http://adsabs.harvard.edu/abs/1994A\%26A...287...43B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Bayin ======
%% ============================================================

@article{PhysRevD.26.1262,
  title = {Anisotropic fluid spheres in general relativity},
  author = {Bayin, S.S.},
  journal = {Phys. Rev. D},
  volume = {26},
  issue = {6},
  pages = {1262--1274},
  numpages = {0},
  year = {1982},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.26.1262},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.26.1262}
}



%% ============================================================
%% ====== Bekenstein J et al. ======
%% ============================================================

% 1984ApJ...286....7B,
@ARTICLE{bekensteinMilgrom1984ApJ,
   author = {{Bekenstein}, J. and {Milgrom}, M.},
    title = "{Does the missing mass problem signal the breakdown of Newtonian gravity?}",
  journal = {\apj},
 keywords = {Galactic Rotation, Gravitation Theory, Mass Distribution, Missing Mass (Astrophysics), Newton Theory, Nonrelativistic Mechanics, Potential Theory, Computational Astrophysics, Cosmology, Equivalence, Poisson Equation},
     year = 1984,
    month = nov,
   volume = 286,
    pages = {7-14},
      doi = {10.1086/162570},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...286....7B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Bershady MA et al. ======
%% ============================================================

% 2010ApJ...716..198B,
@ARTICLE{bershadyEtal2010ApJ1,
   author = {{Bershady}, M.A. and {Verheijen}, M. A. W. and {Swaters}, R. A. and
	{Andersen}, D. R. and {Westfall}, K. B. and {Martinsson}, T.
	},
    title = "{The DiskMass Survey. I. Overview}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1004.4816},
 primaryClass = "astro-ph.CO",
 keywords = {dark matter, galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: halos, galaxies: kinematics and dynamics, galaxies: spiral, galaxies: stellar content, galaxies: structure},
     year = 2010,
    month = jun,
   volume = 716,
    pages = {198-233},
      doi = {10.1088/0004-637X/716/1/198},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...716..198B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2010ApJ...716..234B,
@ARTICLE{bershadyEtal2010ApJ2,
   author = {{Bershady}, M. A. and {Verheijen}, M. A. W. and {Westfall}, K. B. and
	{Andersen}, D. R. and {Swaters}, R. A. and {Martinsson}, T.},
    title = "{The DiskMass Survey. II. Error Budget}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1004.5043},
 primaryClass = "astro-ph.CO",
 keywords = {dark matter, galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: halos, galaxies: kinematics and dynamics, galaxies: spiral, galaxies: stellar content, galaxies: structure, methods: data analysis, techniques: spectroscopic},
     year = 2010,
    month = jun,
   volume = 716,
    pages = {234-268},
      doi = {10.1088/0004-637X/716/1/234},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...716..234B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Bertin G et al. ======
%% ============================================================

%
@book{bertin2014dynamics,
  title={Dynamics of galaxies},
  author={Bertin, Giuseppe},
  year={2014},
  publisher={Cambridge University Press}
}

%% ============================================================
%% ====== Bertschinger E et al. ======
%% ============================================================

%
@misc{bertschinger,
  author={Bertschinger, E.},
  title={General relativity notes, chap. 3: Hamiltonian dynamics of particle motion},
  howpublished={Lecture notes (online resource)},
  note={http://web.mit.edu/edbert/GR/gr3.pdf},
  year={1999}
}

% \bibitem{bertschinger}
% Bertschinger, E., \textit{General relativity notes, cap.3: Hamiltonian dynamics of particle motion},
% http://web.mit.edu/edbert/GR/gr3.pdf


%% ============================================================
%% ====== Bi\v{c}\'ak J et al. (Bicak) ======
%% ============================================================

%1993PhRvD..47.4334B,
@ARTICLE{bicakLyndenbellKatz1993PRD,
   author = {{Bi{\v c}{\'a}k}, J. and {Lynden-Bell}, D. and {Katz}, J.},
    title = "{Relativistic disks as sources of static vacuum spacetimes}",
  journal = {\prd},
 keywords = {Exact solutions},
     year = 1993,
    month = may,
   volume = 47,
    pages = {4334-4343},
      doi = {10.1103/PhysRevD.47.4334},
   adsurl = {http://adsabs.harvard.edu/abs/1993PhRvD..47.4334B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}	

%% ============================================================
%% ====== Bienayme O et al. ======
%% ============================================================

% 2013A&A...549A..89B,
@ARTICLE{bienaymeTraven2013AA,
   author = {{Bienaym{\'e}}, O. and {Traven}, G.},
    title = "{Approximate integrals of motion}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1211.6306},
 primaryClass = "astro-ph.GA",
 keywords = {gravitation, methods: numerical, galaxies: kinematics and dynamics},
     year = 2013,
    month = jan,
   volume = 549,
      eid = {A89},
    pages = {A89},
      doi = {10.1051/0004-6361/201220008},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...549A..89B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2009A&A...500..801B,
@ARTICLE{bienaymeEtal2009AA,
   author = {{Bienaym{\'e}}, O. and {Famaey}, B. and {Wu}, X. and {Zhao}, H. S. and
	{Aubert}, D.},
    title = "{Galactic kinematics with modified Newtonian dynamics}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0904.3893},
 primaryClass = "astro-ph.GA",
 keywords = {gravitation, stars: kinematics, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2009,
    month = jun,
   volume = 500,
    pages = {801-805},
      doi = {10.1051/0004-6361/200809978},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...500..801B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Binney J et al.  ======
%% ============================================================



%series = {Graduate Texts in Mathematics},  volume = 60,
@book{binneytremaineGD,
  author = {{Binney}, J. and {Tremaine}, S.}, edition = {Second},
  title  = {Galactic Dynamics},
  publisher = {Princeton Univ. Press},
  year = {2008},
  address = {Princeton, NJ}	
}

% 2010MNRAS.401.2318B,
@ARTICLE{binney2010MNRAS,
   author = {{Binney}, J.},
    title = "{Distribution functions for the Milky Way}",
  journal = {\mnras},
archivePrefix = "arXiv",
 primaryClass = "astro-ph.GA",
 keywords = {solar neighbourhood, Galaxy: disc, galaxies: kinematics and dynamics},
     year = 2010,
    month = feb,
   volume = 401,
    pages = {2318-2330},
      doi = {10.1111/j.1365-2966.2009.15845.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.401.2318B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
  %   eprint = {0910.1512},
}

% 2011MNRAS.413.1889B,
@ARTICLE{binneyMcmillan2011MNRAS,
   author = {{Binney}, J. and {McMillan}, P.},
    title = "{Models of our Galaxy - II}",
  journal = {\mnras},
archivePrefix = "arXiv",
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disc, Galaxy: kinematics and dynamics, Galaxy: structure, galaxies: kinematics and dynamics},
     year = 2011,
    month = may,
   volume = 413,
    pages = {1889-1898},
      doi = {10.1111/j.1365-2966.2011.18268.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.413.1889B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
    % eprint = {1101.0747},
}


% 2012MNRAS.426.1328B,
@ARTICLE{binney2012MNRAS,
   author = {{Binney}, J.},
    title = "{More dynamical models of our Galaxy}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1207.4917},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disc, solar neighbourhood, galaxies: kinematics and dynamics},
     year = 2012,
    month = oct,
   volume = 426,
    pages = {1328-1337},
      doi = {10.1111/j.1365-2966.2012.21692.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.426.1328B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2012MNRAS.426.1324B,
@ARTICLE{binney2012MNRASactions,
   author = {{Binney}, J.},
    title = "{Actions for axisymmetric potentials}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1207.4910},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: kinematics and dynamics, galaxies: kinematics and dynamics},
     year = 2012,
    month = oct,		
   volume = 426,
    pages = {1324-1327},
      doi = {10.1111/j.1365-2966.2012.21757.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.426.1324B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2014IAUS..298..117B,
@INPROCEEDINGS{binneySanders2014IAUS,
   author = {{Binney}, J. and {Sanders}, J. L.},
    title = "{Dynamical models and Galaxy surveys}",
 keywords = {stellar dynamics, surveys, stars: abundances, Galaxy: disk, Galaxy: kinematics and dynamics, Galaxy: stellar content},
booktitle = {IAU Symposium},
     year = 2014,
   series = {IAU Symposium},
   volume = 298,
archivePrefix = "arXiv",
   eprint = {1309.2790},
 primaryClass = "astro-ph.GA",
   editor = {{Feltzing}, S. and {Zhao}, G. and {Walton}, N. A. and {Whitelock}, P.
	},
    month = jan,
    pages = {117-129},
      doi = {10.1017/S1743921313006297},
   adsurl = {http://adsabs.harvard.edu/abs/2014IAUS..298..117B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Bocaletti D et al.  ======
%% ============================================================

% 1999thor.book.....B,
@BOOK{theoryoforbits2,
   author = {{Boccaletti}, D. and {Pucacco}, G.},
    title = "{Theory of Orbits Volume 2: Perturbative and Geometrical Methods}",
booktitle = {Volume 2: Perturbative and Geometrical Methods, XV, 423 pp. 81 figs..  Springer-Verlag Berlin Heidelberg New York.  Also Astronomy and Astrophysics Library, volume 2},
     year = 1999,
   adsurl = {http://adsabs.harvard.edu/abs/1999thor.book.....B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
  publisher = {Springer-Verlag},
  address = {Berlin}
}


%% ============================================================
%% ====== Bonnor WB et al.  ======
%% ============================================================


%1968CMaPh...8..338B,
@ARTICLE{bonnor1968CMaPh,
   author = {{Bonnor}, W. B. and {Sackfield}, A.},
    title = "{The interpretation of some spheroidal metrics}",
  journal = {Communications in Mathematical Physics},
     year = 1968,
    month = dec,
   volume = 8,
    pages = {338-344},
      doi = {10.1007/BF01646273},
   adsurl = {http://adsabs.harvard.edu/abs/1968CMaPh...8..338B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Bosma A et al.  ======
%% ============================================================

% 2002ASPC..273..223B,
@INPROCEEDINGS{bosma2002ASPconf,
   author = {{Bosma}, A.},
    title = "{HI and Dark Matter in Spiral Galaxies}",
booktitle = {The Dynamics, Structure {\amp} History of Galaxies: A Workshop in Honour of Professor Ken Freeman},
     year = 2002,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 273,
   eprint = {astro-ph/0112080},
   editor = {{Da Costa}, G. S. and {Sadler}, E. M. and {Jerjen}, H.},
    pages = {223},
   adsurl = {http://adsabs.harvard.edu/abs/2002ASPC..273..223B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%Buchdahl


@ARTICLE{1964ApJ...140.1512B,
   author = {{Buchdahl}, H. A.},
    title = "{A Relativistic Fluid Sphere Resembling the Emden Polytrope of Index 5.}",
  journal = {\apj},
     year = 1964,
    month = nov,
   volume = 140,
    pages = {1512},
      doi = {10.1086/148055},
   adsurl = {http://adsabs.harvard.edu/abs/1964ApJ...140.1512B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Bowers  ======
%% ============================================================

@ARTICLE{1974ApJ...188..657B,
   author = {{Bowers}, R. L. and {Liang}, E. P. T.},
    title = "{Anisotropic Spheres in General Relativity}",
  journal = {\apj},
     year = 1974,
    month = mar,
   volume = 188,
    pages = {657},
      doi = {10.1086/152760},
   adsurl = {http://adsabs.harvard.edu/abs/1974ApJ...188..657B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Buchdahl  ======
%% ============================================================


@ARTICLE{1964ApJ...140.1512B,
   author = {{Buchdahl}, H.~A.},
    title = "{A Relativistic Fluid Sphere Resembling the Emden Polytrope of Index 5.}",
  journal = {\apj},
     year = 1964,
    month = nov,
   volume = 140,
    pages = {1512},
      doi = {10.1086/148055},
   adsurl = {http://adsabs.harvard.edu/abs/1964ApJ...140.1512B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%% ============================================================
%% ====== Callen H et al.  ======
%% ============================================================

%
@book{callen1985thermodynamics,
  title={Thermodynamics and an Introduction to Thermostatistics},
  author={Callen, Herbert B},
  year={1985},
  publisher={John Wiley \& Sons},
  address={New York}
}

%% ============================================================
%% ====== Chudakova EM et al.  ======
%% ============================================================

% 2014ARep...58..281C,
@ARTICLE{chudakova2014ARep,
   author = {{Chudakova}, E. M. and {Sil'chenko}, O. K.},
    title = "{The thickness of stellar disks in early-type galaxies}",
  journal = {Astronomy Reports},
archivePrefix = "arXiv",
   eprint = {1410.6713},
     year = 2014,
    month = may,
   volume = 58,
    pages = {281-290},
      doi = {10.1134/S1063772914050023},
   adsurl = {http://adsabs.harvard.edu/abs/2014ARep...58..281C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Chicone C et al.  ======
%% ============================================================

% 2002CQGra..19.4231C,
@ARTICLE{chiconeMashoon2002CQGra,
   author = {{Chicone}, C. and {Mashhoon}, B.},
    title = "{The generalized Jacobi equation}",
  journal = {Classical and Quantum Gravity},
   eprint = {gr-qc/0203073},
     year = 2002,
    month = aug,
   volume = 19,
    pages = {4231-4248},
      doi = {10.1088/0264-9381/19/16/301},
   adsurl = {http://adsabs.harvard.edu/abs/2002CQGra..19.4231C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Coimbra-Araujo C et al.  ======
%% ============================================================

% PhysRevD.76.043522,
@article{coimbraLetelier2007PRD,
  title = {Thin disk in higher dimensional space-time and dark matter interpretation},
  author = {Coimbra-Ara\'ujo, Carlos H. and Letelier, Patricio S.},
  journal = {Phys. Rev. D},
  volume = {76},
  issue = {4},
  pages = {043522},
  numpages = {17},
  year = {2007},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.76.043522},
  adsurl = {http://link.aps.org/doi/10.1103/PhysRevD.76.043522}
}

%% ============================================================
%% ====== Coley  ======
%% ============================================================

@ARTICLE{1994CQGra..11.2553C,
   author = {{Coley}, A. A. and {Tupper}, B. O. J.},
    title = "{Spherically symmetric anisotropic fluid ICKV spacetimes}",
  journal = {Classical and Quantum Gravity},
     year = 1994,
    month = oct,
   volume = 11,
    pages = {2553-2574},
      doi = {10.1088/0264-9381/11/10/015},
   adsurl = {http://adsabs.harvard.edu/abs/1994CQGra..11.2553C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



%% ============================================================
%% ====== Contopoulos G et al.  ======
%% ============================================================


%
@article{contopoulos2001development,
  title={The development of nonlinear dynamics in astronomy},
  author={Contopoulos, G},
  journal={Foundations of Physics},
  volume={31},
  number={1},
  pages={89--114},
  year={2001},
  publisher={Springer}
}

% 2002ocda.book.....C,
@BOOK{contopoulosOCDA2002,
   author = {{Contopoulos}, G.},
    title = "{Order and chaos in dynamical astronomy}",
 keywords = {CELESTIAL MECHANICS, ASTRODYNAMICS, DYNAMICS, CHAOS},
  publisher = {Springer-Verlag},
booktitle = {Order and chaos in dynamical astronomy /George Contopoulos. Berlin : Springer, c2002.  (Astronomy and astrophys library) QB 351 .K58 2002},
     year = 2002,
   adsurl = {http://adsabs.harvard.edu/abs/2002ocda.book.....C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1960ZA.....49..273C,
@ARTICLE{contopoulos1960ZA,
   author = {{Contopoulos}, G.},
    title = "{A third Integral of Motion in a Galaxy}",
  journal = {\zap},
     year = 1960,
   volume = 49,
    pages = {273},
   adsurl = {http://adsabs.harvard.edu/abs/1960ZA.....49..273C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1963AJ.....68....1C,
@ARTICLE{contopoulos1963AJ,
   author = {{Contopoulos}, G.},
    title = "{On the existence of a third integral of motion}",
  journal = {\aj},
     year = 1963,
    month = feb,
   volume = 68,
    pages = {1},
      doi = {10.1086/108903},
   adsurl = {http://adsabs.harvard.edu/abs/1963AJ.....68....1C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Coperstook et al  ======
%% ============================================================

@article{doi:10.1142/S0217751X0703666X,
author = {Cooperstock, F. I. and Tieu, S.},
title = {GALACTIC DYNAMICS VIA GENERAL RELATIVITY: A COMPILATION AND NEW DEVELOPMENTS},
journal = {International Journal of Modern Physics A},
volume = {22},
number = {13},
pages = {2293-2325},
year = {2007},
doi = {10.1142/S0217751X0703666X},

%URL = {http://www.worldscientific.com/doi/abs/10.1142/S0217751X0703666X},
%eprint = {http://www.worldscientific.com/doi/pdf/10.1142/S0217751X0703666X}
}

@Article{Carrick2012,
author="Carrick, J. D.
and Cooperstock, F. I.",
title="General relativistic dynamics applied to the rotation curves of galaxies",
journal="Astrophysics and Space Science",
year="2012",
month="Jan",
day="01",
volume="337",
number="1",
pages="321--329",
abstract="We extend our general relativistic analysis of galactic rotation curves (see Cooperstock and Tieu in Int. J. Mod. Phys. A 22:2293, 2007) with galaxies NGC 2841, NGC 2903 and NGC 5033. As before, we employ the solution of the Einstein field equations of general relativity with an expansion in Bessel functions. As in our earlier studies, the fits to the data are found to be very precise and the calculated baryonic masses are lower than those based upon Newtonian gravity. Also as in our previous studies, the galactic radii at which the optical luminosities terminate are seen to correlate with densities near 10â21.75 kg{\thinspace}mâ3. This concordance lends further support to the correctness of the procedure as well as providing a potentially valuable piece of information in the understanding of galactic evolution.",
%issn="1572-946X",
%doi="10.1007/s10509-011-0854-z",
%url="http://dx.doi.org/10.1007/s10509-011-0854-z"
}




%% ============================================================
%% ====== Corchero  ======
%% ============================================================

@article{0264-9381-15-11-022,
  author={E S Corchero},
  title={Equilibrium of spheres with local anisotropy in post-Newtonian gravity. Application to supermassive stars},
  journal={Classical and Quantum Gravity},
  volume={15},
  number={11},
  pages={3645},
  year={1998},
  %url={http://stacks.iop.org/0264-9381/15/i=11/a=022},
  abstract={A generalization of the theory of stellar equilibrium is proposed which involves the possibility of local anisotropy (unequal principal stresses) even if the star is formed by an otherwise perfect fluid. Using this theory, supermassive stars are studied in the post-Newtonian approximation and it is shown that there are equilibrium configurations with local anisotropy having mass above, or entropy below, the standard limit with local isotropy.}
}


%% ============================================================
%% ====== Das  ======
%% ============================================================


@article{doi:10.1063/1.532002,
author = {A. Das and N. Tariq and D. Aruliah and T. Biech},
title = {Spherically symmetric collapse of an anisotropic fluid body into an exotic black hole},
journal = {Journal of Mathematical Physics},
volume = {38},
number = {8},
pages = {4202-4227},
year = {1997},
doi = {10.1063/1.532002},

%URL = {http://dx.doi.org/10.1063/1.532002

}

@article{doi:10.1063/1.1621056,
author = {A. Das and A. DeBenedictis and N. Tariq},
title = {General solutions of Einstein spherically symmetric gravitational equations with junction conditions},
journal = {Journal of Mathematical Physics},
volume = {44},
number = {12},
pages = {5637-5655},
year = {2003},
doi = {10.1063/1.1621056},

%URL = {http://aip.scitation.org/doi/abs/10.1063/1.1621056

}

@article{PhysRevD.62.104002,
  title = {Analytical solutions of a spherically symmetric collapse of an anisotropic fluid body into a regular black hole},
  author = {Das, A. and Kloster, S.},
  journal = {Phys. Rev. D},
  volume = {62},
  issue = {10},
  pages = {104002},
  numpages = {10},
  year = {2000},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.62.104002},
 % url = {https://link.aps.org/doi/10.1103/PhysRevD.62.104002}
}






%% ============================================================
%% ====== de Blok WJ et al.  ======
%% ============================================================

% 1997MNRAS.290..533D,
@ARTICLE{deblokMcgaugh1997MNRAS,
   author = {{de Blok}, W. J. G. and {McGaugh}, S. S.},
    title = "{The dark and visible matter content of low surface brightness disc galaxies}",
  journal = {\mnras},
   eprint = {astro-ph/9704274},
 keywords = {GALAXIES: FUNDAMENTAL PARAMETERS, GALAXIES: HALOES, GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: SPIRAL, DARK MATTER},
     year = 1997,
    month = sep,
   volume = 290,
    pages = {533-552},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.290..533D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Deg N et al.  ======
%% ============================================================

% 2013MNRAS.428..912D,
@ARTICLE{degWidrow2013MNRAS,
   author = {{Deg}, N. and {Widrow}, L.},
    title = "{The Sagittarius stream and halo triaxiality}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1209.6614},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2013,
    month = jan,
   volume = 428,
    pages = {912-922},
      doi = {10.1093/mnras/sts089},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.428..912D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Dejonghe H et al.  ======
%% ============================================================

% 1988ApJ...333...90D,
@ARTICLE{dejongheDezeeuw1988ApJ,
   author = {{Dejonghe}, H. and {de Zeeuw}, T.},
    title = "{Analytic axisymmetric galaxy models with three integrals of motion}",
  journal = {\apj},
 keywords = {Astronomical Models, Galactic Structure, Stellar Motions, Axisymmetric Flow, Cylindrical Coordinates},
     year = 1988,
    month = oct,
   volume = 333,
    pages = {90-129},
      doi = {10.1086/166727},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...333...90D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== de Zeeuw T et al.  ======
%% ============================================================

% 1985MNRAS.216..273D,
@ARTICLE{dezeeuw1985MNRAS,
   author = {{de Zeeuw}, T.},
    title = "{Elliptical galaxies with separable potentials}",
  journal = {\mnras},
 keywords = {Celestial Mechanics, Elliptical Galaxies, Equations Of Motion, Galactic Structure, Gravitational Fields, Stellar Orbits, Astronomical Models, Density Distribution, Many Body Problem, Mass Distribution},
     year = 1985,
    month = sep,
   volume = 216,
    pages = {273-334},
   adsurl = {http://adsabs.harvard.edu/abs/1985MNRAS.216..273D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1987IAUS..127..271D,
@INPROCEEDINGS{dezeeuw1987IAUS,
   author = {{de Zeeuw}, P. T.},
    title = "{Dynamical models for axisymmetric and triaxial galaxies}",
 keywords = {Astronomical Models, Dynamic Models, Elliptical Galaxies, Galactic Structure, Distribution Functions, Hydrodynamics, Integrals, Stellar Motions},
booktitle = {Structure and Dynamics of Elliptical Galaxies},
     year = 1987,
   series = {IAU Symposium},
   volume = 127,
   editor = {{de Zeeuw}, P. T.},
    pages = {271-289},
   adsurl = {http://adsabs.harvard.edu/abs/1987IAUS..127..271D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1988NYASA.536...15D,
@ARTICLE{dezeeuw1988NYASA,
   author = {{de Zeeuw}, T.},
    title = "{Integrable Models for Galaxies}",
  journal = {Annals of the New York Academy of Sciences},
     year = 1988,
    month = aug,
   volume = 536,
    pages = {15-24},
      doi = {10.1111/j.1749-6632.1988.tb51558.x},
   adsurl = {http://adsabs.harvard.edu/abs/1988NYASA.536...15D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1990ApJ...356..365D,
@ARTICLE{dezeeuwHunter1990ApJ,
   author = {{de Zeeuw}, P. T. and {Hunter}, C.},
    title = "{Oblate galaxy models with thin tube orbits}",
  journal = {\apj},
 keywords = {Astronomical Models, Galactic Structure, Distribution Functions, Integral Equations, Kinematics, Orbital Mechanics, Stellar Motions, Velocity Distribution},
     year = 1990,
    month = jun,
   volume = 356,
    pages = {365-388},
      doi = {10.1086/168846},
   adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...356..365D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ======Dev et al.  ======
%% ============================================================


@article{Dev:2000gt,
      author         = "Dev, Krsna and Gleiser, Marcelo",
      title          = "{Anisotropic stars: Exact solutions}",
      journal        = "Gen. Rel. Grav.",
      volume         = "34",
      year           = "2002",
      pages          = "1793-1818",
      doi            = "10.1023/A:1020707906543",
      %eprint         = "astro-ph/0012265",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0012265;%%"
}


%% ============================================================
%% ====== d'Inverno R et al.  ======
%% ============================================================

%
@book{dinverno,
  title={Introducing Einstein's Relativity},
  year={1992},
  author={d'Inverno, RA},
  publisher={Oxford University Press},
  address ={Oxford}
}

%% ============================================================
%% ====== Eddington  ======
%% ============================================================


@ARTICLE{1916MNRAS..76..572E,
   author = {{Eddington}, A. S.},
    title = "{The distribution of stars in globular clusters}",
  journal = {\mnras},
     year = 1916,
    month = may,
   volume = 76,
    pages = {572-585},
      doi = {10.1093/mnras/76.7.572},
   adsurl = {http://adsabs.harvard.edu/abs/1916MNRAS..76..572E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Efthymiopoulos C et al.  ======
%% ============================================================

% 2007LNP...729..297E,
@INPROCEEDINGS{efthymiopoulosEtal2007LNP,
   author = {{Efthymiopoulos}, C. and {Voglis}, N. and {Kalapotharakos}, C.
	},
    title = "{Special Features of Galactic Dynamics}",
 keywords = {Galactic dynamics, Celestial Mechanics, Dynamical Systems},
booktitle = {Topics in Gravitational Dynamics: Solar, Extra-Solar and Galactic Systems.},
     year = 2007,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 729,
   eprint = {astro-ph/0610246},
   editor = {{Benest}, D. and {Froeschle}, C. and {Lega}, E.},
    pages = {297-389},
      doi = {10.1007/978-3-540-72984-6\_11},
   adsurl = {http://adsabs.harvard.edu/abs/2007LNP...729..297E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2010EPJST.186...91E,
@ARTICLE{efthymiopoulos2010EPJST,
   author = {{Efthymiopoulos}, C.},
    title = "{Special features of galactic dynamics: Disc dynamics}",
  journal = {European Physical Journal Special Topics},
     year = 2010,
    month = sep,
   volume = 186,
    pages = {91-122},
      doi = {10.1140/epjst/e2010-01261-8},
   adsurl = {http://adsabs.harvard.edu/abs/2010EPJST.186...91E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Evans et al.  ======
%% ============================================================

@ARTICLE{2005MNRAS.360..492E,
   author = {{Evans}, N. W. and {An}, J.},
    title = "{Hypervirial models of stellar systems}",
  journal = {\mnras},
   eprint = {astro-ph/0501091},
 keywords = {stellar dynamics, celestial mechanics, galaxies: elliptical and lenticular, cD, galaxies: kinematics and dynamics, galaxies: structure},
     year = 2005,
    month = jun,
   volume = 360,
    pages = {492-498},
      doi = {10.1111/j.1365-2966.2005.09078.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.360..492E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Famaey B et al.  ======
%% ============================================================

% 2005MNRAS.363..603F,
@ARTICLE{famaeyBinney2005MNRAS,
   author = {{Famaey}, B. and {Binney}, J.},
    title = "{Modified Newtonian dynamics in the Milky Way}",
  journal = {\mnras},
   eprint = {astro-ph/0506723},
 keywords = {gravitation, Galaxy: kinematics and dynamics},
     year = 2005,
    month = oct,
   volume = 363,
    pages = {603-608},
      doi = {10.1111/j.1365-2966.2005.09474.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.363..603F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2012LRR....15...10F,
@ARTICLE{famaeyMcgaugh2012LRR,
   author = {{Famaey}, B. and {McGaugh}, S. S.},
    title = "{Modified Newtonian Dynamics (MOND): Observational Phenomenology and Relativistic Extensions}",
  journal = {Living Reviews in Relativity},
archivePrefix = "arXiv",
   eprint = {1112.3960},
 keywords = {astronomical observations, Newtonian limit, equations of motion, extragalactic astronomy, cosmology, theories of gravity, fundamental physics, astrophysics},
     year = 2012,
    month = sep,
   volume = 15,
    pages = {10},
      doi = {10.12942/lrr-2012-10},
   adsurl = {http://adsabs.harvard.edu/abs/2012LRR....15...10F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2012sf2a.conf...15F,
@INPROCEEDINGS{famaey2012SF2A,
   author = {{Famaey}, B.},
    title = "{Gaia and the dynamics of the Galaxy}",
 keywords = {Galaxy: kinematics and dynamics, Galaxy: evolution},
booktitle = {SF2A-2012: Proceedings of the Annual meeting of the French Society of Astronomy and Astrophysics},
     year = 2012,
archivePrefix = "arXiv",
   eprint = {1209.5753},
 primaryClass = "astro-ph.GA",
   editor = {{Boissier}, S. and {de Laverny}, P. and {Nardetto}, N. and {Samadi}, R. and
	{Valls-Gabaud}, D. and {Wozniak}, H.},
    month = dec,
    pages = {15-24},
   adsurl = {http://adsabs.harvard.edu/abs/2012sf2a.conf...15F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Freeman K et al.  ======
%% ============================================================

%1970ApJ...160..811F,
@ARTICLE{freeman1970ApJ,
   author = {{Freeman}, K. C.},
    title = "{On the Disks of Spiral and so Galaxies}",
  journal = {\apj},
     year = 1970,
    month = jun,
   volume = 160,
    pages = {811},
      doi = {10.1086/150474},
   adsurl = {http://adsabs.harvard.edu/abs/1970ApJ...160..811F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Garcia A et al.  ======
%% ============================================================

% 2013arXiv1306.2549G,
@ARTICLE{garciaHackmannEtal2013arxiv,
   author = {{Garcia}, A. and {Hackmann}, E. and {Kunz}, J. and {L{\"a}mmerzahl}, C. and
	{Macias}, A.},
    title = "{Motion of test particles in a regular black hole space--time}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1306.2549},
 primaryClass = "gr-qc",
 keywords = {General Relativity and Quantum Cosmology},
     year = 2013,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1306.2549G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Geroch R et al.  ======
%% ============================================================

% 1987PhRvD..36.1017G,
@ARTICLE{gerochTraschen1987PRD,
   author = {{Geroch}, R. and {Traschen}, J.},
    title = "{Strings and other distributional sources in general relativity}",
  journal = {\prd},
 keywords = {Fundamental problems and general formalism},
     year = 1987,
    month = aug,
   volume = 36,
    pages = {1017-1031},
      doi = {10.1103/PhysRevD.36.1017},
   adsurl = {http://adsabs.harvard.edu/abs/1987PhRvD..36.1017G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Gonzalez GA et al.  ======
%% ============================================================

%1999CQGra..16..479G,
@ARTICLE{gonzalezLetelier1999CQGra,
   author = {{Gonz{\'a}lez}, G. A. and {Letelier}, P. S.},
    title = "{Relativistic static thin discs with radial stress support}",
  journal = {Classical and Quantum Gravity},
   eprint = {gr-qc/9803071},
     year = 1999,
    month = feb,
   volume = 16,
    pages = {479-494},
      doi = {10.1088/0264-9381/16/2/012},
   adsurl = {http://adsabs.harvard.edu/abs/1999CQGra..16..479G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%2006MNRAS.371.1873G,
@ARTICLE{gonzalezReina2006MNRAS,
   author = {{Gonz{\'a}lez}, G. A. and {Reina}, J. I.},
    title = "{An infinite family of generalized Kalnajs discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0806.4266},
 keywords = {stellar dynamics: galaxies: kinematics and dynamics, stellar dynamics, galaxies: kinematics and dynamics},
     year = 2006,
    month = oct,
   volume = 371,
    pages = {1873-1876},
      doi = {10.1111/j.1365-2966.2006.10819.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.371.1873G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%2010MNRAS.404..468G,
@ARTICLE{gonzalezPlataplataRamoscaro2010MNRAS,
   author = {{Gonz{\'a}lez}, G. A. and {Plata-Plata}, S. M. and {Ramos-Caro}, J.},
    title = "{Finite thin disc models of four galaxies in the UrsaMajor cluster: NGC3877, NGC3917, NGC3949 and NGC4010}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0906.1355},
 primaryClass = "astro-ph.GA",
 keywords = {stellar dynamics, galaxies: kinematics and dynamics},
     year = 2010,
    month = may,
   volume = 404,
    pages = {468-474},
      doi = {10.1111/j.1365-2966.2010.16303.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.404..468G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% gonzalez2012stationary
@article{gonzalezGutierrez2012CQGra,
  title={Stationary axially symmetric relativistic thin discs with nonzero radial pressure},
  author={Gonz{\'a}lez, Guillermo A and Guti{\'e}rrez-Pi{\ n}eres, Antonio C},
  journal={Classical and Quantum Gravity},
  volume={29},
  number={13},
  pages={135001},
  year={2012},
  publisher={IOP Publishing}
}


%% ============================================================
%% ====== Håkan Andréasson  ======
%% ============================================================

@Article{Andreasson2011,

author="Andr{\'e}asson, H{\aa}kan",

title="The Einstein-Vlasov System/Kinetic Theory",

journal="Living Reviews in Relativity",
year="2011",
month="May",
day="27",
volume="14",
number="1",
pages="4",

abstract="The main purpose of this article is to provide a guide to theorems on global properties of solutions to the Einstein-Vlasov system. This system couples Einstein's equations to a kinetic matter model. Kinetic theory has been an important field of research during several decades in which the main focus has been on non-relativistic and special relativistic physics, i.e., to model the dynamics of neutral gases, plasmas, and Newtonian self-gravitating systems. In 1990, Rendall and Rein initiated a mathematical study of the Einstein-Vlasov system. Since then many theorems on global properties of solutions to this system have been established. This paper gives introductions to kinetic theory in non-curved spacetimes and then the Einstein-Vlasov system is introduced. We believe that a good understanding of kinetic theory in non-curved spacetimes is fundamental to a good comprehension of kinetic theory in general relativity.",

issn="1433-8351",

doi="10.12942/lrr-2011-4",

url="http://dx.doi.org/10.12942/lrr-2011-4"
}




%% ============================================================
%% ====== Hawking SW et al.  ======
%% ============================================================

%
@book{hawkingEllisLSS,
  author = {{Hawking}, S. W. and {Ellis}, G. F. R.},
  title  = {The Large-Scale Structure of Space-Time},
  publisher = {Cambridge Univ. Press},
  year = {2008},
  address = {Cambridge, UK}	
}

%% ============================================================
%% ====== Helmi A et al.  ======
%% ============================================================

% 2004MNRAS.351..643H,
@ARTICLE{helmi2004MNRAS,
   author = {{Helmi}, A.},
    title = "{Is the dark halo of our Galaxy spherical?}",
  journal = {\mnras},
   eprint = {astro-ph/0309579},
 keywords = {Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure, galaxies: haloes, dark matter},
     year = 2004,
    month = jun,
   volume = 351,
    pages = {643-648},
      doi = {10.1111/j.1365-2966.2004.07812.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.351..643H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Henon M et al.  ======
%% ============================================================

% 1964AJ.....69...73H,
@ARTICLE{henonheiles1964AJ,
   author = {{Henon}, M. and {Heiles}, C.},
    title = "{The applicability of the third integral of motion: Some numerical experiments}",
  journal = {\aj},
     year = 1964,
    month = feb,
   volume = 69,
    pages = {73},
      doi = {10.1086/109234},
   adsurl = {http://adsabs.harvard.edu/abs/1964AJ.....69...73H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Hernandez-Pastora JL et al.  ======
%% ============================================================	

% 2013PhRvD..88f4041H,
@ARTICLE{hernandezpastoraHerreraOspino2013PRD,
   author = {{Hern\'{a}ndez-Pastora}, J. L. and {Herrera}, L. and {Ospino}, J.
	},
    title = "{Geodesics in the linearized multipole solution: Distinguishing black holes from naked singularities}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1309.2455},
 primaryClass = "gr-qc",
 keywords = {Fundamental problems and general formalism, Singularities and cosmic censorship, Experimental tests of gravitational theories, Black holes},
     year = 2013,
    month = sep,
   volume = 88,
   number = 6,
      eid = {064041},
    pages = {064041},
      doi = {10.1103/PhysRevD.88.064041},
   adsurl = {http://adsabs.harvard.edu/abs/2013PhRvD..88f4041H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{doi:10.1139/p03-124,
author = {H. Hern\'{a}ndez and L. A. Nu\~{n}ez},
title = {Nonlocal equation of state in anisotropic static fluid spheres in general relativity},
journal = {Canadian Journal of Physics},
volume = {82},
number = {1},
pages = {29-51},
year = {2004},
doi = {10.1139/p03-124},

%URL = {https://doi.org/10.1139/p03-124

}

%% ============================================================
%% ====== Hernquist L et al.  ======
%% ============================================================	

% 1990ApJ...356..359H,
@ARTICLE{hernquist1990ApJ,
   author = {{Hernquist}, L.},
    title = "{An analytical model for spherical galaxies and bulges}",
  journal = {\apj},
 keywords = {Computational Astrophysics, Elliptical Galaxies, Galactic Bulge, Galactic Structure, Astronomical Models, Astronomical Photometry, Brightness Distribution, Distribution Functions},
     year = 1990,
    month = jun,
   volume = 356,
    pages = {359-364},
      doi = {10.1086/168845},
   adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...356..359H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


7%% ============================================================
%% ====== Herrera et al.  ======
%% ============================================================

@ARTICLE{1997PhR...286...53H,
   author = {{Herrera}, L. and {Santos}, N. O.},
    title = "{Local anisotropy in self-gravitating systems}",
  journal = {\physrep},
     year = 1997,
    month = jul,
   volume = 286,
    pages = {53-130},
      doi = {10.1016/S0370-1573(96)00042-7},
   adsurl = {http://adsabs.harvard.edu/abs/1997PhR...286...53H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{HERRERA1998113,
title = "On the role of density inhomogeneity and local anisotropy in the fate of spherical collapse",
journal = "Physics Letters A",
volume = "237",
number = "3",
pages = "113 - 118",
year = "1998",
note = "",
doi = "http://dx.doi.org/10.1016/S0375-9601(97)00874-8",
author = "L. Herrera and A. Di Prisco and J.L. Hern\'{a}ndez-Pastora and N.O Santos",
%issn = "0375-9601",
%url = "http://www.sciencedirect.com/science/article/pii/S0375960197008748",
}

@article{PhysRevD.69.084026,
  title = {Spherically symmetric dissipative anisotropic fluids: A general study},
  author = {Herrera, L. and Di Prisco, A. and Martin, J. and Ospino, J. and Santos, N. O. and Troconis, O.},
  journal = {Phys. Rev. D},
  volume = {69},
  issue = {8},
  pages = {084026},
  numpages = {12},
  year = {2004},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.69.084026},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.69.084026}
}

@article{PhysRevD.77.027502,
  title = {All static spherically symmetric anisotropic solutions of Einstein's equations},
  author = {Herrera, L. and Ospino, J. and Di Prisco, A.},
  journal = {Phys. Rev. D},
  volume = {77},
  issue = {2},
  pages = {027502},
  numpages = {3},
  year = {2008},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.77.027502},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.77.027502}
}

@article{PhysRevD.87.087303,
  title = {Newtonian polytropes for anisotropic matter: General framework and applications},
  author = {Herrera, L. and Barreto, W.},
  journal = {Phys. Rev. D},
  volume = {87},
  issue = {8},
  pages = {087303},
  numpages = {5},
  year = {2013},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.87.087303},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.87.087303}
}







%% ============================================================
%% ====== Hieratinta J et al.  ======
%% ============================================================

% 1987PhR...147...87H,
@ARTICLE{hieratinta1987PhR,
   author = {{Hietarinta}, J.},
    title = "{Direct methods for the search of the second invariant}",
  journal = {\physrep},
     year = 1987,
    month = mar,
   volume = 147,
    pages = {87-154},
      doi = {10.1016/0370-1573(87)90089-5},
   adsurl = {http://adsabs.harvard.edu/abs/1987PhR...147...87H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Hirata CM et al.  ======
%% ============================================================

% 2011MNRAS.414.3198H,
@ARTICLE{hirata2011MNRAS1,
   author = {{Hirata}, C. M.},
    title = "{Lindblad resonance torques in relativistic discs - I. Basic equations}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1010.0758},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, black hole physics, relativistic processes},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {3198-3211},
      doi = {10.1111/j.1365-2966.2011.18617.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.3198H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2011MNRAS.414.3212H,
@ARTICLE{hirata2011MNRAS2,
   author = {{Hirata}, C. M.},
    title = "{Lindblad resonance torques in relativistic discs - II. Computation of resonance strengths}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1010.0759},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, black hole physics, relativistic processes},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {3212-3230},
      doi = {10.1111/j.1365-2966.2011.18619.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.3212H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Holmberg J et al.  ======
%% ============================================================	

% 2004MNRAS.352..440H,
@ARTICLE{holmbergFlynn2004MNRAS,
   author = {{Holmberg}, J. and {Flynn}, C.},
    title = "{The local surface density of disc matter mapped by Hipparcos}",
  journal = {\mnras},
   eprint = {astro-ph/0405155},
 keywords = {Galaxy: kinematics and dynamics, Galaxy: structure, dark matter},
     year = 2004,
    month = aug,
   volume = 352,
    pages = {440-446},
      doi = {10.1111/j.1365-2966.2004.07931.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.352..440H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Hunter C et al.  ======
%% ============================================================	

% 1963MNRAS.126..299H,
@ARTICLE{hunter1963MNRAS,
   author = {{Hunter}, C.},
    title = "{The structure and stability of self-gravitating disks}",
  journal = {\mnras},
     year = 1963,
   volume = 126,
    pages = {299},
   adsurl = {http://adsabs.harvard.edu/abs/1963MNRAS.126..299H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2003LNP...626..137H,
@INPROCEEDINGS{hunter2003LNP,
   author = {{Hunter}, C.},
    title = "{Disk-Crossing Orbits}",
booktitle = {Galaxies and Chaos},
     year = 2003,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 626,
   editor = {{Contopoulos}, G. and {Voglis}, N.},
    pages = {137-153},
      doi = {10.1007/978-3-540-45040-5\_11},
   adsurl = {http://adsabs.harvard.edu/abs/2003LNP...626..137H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2005NYASA1045..120H,
@ARTICLE{hunter2005NYASA,
   author = {{Hunter}, C.},
    title = "{Chaos in Orbits Due to Disk Crossings}",
  journal = {Annals of the New York Academy of Sciences},
     year = 2005,
    month = jan,
   volume = 1045,
    pages = {120},
      doi = {10.1196/annals.1350.011},
   adsurl = {http://adsabs.harvard.edu/abs/2005NYASA1045..120H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Ibata RA et al.  ======
%% ============================================================	

% 2013ApJ...765L..15I,
@ARTICLE{ibataEtal2013ApJL,
   author = {{Ibata}, R. and {Lewis}, G. F. and {Martin}, N. F. and {Bellazzini}, M. and
	{Correnti}, M.},
    title = "{Does the Sagittarius Stream Constrain the Milky Way Halo to be Triaxial?}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1212.4958},
 primaryClass = "astro-ph.GA",
 keywords = {dark matter, galaxies: dwarf, Galaxy: halo },
     year = 2013,
    month = mar,
   volume = 765,
      eid = {L15},
    pages = {L15},
      doi = {10.1088/2041-8205/765/1/L15},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...765L..15I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Iorio L et al.  ======
%% ============================================================	

% 2012EM&P..108..189I,
@ARTICLE{iorio2012EMP,
   author = {{Iorio}, L.},
    title = "{Orbital Perturbations Due to Massive Rings}",
  journal = {Earth Moon and Planets},
archivePrefix = "arXiv",
   eprint = {1201.5307},
 primaryClass = "gr-qc",
 keywords = {Gravity, Asteroid belt, Interplanetary dust, Perturbation methods},
     year = 2012,
    month = jun,
   volume = 108,
    pages = {189-217},
      doi = {10.1007/s11038-012-9391-1},
   adsurl = {http://adsabs.harvard.edu/abs/2012EM%26P..108..189I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Irrgang A et al.  ======
%% ============================================================	

% 2013A&A...549A.137I,
@ARTICLE{irrgangEtal2013AA,
   author = {{Irrgang}, A. and {Wilcox}, B. and {Tucker}, E. and {Schiefelbein}, L.
	},
    title = "{Milky Way mass models for orbit calculations}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1211.4353},
 primaryClass = "astro-ph.GA",
 keywords = {dark matter, Galaxy: fundamental parameters, Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure, stars: kinematics and dynamics},
     year = 2013,
    month = jan,
   volume = 549,
      eid = {A137},
    pages = {A137},
      doi = {10.1051/0004-6361/201220540},
   adsurl = {http://adsabs.harvard.edu/abs/2013A\%26A...549A.137I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Jackson JD et al.  ======
%% ============================================================	

%
@book{jackson1962classical,
  title={Classical electrodynamics},
  author={Jackson, John David and Jackson, John D},
  volume={3},
  year={1962},
  publisher={Wiley New York etc.}
}


%% ============================================================
%% ====== Jaffe  ======
%% ============================================================	

@ARTICLE{1983MNRAS.202..995J,
   author = {{Jaffe}, W.},
    title = "{A simple model for the distribution of light in spherical galaxies}",
  journal = {\mnras},
 keywords = {Astronomical Models, Brightness Distribution, Galactic Radiation, Gravitational Fields, Light Emission, Surface Properties},
     year = 1983,
    month = mar,
   volume = 202,
    pages = {995-999},
      doi = {10.1093/mnras/202.4.995},
   adsurl = {http://adsabs.harvard.edu/abs/1983MNRAS.202..995J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%% ============================================================
%% ====== Johnston KV et al.  ======
%% ============================================================	

% 1995ApJ...451..598J,
@ARTICLE{johnstonEtal1995,
   author = {{Johnston}, K. V. and {Spergel}, D. N. and {Hernquist}, L.},
    title = "{The Disruption of the Sagittarius Dwarf Galaxy}",
  journal = {\apj},
   eprint = {astro-ph/9502005},
 keywords = {GALAXIES: EVOLUTION, GALAXIES: INDIVIDUAL NAME: SAGITTARIUS, GALAXIES: INTERACTIONS, GALAXY: STRUCTURE},
     year = 1995,
    month = oct,
   volume = 451,
    pages = {598},
      doi = {10.1086/176247},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...451..598J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Juric M et al.  ======
%% ============================================================	

% 2008ApJ...673..864J,
@ARTICLE{juricEtal2008ApJ,
   author = {{Juri{\'c}}, M. and {Ivezi{\'c}}, {\v Z}. and {Brooks}, A. and
	{Lupton}, R. H. and {Schlegel}, D. and {Finkbeiner}, D. and
	{Padmanabhan}, N. and {Bond}, N. and {Sesar}, B. and {Rockosi}, C. M. and
	{Knapp}, G. R. and {Gunn}, J. E. and {Sumi}, T. and {Schneider}, D. P. and
	{Barentine}, J. C. and {Brewington}, H. J. and {Brinkmann}, J. and
	{Fukugita}, M. and {Harvanek}, M. and {Kleinman}, S. J. and
	{Krzesinski}, J. and {Long}, D. and {Neilsen}, Jr., E. H. and
	{Nitta}, A. and {Snedden}, S. A. and {York}, D. G.},
    title = "{The Milky Way Tomography with SDSS. I. Stellar Number Density Distribution}",
  journal = {\apj},
   eprint = {astro-ph/0510520},
 keywords = {Galaxy: Disk, Galaxy: Fundamental Parameters, Galaxy: Halo, Galaxy: Structure},
     year = 2008,
    month = feb,
   volume = 673,
    pages = {864-914},
      doi = {10.1086/523619},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...673..864J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Semerak et al.  ======
%% ============================================================	

% 2004CQGra..21R...1K,
@ARTICLE{karasHureSemerak2004CQGra,
   author = {{Karas}, V. and {Hur{\'e}}, J.-M. and {Semer{\'a}k}, O.},
    title = "{TOPICAL REVIEW:  Gravitating discs around black holes}",
  journal = {Classical and Quantum Gravity},
   eprint = {astro-ph/0401345},
     year = 2004,
    month = apr,
   volume = 21,
    pages = {1},
      doi = {10.1088/0264-9381/21/7/R01},
   adsurl = {http://adsabs.harvard.edu/abs/2004CQGra..21R...1K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{0264-9381-17-7-303,
  author={O. Semer\'{a}k and M. Z\'{a}cek},
  title={Gravitating discs around a Schwarzschild black hole: I},
  journal={Classical and Quantum Gravity},
  volume={17},
  number={7},
  pages={1613},
  year={2000},
  abstract={We study the class of Lemos-Letelier annular discs (realistic gravitating static axisymmetric thin discs obtained by inversion of the first Morgan-Morgan solution) around Schwarzschild black holes. For each value of the inner radius, the range of masses is found when all of the disc can be interpreted by counter-rotating streams of particles on stable timelike geodesics. One can then consider a sequence of stable physical discs with different masses and inner rims at the corresponding least possible radii. The basic properties of this sequence are shown on positions of the inner rims and of important circular orbits, on positions of the horizon and on density and Keplerian-velocity profiles within the discs, plotted in terms of the Schwarzschild radial coordinate, circumferential radius and proper distance from the horizon.}
% url={http://stacks.iop.org/0264-9381/17/i=7/a=303},
}

@article{0264-9381-19-14-321,
  author={O Semer\'{a}k},
  title={Thin disc around a rotating black hole, but with support in-between},
  journal={Classical and Quantum Gravity},
  volume={19},
  number={14},
  pages={3829},
  year={2002},
  abstract={In the previous paper, we presented the metric obtained from a general Weyl seed using the BelinskiiâZakharov inverse-scattering technique with two real solitons. It describes the field of a stationary black hole surrounded by a source inherited from the seed. In the present paper, we study the solution in further detail with the inverted first MorganâMorgan counter-rotating disc employed as a seed. In particular, the properties of the horizon, the static limit, the equatorial plane, the extreme limit of the solution and the resulting external disc are analysed and illustrated. It turns out that there is a jump in derivatives of the metric in the equatorial plane even below the seed disc, indicating the presence of a 'suspension layer' that confines the system against gravitational collapse or decay. Hence, the solution cannot represent a realistic axisymmetric accretion disc around a rotating black hole.}
%  url={http://stacks.iop.org/0264-9381/19/i=14/a=321},
}

@Article{semerak2002,
author="{\v{Z}}{\'a}{\v{c}}ek, M.
and Semer{\'a}k, O.",
title="Gravitating discs around a Schwarzschild black hole II",
journal="Czechoslovak Journal of Physics",
year="2002",
month="Jan",
day="01",
volume="52",
number="1",
pages="19--27",
abstract="A sequence of exact spacetimes is obtained describing the fields of a Schwarzschild black hole surrounded by stable static axisymmetric thin discs having their inner rim at the least possible radius. In the previous paper we only required stability with respect to perturbations in the disc plane, while it turns out that for discs with relative mass >0.23 the perturbations in perpendicular direction are more dangerous. The discs of the resulting sequence have their inner rims just on, or very close to, circular geodesics marginally stable with respect to either of the perturbations. Redshift from static and Keplerian observers in the disc is computed. The inverted first Morgan-Morgan counter-rotating disc, used in superpositions, has a number of satisfactory physical properties, but it has turned out to have a curvature singularity at the inner rim. However, this is only a consequence of a too steep radial start of density, not present in (inverted) ``higher'' Morgan-Morgan solutions.",
%issn="1572-9486",
%doi="10.1023/A:1013957512339",
%url="http://dx.doi.org/10.1023/A:1013957512339"
}

%% ============================================================
%% ====== Kehagias A et al.  ======
%% ============================================================	

% 2009PhLB..678..123K,
@ARTICLE{kehagiasSfetsos2009PhLB,
   author = {{Kehagias}, A. and {Sfetsos}, K.},
    title = "{The black hole and FRW geometries of non-relativistic gravity}",
  journal = {Physics Letters B},
archivePrefix = "arXiv",
   eprint = {0905.0477},
 primaryClass = "hep-th",
     year = 2009,
    month = jul,
   volume = 678,
    pages = {123-126},
      doi = {10.1016/j.physletb.2009.06.019},
   adsurl = {http://adsabs.harvard.edu/abs/2009PhLB..678..123K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Kent SM et al.  ======
%% ============================================================	

% 1986AJ.....91.1301K,
@ARTICLE{kent1986AJ,
   author = {{Kent}, S. M.},
    title = "{Dark matter in spiral galaxies. I - Galaxies with optical rotation curves}",
  journal = {\aj},
 keywords = {Brightness Distribution, Galactic Structure, Missing Mass (Astrophysics), Spectral Energy Distribution, Spiral Galaxies, Visible Spectrum, Astronomical Models, Charge Coupled Devices, Mass Distribution, Mass To Light Ratios, Tables (Data)},
     year = 1986,
    month = jun,
   volume = 91,
    pages = {1301-1327},
      doi = {10.1086/114106},
   adsurl = {http://adsabs.harvard.edu/abs/1986AJ.....91.1301K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1987AJ.....93..816K,
@ARTICLE{kent1987AJ,
   author = {{Kent}, S. M.},
    title = "{Dark matter in spiral galaxies. II - Galaxies with H I rotation curves}",
  journal = {\aj},
 keywords = {Angular Velocity, Brightness Distribution, Dark Matter, Hydrogen Clouds, Mass Distribution, Spiral Galaxies, Astronomical Models, Galactic Structure, Mass To Light Ratios, Star Distribution},
     year = 1987,
    month = apr,
   volume = 93,
    pages = {816-832},
      doi = {10.1086/114366},
   adsurl = {http://adsabs.harvard.edu/abs/1987AJ.....93..816K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Kluzniak W et al.  ======
%% ============================================================	

% 2013MNRAS.434.2825K,
@ARTICLE{kluzniakRosinska2013MNRAS,
   author = {{Klu{\'z}niak}, W. and {Rosi{\'n}ska}, D.},
    title = "{Orbital and epicyclic frequencies of Maclaurin spheroids}",
  journal = {\mnras},
 keywords = {black hole physics, dense matter, gravitation, instabilities, stars: neutron},
     year = 2013,
    month = oct,
   volume = 434,
    pages = {2825-2829},
      doi = {10.1093/mnras/stt1185},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.434.2825K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Landau LD et al.  ======
%% ============================================================	

%
@book{landauLifshitzFM,
  author = {{Landau}, L. D. and {Lifshitz}, E. M.}, edition = {Second},
  title  = {Fluid Mechanics},
  publisher = {Elsevier},
  year = {2007},
  address = {Oxford, UK},	
  series = {Course of Theoretical Physics},  volume = {VI},
}

%% ============================================================
%% ====== Law DR et al.  ======
%% ============================================================	

% 2009ApJ...703L..67L,
@ARTICLE{lawEtal2009ApJL,
   author = {{Law}, D. R. and {Majewski}, S. R. and {Johnston}, K. V.},
    title = "{Evidence for a Triaxial Milky Way Dark Matter Halo from the Sagittarius Stellar Tidal Stream}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0908.3187},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2009,
    month = sep,
   volume = 703,
    pages = {L67-L71},
      doi = {10.1088/0004-637X/703/1/L67},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...703L..67L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Lee JM et al.  ======
%% ============================================================	

%
@book{lee2012smooth,
  title={Introduction to smooth manifolds},
  author={Lee, John},
  volume={218},
  year={2012},
  publisher={Springer}
}

%% ============================================================
%% ====== Lemos JPS et al.  ======
%% ============================================================	

% 1994PhRvD..49.5135L,
@ARTICLE{lemosLetelier1994PRD,
   author = {{Lemos}, J. P. S. and {Letelier}, P. S.},
    title = "{Exact general relativistic thin disks around black holes}",
  journal = {\prd},
 keywords = {Exact solutions, Black holes},
     year = 1994,
    month = may,
   volume = 49,
    pages = {5135-5143},
      doi = {10.1103/PhysRevD.49.5135},
   adsurl = {http://adsabs.harvard.edu/abs/1994PhRvD..49.5135L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{0264-9381-10-6-003,
  author={J P S Lemos and P S Letelier},
  title={Superposition of Morgan and Morgan discs with a Schwarzschild black hole},
  journal={Classical and Quantum Gravity},
  volume={10},
  number={6},
  pages={L75},
  year={1993},
  abstract={The exact superposition of a black hole and a thin disc is considered. The disc is made of counter-rotating particles and belongs to the Morgan and Morgan family (1969). There are three parameters to play with, the black hole mass, and the disc mass and radius. The superposed exact solution comprehends several configurations, some yield mass ratios in conformity with the usual accretion discs. There is also a remarkable configuration of a black hole surrounded by a disc made of pure superluminal matter up to the edge, which is at the photonic orbit.}
%url={http://stacks.iop.org/0264-9381/10/i=6/a=003},
}




%% ============================================================
%% ====== Letelier PS et al.  ======
%% ============================================================	

% 2003PhRvD..68j4002L,
@ARTICLE{letelier2003PRD,
   author = {{Letelier}, P. S.},
    title = "{Stability of circular orbits of particles moving around black holes surrounded by axially symmetric structures}",
  journal = {\prd},
   eprint = {gr-qc/0309033},
 keywords = {Classical black holes, Orbit determination and improvement, Infall and accretion, Infall accretion and accretion disks},
     year = 2003,
    month = nov,
   volume = 68,
   number = 10,
      eid = {104002},
    pages = {104002},
      doi = {10.1103/PhysRevD.68.104002},
   adsurl = {http://adsabs.harvard.edu/abs/2003PhRvD..68j4002L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%1987JMP....28..165L,
@ARTICLE{letelierOliveira1987JMP,
   author = {{Letelier}, P. S. and {Oliveira}, S. R.},
    title = "{Exact self-gravitating disks and rings: A solitonic approach}",
  journal = {Journal of Mathematical Physics},
     year = 1987,
    month = jan,
   volume = 28,
    pages = {165-170},
      doi = {10.1063/1.527800},
   adsurl = {http://adsabs.harvard.edu/abs/1987JMP....28..165L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%
@article{letelier2005RBEF,
  title={Solu{\c{c}}{\~o}es exatas das equa{\c{c}}{\~o}es de Einstein com simetria axial},
  author={Letelier, Patricio S},
  journal={Revista Brasileira de Ensino de F{\'\i}sica},
  volume={27},
  number={1},
  pages={121--136},
  year={2005},
  publisher={SciELO Brasil}
}

% 2007MNRAS.381.1031L,
@ARTICLE{letelier2007MNRAS,
   author = {{Letelier}, P. S.},
    title = "{Simple potential-density pairs for flat rings}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0706.2802},
 keywords = {instabilities, planets: rings},
     year = 2007,
    month = nov,
   volume = 381,
    pages = {1031-1034},
      doi = {10.1111/j.1365-2966.2007.12128.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.381.1031L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{PhysRevD.62.064025,
  title = {Rotating relativistic thin disks},
  author = {Gonz\'alez, Guillermo A. and Letelier, Patricio S.},
  journal = {Phys. Rev. D},
  volume = {62},
  issue = {6},
  pages = {064025},
  numpages = {8},
  year = {2000},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.62.064025},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.62.064025}
}


%% ============================================================
%% ====== Lichtenberg AJ et al.  ======
%% ============================================================	

%
@book{lichtenbergLieberman1992,
  title={Regular and Chaotic Dynamics},
  author={Lichtenberg, AJ and Lieberman, M},
  publisher={Springer, New York},
  series={Applied Mathematical Sciences},
  volume={38},
  year={1992}
}

%% ============================================================
%% ====== Lynden-Bell  ======
%% ============================================================	


@ARTICLE{1962MNRAS.123..447L,
   author = {{Lynden-Bell}, D.},
    title = "{Stellar dynamics: Exact solution of the self-gravitation equation}",
  journal = {\mnras},
     year = 1962,
   volume = 123,
    pages = {447},
      doi = {10.1093/mnras/123.5.447},
   adsurl = {http://adsabs.harvard.edu/abs/1962MNRAS.123..447L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%% ============================================================
%% ====== Lora-Clavijo FD et al.  ======
%% ============================================================	

% 2010PhRvD..82h4005L,
@ARTICLE{loraclavijo-ospinahenao-pedraza2010PRD,
   author = {{Lora-Clavijo}, F. D. and {Ospina-Henao}, P. A. and {Pedraza}, J. F.
	},
    title = "{Charged annular disks and Reissner-Nordstr{\"o}m type black holes from extremal dust}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1009.1005},
 primaryClass = "gr-qc",
 keywords = {Exact solutions, Einstein-Maxwell spacetimes spacetimes with fluids radiation or classical fields, Galactic nuclei circumnuclear matter and bulges},
     year = 2010,
    month = oct,
   volume = 82,
   number = 8,
      eid = {084005},
    pages = {084005},
      doi = {10.1103/PhysRevD.82.084005},
   adsurl = {http://adsabs.harvard.edu/abs/2010PhRvD..82h4005L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Maharaj et al.  ======
%% ============================================================

@Article{Maharaj2006,
author="Maharaj, S. D.
and Chaisi, M.",
title="Equation of state for anisotropic spheres",
journal="General Relativity and Gravitation",
year="2006",
month="Nov",
day="01",
volume="38",
number="11",
pages="1723--1726",
abstract="We present a new class of exact interior solutions for anisotropic spheres to the Einstein field equations with a prescribed energy density. This category of solutions has similar energy density profiles to the models of Chaisi and Maharaj (Gen. Rel. Grav. 37, 1177--1189, 2005) whose approach we follow in the integration process. A distinguishing feature of the solutions presented is that they satisfy a barotropic equation of state linearly relating the radial pressure to the energy density.",
%issn="1572-9532",
%doi="10.1007/s10714-006-0353-7",
%url="http://dx.doi.org/10.1007/s10714-006-0353-7"
}

@article {MMA:MMA665,
author = {Maharaj, S. D. and Chaisi, M.},
title = {New anisotropic models from isotropic solutions},
journal = {Mathematical Methods in the Applied Sciences},
volume = {29},
number = {1},
publisher = {John Wiley & Sons, Ltd.},
doi = {10.1002/mma.665},
pages = {67--83},
keywords = {astrophysics, Einstein equations, dense stars},
year = {2006},
%issn = {1099-1476},
%url = {http://dx.doi.org/10.1002/mma.665},
}




%% ============================================================
%% ====== Mak et al.  ======
%% ============================================================	

@article {Mak393,
	author = {Mak, M.K. and Harko, T.},
	title = {Anisotropic stars in general relativity},
	volume = {459},
	number = {2030},
	pages = {393--408},
	year = {2003},
	doi = {10.1098/rspa.2002.1014},
	publisher = {The Royal Society},
	abstract = {We present a class of exact solutions of Einstein{\textquoteright}s gravitational{\textendash}field equations describing spherically symmetric and static anisotropic stellar{\textendash}type configurations. The solutions are obtained by assuming a particular form of the anisotropy factor. The energy density and both radial and tangential pressures are finite and positive inside the anisotropic star. Numerical results show that the basic physical parameters (mass and radius) of the model can describe realistic astrophysical objects such as neutron stars.},
	%issn = {1364-5021},
%	URL = {http://rspa.royalsocietypublishing.org/content/459/2030/393},
%	eprint = {http://rspa.royalsocietypublishing.org/content/459/2030/393.full.pdf},
	journal = {Proceedings of the Royal Society of London A: Mathematical, Physical and Engineering Sciences}
}

%% ============================================================
%% ====== McMillan PJ et al.  ======
%% ============================================================	

% 2008MNRAS.390..429M,
@ARTICLE{mcmillanBinney2008MNRAS,
   author = {{McMillan}, P. J. and {Binney}, J. J.},
    title = "{Disassembling the Galaxy with angle-action coordinates}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0806.0319},
 keywords = {methods: numerical , Galaxy: kinematics and dynamics , solar neighbourhood , Galaxy: structure},
     year = 2008,
    month = oct,
   volume = 390,
    pages = {429-437},
      doi = {10.1111/j.1365-2966.2008.13767.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.390..429M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2011MNRAS.414.2446M,
@ARTICLE{mcmillan2011MNRAS,
   author = {{McMillan}, P. J.},
    title = "{Mass models of the Milky Way}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1102.4340},
 primaryClass = "astro-ph.GA",
 keywords = {methods: statistical, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {2446-2457},
      doi = {10.1111/j.1365-2966.2011.18564.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.2446M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Milgrom M et al.  ======
%% ============================================================	

% 1983ApJ...270..365M,
@ARTICLE{milgrom1983ApJ,
   author = {{Milgrom}, M.},
    title = "{A modification of the Newtonian dynamics as a possible alternative to the hidden mass hypothesis}",
  journal = {\apj},
 keywords = {Cosmology, Galactic Structure, Nonrelativistic Mechanics, Stellar Motions, Particle Acceleration, Solar System},
     year = 1983,
    month = jul,
   volume = 270,
    pages = {365-370},
      doi = {10.1086/161130},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...270..365M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1983ApJ...270..371M,
@ARTICLE{milgrom1983ApJgalaxies,
   author = {{Milgrom}, M.},
    title = "{A modification of the Newtonian dynamics - Implications for galaxies}",
  journal = {\apj},
 keywords = {Galactic Structure, Newton Theory, Stellar Motions, Angular Velocity, Disk Galaxies, Elliptical Galaxies, Galactic Rotation, Mass Distribution, Milky Way Galaxy, Oort Cloud},
     year = 1983,
    month = jul,
   volume = 270,
    pages = {371-389},
      doi = {10.1086/161131},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...270..371M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1983ApJ...270..384M,
@ARTICLE{milgrom1983ApJgalaxysystems,
   author = {{Milgrom}, M.},
    title = "{A Modification of the Newtonian Dynamics - Implications for Galaxy Systems}",
  journal = {\apj},
     year = 1983,
    month = jul,
   volume = 270,
    pages = {384},
      doi = {10.1086/161132},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...270..384M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% 2010MNRAS.403..886M,
@ARTICLE{milgrom2010MNRAS,
   author = {{Milgrom}, M.},
    title = "{Quasi-linear formulation of MOND}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0911.5464},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: kinematics and dynamics, cosmology: theory, dark matter},
     year = 2010,
    month = apr,
   volume = 403,
    pages = {886-895},
      doi = {10.1111/j.1365-2966.2009.16184.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403..886M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% 2014MNRAS.437.2531M,
@ARTICLE{milgrom2014MNRAS,
   author = {{Milgrom}, M.},
    title = "{MOND laws of galactic dynamics}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1212.2568},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: general, galaxies: kinematics and dynamics, dark matter},
     year = 2014,
    month = jan,
   volume = 437,
    pages = {2531-2541},
      doi = {10.1093/mnras/stt2066},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.437.2531M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Mimoso et al. ======
%% ============================================================	

@article{PhysRevD.88.027301,
  title = {Separating expansion and collapse in general fluid models with heat flux},
  author = {Le Delliou, Morgan and Mimoso, Jos\'e P. and Mena, Filipe C. and Fontanini, Michele and Guariento, Daniel C. and Abdalla, Elcio},
  journal = {Phys. Rev. D},
  volume = {88},
  issue = {2},
  pages = {027301},
  numpages = {5},
  year = {2013},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.88.027301},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.88.027301}
}


%% ============================================================
%% ====== Misner CW et al. ======
%% ============================================================	

%
@book{misner1973gravitation,
  title={Gravitation},
  author={Misner, Charles W and Thorne, Kip S and Wheeler, John Archibald},
  year={1973},
  publisher={W. H. Freeman and Company},
  address={San Francisco}
}

%% ============================================================
%% ====== Miyamoto-Nagai  ======
%% ============================================================	

% 1975PASJ...27..533M,
@ARTICLE{miyamotoNagai1975PASJ,
   author = {{Miyamoto}, M. and {Nagai}, R.},
    title = "{Three-dimensional models for the distribution of mass in galaxies}",
  journal = {\pasj},
 keywords = {Astronomical Models, Density Distribution, Galactic Structure, Mass Distribution, Potential Theory, Three Dimensional Models, Functions (Mathematics), Globular Clusters, Gravitational Effects, Mathematical Models, Milky Way Galaxy},
     year = 1975,
   volume = 27,
    pages = {533-543},
   adsurl = {http://adsabs.harvard.edu/abs/1975PASJ...27..533M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Morgan & Morgan  ======
%% ============================================================	

% 1969PhRv..183.1097M,
@ARTICLE{morganMorgan1969PR,
   author = {{Morgan}, T. and {Morgan}, L.},
    title = "{The Gravitational Field of a Disk}",
  journal = {Physical Review},
     year = 1969,
    month = jul,
   volume = 183,
    pages = {1097-1101},
      doi = {10.1103/PhysRev.183.1097},
   adsurl = {http://adsabs.harvard.edu/abs/1969PhRv..183.1097M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1970PhRvD...2.2756M,
@ARTICLE{morganMorgan1970PRD,
   author = {{Morgan}, L. and {Morgan}, T.},
    title = "{Gravitational Field of Shells and Disks in General Relativity}",
  journal = {\prd},
     year = 1970,
    month = dec,
   volume = 2,
    pages = {2756-2761},
      doi = {10.1103/PhysRevD.2.2756},
   adsurl = {http://adsabs.harvard.edu/abs/1970PhRvD...2.2756M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Ollongren A et al.  ======
%% ============================================================	

% 1962BAN....16..241O,
@ARTICLE{ollongren1962BAIN,
   author = {{Ollongren}, A.},
    title = "{Three-dimensional galactic stellar orbits}",
  journal = {\bain},
     year = 1962,
    month = oct,
   volume = 16,
    pages = {241},
   adsurl = {http://adsabs.harvard.edu/abs/1962BAN....16..241O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Nucamendi et al.  ======
%% ============================================================	


@article{1742-6596-545-1-012006,
  author={A Herrera-Aguilar and U Nucamendi},
  title={A relativistic axisymmetric approach to the galactic rotation curves problem},
  journal={Journal of Physics: Conference Series},
  volume={545},
  number={1},
  pages={012006},
  year={2014},
  abstract={It is known that galactic potentials can be kinematically linked to the observed red/blue shifts of the corresponding galactic rotation curves under a minimal set of assumptions (see [1] and [2] for details): i ) that emitted photons come to us from stable timelike circular geodesic orbits of stars in a static spherically symmetric gravitational field, and ii ) that these photons propagate to us along null geodesics. This relation can be established without appealing at all to a concrete theory of gravitational interaction. This kinematical spherically symmetric approach to the galactic rotation curves problem can be generalized to the stationary axisymmetric realm, which is precisely the symmetry that spiral galaxies possess [3]. Here we review the relativistic results obtained in the latter work. Namely, by making use of the most general stationary axisymmetric metric, we consider stable circular orbits of stars that emit signals which travel to a distant observer along null geodesics and express the galactic red/blue shifts in terms of three arbitrary metric functions, clarifying the contribution of the rotation as well as the dragging of the gravitational field. This stationary axisymmetric approach distinguishes between red and blue shifts emitted by circularly orbiting receding and approaching stars, respectively, even when they are considered with respect to the center of a spiral galaxy, indicating the need of precise measurements in order to confront predictions with observations. We also point out the difficulties one encounters in the attempt of determining the metric functions from observations and list some potential strategies to overcome them.}
 % url={http://stacks.iop.org/1742-6596/545/i=1/a=012006},
}



%% ============================================================
%% ====== Papapetrou A et al.  ======
%% ============================================================	


@article{papapetrou1966,
author = {Papapetrou, A.},
journal = {Annales de l'institut Henri Poincar{\'e} (A) Physique th{\'e}orique},
language = {fre},
number = {2},
pages = {83-105},
publisher = {Gauthier-villars},
title = {Champs gravitationnels stationnaires {\`a} sym{\'e}trie axiale},
adsurl = {http://eudml.org/doc/75527},
volume = {4},
year = {1966},
}

%% ============================================================
%% ====== Pauli EM et al.  ======
%% ============================================================	

% 2003A&A...400..877P,
@ARTICLE{pauliEtal2003AA,
   author = {{Pauli}, E.-M. and {Napiwotzki}, R. and {Altmann}, M. and {Heber}, U. and
	{Odenkirchen}, M. and {Kerber}, F.},
    title = "{3D kinematics of white dwarfs from the SPY project}",
  journal = {\aap},
   eprint = {astro-ph/0301467},
 keywords = {stars: white dwarfs, stars: kinematics and dynamics, Galaxy: halo, Galaxy: disk, Galaxy: kinematics and dynamics},
     year = 2003,
    month = mar,
   volume = 400,
    pages = {877-890},
      doi = {10.1051/0004-6361:20030012},
   adsurl = {http://adsabs.harvard.edu/abs/2003A\%26A...400..877P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Pedraza JF et al.  ======
%% ============================================================	

% 2008MNRAS.390.1587P,
@ARTICLE{pedrazaRamoscaroGonzalez2008MNRAS,
   author = {{Pedraza}, J. F. and {Ramos-Caro}, J. and {Gonz{\'a}lez}, G. A.},
    title = "{An infinite family of self-consistent models for axisymmetric flat galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
 keywords = {stellar dynamics , galaxies: kinematics and dynamics},
     year = 2008,
    month = nov,
   volume = 390,
    pages = {1587-1597},
      doi = {10.1111/j.1365-2966.2008.13846.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.390.1587P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
  %  eprint = {0806.4277},
}

@article{PhysRevD.88.064020,
  title = {Anisotropic models for globular clusters, Galactic bulges, and dark halos},
  author = {Nguyen, P. H. and Pedraza, J. F.},
  journal = {Phys. Rev. D},
  volume = {88},
  issue = {6},
  pages = {064020},
  numpages = {27},
  year = {2013},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.88.064020},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.88.064020}
}


@article{PhysRevD.82.084005,
  title = {Charged annular disks and Reissner-Nordstr\"om type black holes from extremal dust},
  author = {Lora-Clavijo, F. D. and Ospina-Henao, P. A. and Pedraza, J. F.},
  journal = {Phys. Rev. D},
  volume = {82},
  issue = {8},
  pages = {084005},
  numpages = {13},
  year = {2010},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.82.084005},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.82.084005}
}






%% ============================================================
%% ====== Persic M et al.  ======
%% ============================================================	

% 1996MNRAS.281...27P,
@ARTICLE{persicSalucci1996MNRAS,
   author = {{Persic}, M. and {Salucci}, P. and {Stel}, F.},
    title = "{The universal rotation curve of spiral galaxies - I. The dark matter connection}",
  journal = {\mnras},
   eprint = {astro-ph/9506004},
 keywords = {GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: SPIRAL, GALAXIES: STRUCTURE, DARK MATTER},
     year = 1996,
    month = jul,
   volume = 281,
    pages = {27-47},
   adsurl = {http://adsabs.harvard.edu/abs/1996MNRAS.281...27P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Plummer  ======
%% ============================================================	

@ARTICLE{1911MNRAS..71..460P,
   author = {{Plummer}, H. C.},
    title = "{On the problem of distribution in globular star clusters}",
  journal = {\mnras},
     year = 1911,
    month = mar,
   volume = 71,
    pages = {460-470},
      doi = {10.1093/mnras/71.5.460},
   adsurl = {http://adsabs.harvard.edu/abs/1911MNRAS..71..460P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





%% ============================================================
%% ====== Pugliese D et al.  ======
%% ============================================================	

% 2011PhRvD..83b4021P,
@ARTICLE{puglieseQuevedoRuffini2011PRD,
   author = {{Pugliese}, D. and {Quevedo}, H. and {Ruffini}, R.},
    title = "{Circular motion of neutral test particles in Reissner-Nordstr{\"o}m spacetime}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1012.5411},
 primaryClass = "astro-ph.HE",
 keywords = {Classical general relativity, Relativistic stars: structure stability and oscillations, Classical black holes},
     year = 2011,
    month = jan,
   volume = 83,
   number = 2,
      eid = {024021},
    pages = {024021},
      doi = {10.1103/PhysRevD.83.024021},
   adsurl = {http://adsabs.harvard.edu/abs/2011PhRvD..83b4021P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Ramos-Caro J et al.  ======
%% ============================================================	

% 2008MNRAS.386..440R,
@ARTICLE{ramoscaroLopezsuspesGonzalez2008MNRAS,
   author = {{Ramos-Caro}, J. and {L{\'o}pez-Suspes}, F. and {Gonz{\'a}lez}, G. A.
	},
    title = "{Chaotic and regular motion around generalized Kalnajs discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0806.4272},
 keywords = {stellar dynamics, galaxies: kinematics and dynamics},
     year = 2008,
    month = may,
   volume = 386,
    pages = {440-446},
      doi = {10.1111/j.1365-2966.2008.13047.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386..440R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2011MNRAS.414.3105R,
@ARTICLE{ramoscaroPedrazaLetelier2011MNRAS,
   author = {{Ramos-Caro}, J. and {Pedraza}, J. F. and {Letelier}, P. S.},
    title = "{Motion around a monopole + ring system - I. Stability of equatorial circular orbits versus regularity of three-dimensional motion}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1103.4616},
 primaryClass = "astro-ph.EP",
 keywords = {chaos, celestial mechanics, planets and satellites: rings},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {3105-3116},
      doi = {10.1111/j.1365-2966.2011.18618.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.3105R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{PhysRevD.86.043008,
  title = {Kinetic theory of collisionless self-gravitating gases. II. Relativistic corrections in galactic dynamics},
  author = {Ramos-Caro, J. and Ag\'on, C. A. and Pedraza, J. F.},
  journal = {Phys. Rev. D},
  volume = {86},
  issue = {4},
  pages = {043008},
  numpages = {15},
  year = {2012},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.86.043008},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.86.043008}
}

@article{0264-9381-25-4-045011,
  author={Javier Ramos-Caro and Guillermo A Gonz\'{a}lez},
  title={FokkerâPlanckâRosenbluth-type equations for self-gravitating systems in the 1PN approximation},
  journal={Classical and Quantum Gravity},
  volume={25},
  number={4},
  pages={045011},
  year={2008},
  abstract={We present two formulations of FokkerâPlanckâRosenbluth-type (FPR) equations for many-particle self-gravitating systems, with first-order relativistic corrections in the post-Newtonian approach (1PN). The first starts from a covariant FokkerâPlanck equation for a simple gas, introduced recently by ChacÃ³n-Acosta and Kremer (2007 Phys. Rev. E 76 021201). The second derivation is based on the establishment of an 1PN-BBGKY hierarchy, developed systematically from the 1PN microscopic law of force and using the KlimontovichâDupree (KD) method. We close the hierarchy by the introduction of a two-point correlation function that describes adequately the relaxation process. This picture reveals an aspect that is not considered in the first formulation: the contribution of ternary correlation patterns to the diffusion coefficients, as a consequence of the nature of 1PN interaction. Both formulations can be considered as a generalization of the equation derived by Rezania and Sobouti (2000 Astron. Astrophys. 354 1110), to stellar systems where the relativistic effects of gravitation play a significant role.}
%  url={http://stacks.iop.org/0264-9381/25/i=4/a=045011},
}

%% ============================================================
%% ====== Rodrigues DC et al.  ======
%% ============================================================	

% 2010JCAP...04..020R,
@ARTICLE{rodriguesShapiroLetelier2010JCAP,
   author = {{Rodrigues}, D. C. and {Letelier}, P. S. and {Shapiro}, I. L.
	},
    title = "{Galaxy rotation curves from general relativity with renormalization group corrections}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {0911.4967},
 primaryClass = "astro-ph.CO",
     year = 2010,
    month = apr,
   volume = 4,
      eid = {020},
    pages = {20},
      doi = {10.1088/1475-7516/2010/04/020},
   adsurl = {http://adsabs.harvard.edu/abs/2010JCAP...04..020R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{1475-7516-2012-09-031,
  author={Davi C. Rodrigues},
  title={Elliptical galaxies kinematics within general relativity with renormalization group effects},
  journal={Journal of Cosmology and Astroparticle Physics},
  volume={2012},
  number={09},
  pages={031},
  year={2012},
  abstract={The renormalization group framework can be applied to Quantum Field Theory on curved space-time, but there is no proof whether the beta-function of the gravitational coupling indeed goes to zero in the far infrared or not. In a recent paper [ 1 [http://dx.doi.org/10.1088/1475-7516/2010/04/020] ] we have shown that the amount of dark matter inside spiral galaxies may be negligible if a small running of the General Relativity coupling G is present (Î´ G / G 0 ##IMG## [http://ej.iop.org/icons/Entities/lesssim.gif] {lesssim} 10 â7 across a galaxy). Here we extend the proposed model to elliptical galaxies and present a detailed analysis on the modeling of NGC 4494 (an ordinary elliptical) and NGC 4374 (a giant elliptical). In order to compare our results to a well known alternative model to the standard dark matter picture, we also evaluate NGC 4374 with MOND. In this galaxy MOND leads to a significative discrepancy with the observed velocity dispersion curve and has a significative tendency towards tangential anisotropy. On the other hand, the approach based on the renormalization group and general relativity (RGGR) could be applied with good results to these elliptical galaxies and is compatible with lower mass-to-light ratios (of about the Kroupa IMF type).}
%url={http://stacks.iop.org/1475-7516/2012/i=09/a=031},
}

%% ============================================================
%% ====== Rosa VM et al.  ======
%% ============================================================	

% 2007GReGr..39.1419R,
@ARTICLE{rosaLetelier2007GRG,
   author = {{Rosa}, V. M. and {Letelier}, P. S.},
    title = "{Stability of closed timelike curves in the G{\"o}del universe}",
  journal = {General Relativity and Gravitation},
   eprint = {gr-qc/0703100},
     year = 2007,
    month = sep,
   volume = 39,
    pages = {1419-1435},
      doi = {10.1007/s10714-007-0464-9},
   adsurl = {http://adsabs.harvard.edu/abs/2007GReGr..39.1419R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2007PhLA..370...99R,
@ARTICLE{rosaletelier2007PhLA,
   author = {{Rosa}, V. M. and {Letelier}, P. S.},
    title = "{Stability of closed timelike geodesics}",
  journal = {Physics Letters A},
   eprint = {gr-qc/0703148},
 keywords = {Spacetime topology causal structure spinor structure, Exact solutions},
     year = 2007,
    month = oct,
   volume = 370,
    pages = {99-103},
      doi = {10.1016/j.physleta.2007.05.041},
   adsurl = {http://adsabs.harvard.edu/abs/2007PhLA..370...99R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Saa A et al.  ======
%% ============================================================	

% 1999PhLA..259..201S,
@ARTICLE{saaVenegeroles1999PhLA,
   author = {{Saa}, A. and {Venegeroles}, R.},
    title = "{Chaos around the superposition of a black-hole and a thin disk}",
  journal = {Physics Letters A},
   eprint = {gr-qc/9906028},
     year = 1999,
    month = aug,
   volume = 259,
    pages = {201-206},
      doi = {10.1016/S0375-9601(99)00447-8},
   adsurl = {http://adsabs.harvard.edu/abs/1999PhLA..259..201S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Sanders J et al.  ======
%% ============================================================

% 2012MNRAS.426..128S,
@ARTICLE{sanders2012MNRAS,
   author = {{Sanders}, J.},
    title = "{Angle-action estimation in a general axisymmetric potential}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1208.2813},
 keywords = {methods: numerical, Galaxy: kinematics and dynamics, solar neighbourhood, Galaxy: structure, galaxies: kinematics and dynamics },
     year = 2012,
    month = oct,
   volume = 426,
    pages = {128-139},
      doi = {10.1111/j.1365-2966.2012.21698.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.426..128S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2014MNRAS.441.3284S,
@ARTICLE{sandersBinney2014MNRAS,
   author = {{Sanders}, J. L. and {Binney}, J.},
    title = "{Actions, angles and frequencies for numerically integrated orbits}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1401.3600},
 keywords = {methods: numerical, Galaxy: kinematics and dynamics, galaxies: kinematics and dynamics},
     year = 2014,
    month = jul,
   volume = 441,
    pages = {3284-3295},
      doi = {10.1093/mnras/stu796},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.441.3284S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Sanders RH et al.  ======
%% ============================================================

% 2002ARA&A..40..263S,
@ARTICLE{sandersMcgaughARAA2002,
   author = {{Sanders}, R. H. and {McGaugh}, S. S.},
    title = "{Modified Newtonian Dynamics as an Alternative to Dark Matter}",
  journal = {\araa},
   eprint = {astro-ph/0204521},
 keywords = {dark matter, galaxy dynamics, gravitational theory, cosmology},
     year = 2002,
   volume = 40,
    pages = {263-317},
      doi = {10.1146/annurev.astro.40.060401.093923},
   adsurl = {http://adsabs.harvard.edu/abs/2002ARA\%26A..40..263S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== SemerÃ¡k O et al.  ======
%% ============================================================	

% 1999MNRAS.308..691S,
@ARTICLE{semerakZellerinZacek1999MNRAS,
   author = {{Semer{\'a}k}, O. and {Zellerin}, T. and {{\v Z}{\'a}{\v c}ek}, M.
	},
    title = "{The structure of superposed Weyl fields}",
  journal = {\mnras},
     year = 1999,
    month = sep,
   volume = 308,
    pages = {691-704},
      doi = {10.1046/j.1365-8711.1999.02748.x},
   adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.308..691S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1999MNRAS.308..705S,
@ARTICLE{semerakZacekZellerin1999MNRAS,
   author = {{Semer{\'a}k}, O. and {{\v Z}{\'a}{\v c}ek}, M. and {Zellerin}, T.
	},
    title = "{Test-particle motion in superposed Weyl fields}",
  journal = {\mnras},
     year = 1999,
    month = sep,
   volume = 308,
    pages = {705-717},
      doi = {10.1046/j.1365-8711.1999.02749.x},
   adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.308..705S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2000PASJ...52.1067S,
@ARTICLE{semerakZacek2000PASJ,
   author = {{Semer{\'a}k}, O. and {{\v Z}{\'a}{\v c}ek}, M.},
    title = "{Oscillations of Static Discs around Schwarzschild Black Holes: Effect of Self-Gravitation}",
  journal = {\pasj},
 keywords = {ACCRETION DISCS, BLACK-HOLE PHYSICS, RELATIVITY},
     year = 2000,
    month = dec,
   volume = 52,
    pages = {1067-},
      doi = {10.1093/pasj/52.6.1067},
   adsurl = {http://adsabs.harvard.edu/abs/2000PASJ...52.1067S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2000CQGra..17.1613S,
@ARTICLE{semerakZacek2000CQGra,
   author = {{Semer{\'a}k}, O. and {Z{\'a}{\v c}ek}, M.},
    title = "{Gravitating discs around a Schwarzschild black hole: I}",
  journal = {Classical and Quantum Gravity},
     year = 2000,
    month = apr,
   volume = 17,
    pages = {1613-1626},
      doi = {10.1088/0264-9381/17/7/303},
   adsurl = {http://adsabs.harvard.edu/abs/2000CQGra..17.1613S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2002gfpi.conf..111S,
@INPROCEEDINGS{semerak2002review,
   author = {{Semer{\'a}k}, O.},
    title = "{Towards gravitating discs around stationary black holes}",
booktitle = {Gravitation: Following the Prague Inspiration},
     year = 2002,
   eprint = {gr-qc/0204025},
   editor = {{Semer{\'a}k}, O. and {Podolsk{\'y}}, J. and {Zofka}, M.},
    pages = {111},
   adsurl = {http://adsabs.harvard.edu/abs/2002gfpi.conf..111S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2010MNRAS.404..545S,
@ARTICLE{semerakSukova2010MNRAS,
   author = {{Semer{\'a}k}, O. and {Sukov{\'a}}, P.},
    title = "{Free motion around black holes with discs or rings: between integrability and chaos - I}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1211.4106},
 primaryClass = "gr-qc",
 keywords = {black hole physics, gravitation, relativity},
     year = 2010,
    month = may,
   volume = 404,
    pages = {545-574},
      doi = {10.1111/j.1365-2966.2009.16003.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.404..545S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2012MNRAS.425.2455S,
@ARTICLE{semerakSukova2012MNRAS,
   author = {{Semer{\'a}k}, O. and {Sukov{\'a}}, P.},
    title = "{Free motion around black holes with discs or rings: between integrability and chaos - II}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1211.4107},
 primaryClass = "gr-qc",
 keywords = {black hole physics, chaos, gravitation},
     year = 2012,
    month = oct,
   volume = 425,
    pages = {2455-2476},
      doi = {10.1111/j.1365-2966.2012.21630.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.425.2455S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Sgro et al.  ======
%% ============================================================	

@article{doi:10.1093/mnras/stt773,
author = {Sgr\'{o}, Mario A. and Paz, Dante J. and Merch\'{a}n, Manuel},
title = {Anisotropic halo model: implementation and numerical results},
journal = {Monthly Notices of the Royal Astronomical Society},
volume = {433},
number = {1},
pages = {787},
year = {2013},
doi = {10.1093/mnras/stt773},
%URL = { + http://dx.doi.org/10.1093/mnras/stt773},
%eprint = {/oup/backfile/content_public/journal/mnras/433/1/10.1093/mnras/stt773/3/stt773.pdf}
}



%% ============================================================
%% ====== Shrama et al.  ======
%% ============================================================	

@Article{Sharma2012,
author="Sharma, Ranjan
and Tikekar, Ramesh",
title="Space--time inhomogeneity, anisotropy and gravitational collapse",
journal="General Relativity and Gravitation",
year="2012",
month="Oct",
day="01",
volume="44",
number="10",
pages="2503--2520",
abstract="We investigate the evolution of non-adiabatic collapse of a shear-free spherically symmetric stellar configuration with anisotropic stresses accompanied with radial heat flux. The collapse begins from a curvature singularity with infinite mass and size on an inhomogeneous space--time background. The collapse is found to proceed without formation of an even horizon to singularity when the collapsing configuration radiates all its mass energy. The impact of inhomogeneity on various parameters of the collapsing stellar configuration is examined in some specific space--time backgrounds.",
%issn="1572-9532",
%doi="10.1007/s10714-012-1406-8",
%url="http://dx.doi.org/10.1007/s10714-012-1406-8"
}




%% ============================================================
%% ====== Shirokov MF et al.  ======
%% ============================================================	

% 1973GReGr...4..131S,
@ARTICLE{shirokov1973GRG,
   author = {{Shirokov}, M.F.},
    title = "{On one new effect of the Einsteinian theory of gravitation}",
  journal = {General Relativity and Gravitation},
     year = 1973,
    month = mar,
   volume = 4,
    pages = {131-136},
      doi = {10.1007/BF00762799},
   adsurl = {http://adsabs.harvard.edu/abs/1973GReGr...4..131S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Sing et al  ======
%% ============================================================


@ARTICLE{1992IJTP...31..545S,
   author = {{Singh}, T. and {Singh}, G. P. and {Srivastava}, R. S.},
    title = "{Static anisotropic fluid spheres in general relativity with nonuniform density}",
  journal = {International Journal of Theoretical Physics},
     year = 1992,
    month = mar,
   volume = 31,
    pages = {545-551},
      doi = {10.1007/BF00740004},
   adsurl = {http://adsabs.harvard.edu/abs/1992IJTP...31..545S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%% ============================================================
%% ====== Sofue Y et al.  ======
%% ============================================================

% 2001ARA&A..39..137S,
@ARTICLE{sofueRubin2001ARAA,
   author = {{Sofue}, Y. and {Rubin}, V.},
    title = "{Rotation Curves of Spiral Galaxies}",
  journal = {\araa},
   eprint = {astro-ph/0010594},
     year = 2001,
   volume = 39,
    pages = {137-174},
      doi = {10.1146/annurev.astro.39.1.137},
   adsurl = {http://adsabs.harvard.edu/abs/2001ARA%26A..39..137S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1999ApJ...523..136S,
@ARTICLE{sofueEtal1999ApJ,
   author = {{Sofue}, Y. and {Tutui}, Y. and {Honma}, M. and {Tomita}, A. and
	{Takamiya}, T. and {Koda}, J. and {Takeda}, Y.},
    title = "{Central Rotation Curves of Spiral Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/9905056},
 keywords = {GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: NUCLEI, GALAXIES: SPIRAL, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Galaxies: Spiral},
     year = 1999,
    month = sep,
   volume = 523,
    pages = {136-146},
      doi = {10.1086/307731},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...523..136S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2009PASJ...61..227S,
@ARTICLE{sofueHonmaOmodaka2009PASJ,
   author = {{Sofue}, Y. and {Honma}, M. and {Omodaka}, T.},
    title = "{Unified Rotation Curve of the Galaxy -- Decomposition into de Vaucouleurs Bulge, Disk, Dark Halo, and the 9-kpc Rotation Dip --}",
  journal = {\pasj},
archivePrefix = "arXiv",
   eprint = {	},
 keywords = {Galaxy: bulge, Galaxy: disk, Galaxy: rotation curve, Galaxy: structure},
     year = 2009,
    month = feb,
   volume = 61,
    pages = {227-},
      doi = {10.1093/pasj/61.2.227},
   adsurl = {http://adsabs.harvard.edu/abs/2009PASJ...61..227S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Sotomayor J et al.  ======
%% ============================================================

%
@book{sotomayor1979li,
  title={Li\c{c}\~oes de equa\c{c}\~oes diferenciais ordin{\'a}rias},
  author={Sotomayor, Jorge},
  volume={11},
  year={1979},
  publisher={Instituto de Matem{\'a}tica Pura e Aplicada, CNPq}
}

%% ============================================================
%% ====== Stephani H et al.  ======
%% ============================================================

%
@book{stephani2003exact,
  title={Exact solutions of Einstein's field equations},
  author={Stephani, Hans and Kramer, Dietrich and MacCallum, Malcolm and Hoenselaers, Cornelius and Herlt, Eduard},
  year={2003},
  publisher={Cambridge University Press}
}

%% ============================================================
%% ====== Steinmetz M et al.  ======
%% ============================================================

% 2012AN....333..523S,
@ARTICLE{steinmetz2012AN,
   author = {{Steinmetz}, M.},
    title = "{The Galactic thin and thick disk}",
  journal = {Astronomische Nachrichten},
archivePrefix = "arXiv",
   eprint = {1205.6098},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: abundances, Galaxy: evolution, Galaxy: formation, Galaxy: kinematics and dynamics, Galaxy: stellar content, Galaxy: structure, surveys},
     year = 2012,
    month = jun,
   volume = 333,
    pages = {523},
      doi = {10.1002/asna.201211698},
   adsurl = {http://adsabs.harvard.edu/abs/2012AN....333..523S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Stuchlik Z et al.  ======
%% ============================================================

%
@ARTICLE{stuchlikHedlik2002AcPSl,
   author = {{Stuchl{\'i}k}, Z. and {Hled{\'i}k}, S.},
    title = "{Properties of the Reissner-Nordstr{\"o}m spacetimes with a nonzero cosmological constant}",
  journal = {Acta Physica Slovaca},
     year = 2002,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1311.5820V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== SukovÃ¡ P et al.  ======
%% ============================================================

% 2013MNRAS.436..978S,
@ARTICLE{sukovaSemerak2013MNRAS,
   author = {{Sukov{\'a}}, P. and {Semer{\'a}k}, O.},
    title = "{Free motion around black holes with discs or rings: between integrability and chaos - III}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1308.4306},
 primaryClass = "gr-qc",
 keywords = {black hole physics, chaos, gravitation, Galaxy: centre},
     year = 2013,
    month = dec,
   volume = 436,
    pages = {978-996},
      doi = {10.1093/mnras/stt1587},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.436..978S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Tabor M et al.  ======
%% ============================================================

%
@book{tabor1989chaos,
  title={Chaos and integrability in nonlinear dynamics},
  author={Tabor, Michael},
  year={1989},
  publisher={Wiley}
}

%% ============================================================
%% ====== Taub AH et al.  ======
%% ============================================================

% 1980JMP....21.1423T,
@ARTICLE{taub1980JMP,
   author = {{Taub}, A. H.},
    title = "{Space-times with distribution valued curvature tensors.}",
  journal = {Journal of Mathematical Physics},
 keywords = {Relativity:Space-Time},
     year = 1980,
   volume = 21,
    pages = {1423-1431},
      doi = {10.1063/1.524568},
   adsurl = {http://adsabs.harvard.edu/abs/1980JMP....21.1423T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Ujevic M et al.  ======
%% ============================================================

% 2004PhRvD..70h4015U,
@ARTICLE{ujevicLetelier2004PRD,
   author = {{Ujevic}, M. and {Letelier}, P. S.},
    title = "{Stability of general relativistic geometric thin disks}",
  journal = {\prd},
   eprint = {gr-qc/0409110},
 keywords = {Relativistic stars: structure stability and oscillations, Exact solutions, Spiral arms and bars, galactic disks},
     year = 2004,
    month = oct,
   volume = 70,
   number = 8,
      eid = {084015},
    pages = {084015},
      doi = {10.1103/PhysRevD.70.084015},
   adsurl = {http://adsabs.harvard.edu/abs/2004PhRvD..70h4015U},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== van der Kruit PC et al.  ======
%% ============================================================

% 1988A&A...192..117V,
@ARTICLE{vanderkruit1988AA,
   author = {{van der Kruit}, P. C.},
    title = "{The three-dimensional distribution of light and mass in disks of spiral galaxies}",
  journal = {\aap},
 keywords = {Gas Dynamics, Mass To Light Ratios, Spiral Galaxies, Star Distribution, Astronomical Models, Density Distribution, Mass Distribution, Radial Velocity, Velocity Distribution, Vertical Distribution},
     year = 1988,
    month = mar,
   volume = 192,
    pages = {117-127},
   adsurl = {http://adsabs.harvard.edu/abs/1988A\%26A...192..117V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2011ARA&A..49..301V,
@ARTICLE{vanderkruitFreeman2011ARAA,
   author = {{van der Kruit}, P. C. and {Freeman}, K. C.},
    title = "{Galaxy Disks}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1101.1771},
 primaryClass = "astro-ph.GA",
     year = 2011,
    month = sep,
   volume = 49,
    pages = {301-371},
      doi = {10.1146/annurev-astro-083109-153241},
   adsurl = {http://adsabs.harvard.edu/abs/2011ARA\%26A..49..301V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Veltz L et al.  ======
%% ============================================================

% 2008A&A...480..753V,
@ARTICLE{veltzEtal2008AA,
   author = {{Veltz}, L. and {Bienaym{\'e}}, O. and {Freeman}, K. C. and
	{Binney}, J. and {Bland-Hawthorn}, J. and {Gibson}, B. K. and
	{Gilmore}, G. and {Grebel}, E. K. and {Helmi}, A. and {Munari}, U. and
	{Navarro}, J. F. and {Parker}, Q. A. and {Seabroke}, G. M. and
	{Siebert}, A. and {Steinmetz}, M. and {Watson}, F. G. and {Williams}, M. and
	{Wyse}, R. F. G. and {Zwitter}, T.},
    title = "{Galactic kinematics with RAVE data. I. The distribution of stars towards the Galactic poles}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0801.2120},
 keywords = {stars: kinematics, Galaxy: disk, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2008,
    month = mar,
   volume = 480,
    pages = {753-765},
      doi = {10.1051/0004-6361:20066948},
   adsurl = {http://adsabs.harvard.edu/abs/2008A\%26A...480..753V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Vieira RSS et al.  ======
%% ============================================================

% 2014GReGr..46.1641V,
@ARTICLE{vieiraLetelier2014GRG,
   author = {{Vieira}, R. S. S. and {Letelier}, P. S.},
    title = "{Thin-disk models in an integrable Weyl-Dirac theory}",
  journal = {General Relativity and Gravitation},
archivePrefix = "arXiv",
   eprint = {1305.2662},
 primaryClass = "gr-qc",
 keywords = {Weyl-Dirac theory, Exact solutions, Galaxy astrophysics, Modified gravity},
     year = 2014,
    month = jan,
   volume = 46,
    pages = {1641},
      doi = {10.1007/s10714-013-1641-7},
   adsurl = {http://adsabs.harvard.edu/abs/2014GReGr..46.1641V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2014ApJ...786...27V,
@ARTICLE{vieiraRamoscaro2014ApJ,
   author = {{Vieira}, R. S. S. and {Ramos-Caro}, J.},
    title = "{A Simple Formula for the Third Integral of Motion of Disk-crossing Stars in the Galaxy}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1305.7078},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: spiral, Galaxy: disk, Galaxy: kinematics and dynamics },
     year = 2014,
    month = may,
   volume = 786,
      eid = {27},
    pages = {27},
      doi = {10.1088/0004-637X/786/1/27},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...786...27V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2014PhRvD..90b4035V,
@ARTICLE{vieiraMarekEtal2014PRD,
   author = {{Vieira}, R. S. S. and {Schee}, J. and {Klu{\'z}niak}, W. and
	{Stuchl{\'{\i}}k}, Z. and {Abramowicz}, M.},
    title = "{Circular geodesics of naked singularities in the Kehagias-Sfetsos metric of Ho{\v r}ava's gravity}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1311.5820},
 primaryClass = "gr-qc",
 keywords = {Modified theories of gravity, Classical black holes, Relativistic stars: structure stability and oscillations, Orbit determination and improvement},
     year = 2014,
    month = jul,
   volume = 90,
   number = 2,
      eid = {024035},
    pages = {024035},
      doi = {10.1103/PhysRevD.90.024035},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..90b4035V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% 2016CeMDA.tmp...40V
@ARTICLE{vieiraRamoscaro2016CeMDA,
   author = {{Vieira}, R. S. S. and {Ramos-Caro}, J.},
    title = "{Integrability of motion around galactic razor-thin disks}",
  journal = {Celestial Mechanics and Dynamical Astronomy},
archivePrefix = "arXiv",
   eprint = {1606.06349},
 keywords = {Dynamics of galaxies, Razor-thin disks, Disk-crossing orbits, Vertical stability, Third integral, Adiabatic approximation},
     year = 2016,
    month = jun,
     note = {(published online, doi:10.1007/s10569-016-9705-0)},
      doi = {10.1007/s10569-016-9705-0},
   adsurl = {http://adsabs.harvard.edu/abs/2016CeMDA.tmp...40V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% doi:10.1142/9789814623995_0438
@inproceedings{vieiraRamoscaro2015MG13,
author = {{Vieira}, R. S. S. and {Ramos-Caro}, J.},
title = {On the Stability of Circular Orbits in Galactic Dynamics: Newtonian Thin Disks},
booktitle = {The Thirteenth Marcel Grossmann Meeting},
editor = {Kjell Rosquist and Robert T. Jantzen and Remo Ruffini},
chapter = {438},
pages = {2346-2348},
year={2015},
publisher= {World Scientific},
doi = {10.1142/9789814623995_0438}
}



% 1PN razor thin disks
@article{PhysRevD.86.043008,
  title = {Kinetic theory of collisionless self-gravitating gases. II. Relativistic corrections in galactic dynamics},
  author = {Ramos-Caro, J. and Ag\'on, C. A. and Pedraza, J. F.},
  journal = {Phys. Rev. D},
  volume = {86},
  issue = {4},
  pages = {043008},
  numpages = {15},
  year = {2012},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.86.043008},
  adsurl = {http://link.aps.org/doi/10.1103/PhysRevD.86.043008}
}


%% ============================================================
%% ====== Vogt D et al.  ======
%% ============================================================

% 2003PhRvD..68h4010V,
@ARTICLE{vogtLetelier2003PRD,
   author = {{Vogt}, D. and {Letelier}, P. S.},
    title = "{Exact general relativistic perfect fluid disks with halos}",
  journal = {\prd},
   eprint = {gr-qc/0308031},
 keywords = {Exact solutions, Self-gravitating systems, continuous media and classical fields in curved spacetime, Accretion and accretion disks},
     year = 2003,
    month = oct,
   volume = 68,
   number = 8,
      eid = {084010},
    pages = {084010},
      doi = {10.1103/PhysRevD.68.084010},
   adsurl = {http://adsabs.harvard.edu/abs/2003PhRvD..68h4010V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2005MNRAS.363..268V,
@ARTICLE{vogtLetelier2005MNRAS,
   author = {{Vogt}, D. and {Letelier}, P. S.},
    title = "{Relativistic models of galaxies}",
  journal = {\mnras},
   eprint = {astro-ph/0507406},
 keywords = {relativity, stellar dynamics, celestial mechanics, galaxies: kinematics and dynamics},
     year = 2005,
    month = oct,
   volume = 363,
    pages = {268-284},
      doi = {10.1111/j.1365-2966.2005.09436.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.363..268V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2009MNRAS.396.1487V,
@ARTICLE{vogtLetelier2009MNRAS,
   author = {{Vogt}, D. and {Letelier}, P. S.},
    title = "{Analytical potential-density pairs for flat rings and toroidal structures}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0906.0919},
 primaryClass = "astro-ph.GA",
 keywords = {planets: rings , galaxies: kinematics and dynamics},
     year = 2009,
    month = jul,
   volume = 396,
    pages = {1487-1498},
      doi = {10.1111/j.1365-2966.2009.14803.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.396.1487V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{doi:10.1111/j.1365-2966.2009.15967.x,
author = {Vogt, D. and Letelier, P. S.},
title = {Newtonian and General Relativistic models of spherical shells},
journal = {Monthly Notices of the Royal Astronomical Society},
volume = {402},
number = {2},
pages = {1313},
year = {2010},
doi = {10.1111/j.1365-2966.2009.15967.x},
%URL = { + http://dx.doi.org/10.1111/j.1365-2966.2009.15967.x},
%eprint = {/oup/backfile/content_public/journal/mnras/402/2/10.1111/j.1365-2966.2009.15967.x/2/mnras0402-1313.pdf}
}

@article{doi:10.1111/j.1365-2966.2010.16863.x,
author = {Vogt, D. and Letelier, P. S.},
title = {Newtonian and General Relativistic models of spherical shells â II},
journal = {Monthly Notices of the Royal Astronomical Society},
volume = {406},
number = {4},
pages = {2689},
year = {2010},
doi = {10.1111/j.1365-2966.2010.16863.x},
%URL = { + http://dx.doi.org/10.1111/j.1365-2966.2010.16863.x},
%eprint = {/oup/backfile/content_public/journal/mnras/406/4/10.1111/j.1365-2966.2010.16863.x/2/mnras0406-2689.pdf}
}


%
@phdthesis{vogtthesis,
  author={Vogt, Daniel},
  title={Modelos de discos e outras estruturas auto-gravitantes em relatividade geral},
  school={Universidade Estadual de Campinas, Instituto de Fisica Gleb Wataghin},
  year={2006}
}



%% ============================================================
%% ====== Voorhees BH et al.  ======
%% ============================================================

% 1972PhRvD...5.2413V,
@ARTICLE{voorhees1972PRD,
   author = {{Voorhees}, B. H.},
    title = "{Relativistic Disks. I. Background Models}",
  journal = {\prd},
     year = 1972,
    month = may,
   volume = 5,
    pages = {2413-2418},
      doi = {10.1103/PhysRevD.5.2413},
   adsurl = {http://adsabs.harvard.edu/abs/1972PhRvD...5.2413V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Wald R et al.  ======
%% ============================================================

%
@book{waldGR,	
  author = {R. Wald},
  title  = {General Relativity},
  publisher = {The University of Chicago Press},
  year = {1984},
  address = {Chicago, IL}	
}

%% ============================================================
%% ====== Witzany V et al.  ======
%% ============================================================

% 2015MNRAS.451.1770W
@ARTICLE{witzanySemerakSukova2015MNRAS,
   author = {{Witzany}, V. and {Semer{\'a}k}, O. and {Sukov{\'a}}, P.},
    title = "{Free motion around black holes with discs or rings: between integrability and chaos - IV}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1503.09077},
 primaryClass = "astro-ph.HE",
 keywords = {black hole physics, chaos, gravitation},
     year = 2015,
    month = aug,
   volume = 451,
    pages = {1770-1794},
      doi = {10.1093/mnras/stv1148},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.451.1770W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Zacek M et al.  ======
%% ============================================================

% 2002CzJPh..52...19Z,
@ARTICLE{zacekSemerak2002CzJP,
   author = {{{\v Z}{\'a}{\v c}ek}, M. and {Semer{\'a}k}, O.},
    title = "{Gravitating Discs Around a Schwarzschild Black Hole II}",
  journal = {Czechoslovak Journal of Physics},
 keywords = {general relativity - black holes - exact solutions of Einstein equations},
     year = 2002,
    month = jan,
   volume = 52,
    pages = {19-27},
      doi = {10.1023/A:1013957512339},
   adsurl = {http://adsabs.harvard.edu/abs/2002CzJPh..52...19Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



%% ============================================================
%% ====== Zharnitsky V et al.  ======
%% ============================================================

% 2000CMaPh.211..289Z,
@ARTICLE{zharnitsky2000CMaPh,
   author = {{Zharnitsky}, V.},
    title = "{Invariant Tori in Hamiltonian Systems with Impacts}",
  journal = {Communications in Mathematical Physics},
     year = 2000,
   volume = 211,
    pages = {289-302},
      doi = {10.1007/s002200050813},
   adsurl = {http://adsabs.harvard.edu/abs/2000CMaPh.211..289Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{Nguyen,
  author    = {Nguyen, Phuc H. and Lingam, Manasvi},
  title     = {Analytical families of two-component anisotropic polytropes and their relativistic extensions},
  journal   = {Monthly Notices of the Royal Astronomical Society},
  year      = {2013},
  volume    = {436},
  number    = {3},
  pages     = {2014},
  month     = {oct},
  doi       = {10.1093/mnras/stt1719},
  keywords  = {rank5},
  publisher = {Oxford University Press ({OUP})},
  %url       = {http://dx.doi.org/10.1093/mnras/stt1719},
}

@Book{poissontoolkit,
  title     = {A Relativist's Toolkit},
  publisher = {Cambridge University Press},
  year      = {2007},
  author    = {Eric Poisson},
  date      = {2007-11-05},
  ean       = {9780521537803},
  isbn      = {0521537800},
  pagetotal = {252},
}

@Book{Weinberg,
  title     = {Gravitation and Cosmology},
  publisher = {John Wiley and Sons Ltd},
  year      = {1972},
  author    = {Steven Weinberg},
  date      = {1972-01-01},
  ean       = {9780471925675},
  pagetotal = {688},
   % isbn      = {0471925675},

   @Book{Kremer,
  title     = {The Relativistic Boltzmann Equation: Theory and Applications},
  publisher = {Birkhäuser Basel},
  year      = {2002},
  author    = {Carlo Cercignani and Gilberto M. Kremer},
  date      = {2002-01-01},
  ean       = {},
  pagetotal = {384},
   % isbn      = {978-3-7643-6693-3},
}
@article{Fackerell_1968,
	doi = {10.1086/149693},
	year = 1968,
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {153},
	pages = {643},
	author = {Edward D. Fackerell},
	title = {Relativistic Stellar Dynamics},
	journal = {The Astrophysical Journal}
	%url = {https://doi.org/10.1086%2F149693},
}

@Book{Polyanin,
  title     = {Handbook of Integral Equations},
  publisher = {Chapman and Hall/CRC},
  year      = {2008},
  author    = {Andrei D. Polyanin and Alexander V. Manzhirov},
  edition   = {Second Edition},
  keywords  = {rank5},
}

@Book{Straumann,
  title     = {General Relativity},
  publisher = {Springer Netherlands},
  year      = {2013},
  author    = {Norbert Straumann},
  edition   = {Second Edition},
}

@Comment{jabref-meta: databaseType:bibtex;}


==> stabgr_refs.tex <==
% Encoding: UTF-8




%% Organizado pelo nome do primeiro autor e ano

%% ============================================================
%% ====== Abramowicz MA et al. ======
%% ============================================================

% 1990MNRAS.245..733A,
@ARTICLE{abramowicz1990MNRAS,
   author = {{Abramowicz}, M. A.},
    title = "{Centrifugal Force - a Few Surprises}",
  journal = {\mnras},
     year = 1990,
    month = aug,
   volume = 245,
    pages = {733},
   adsurl = {http://adsabs.harvard.edu/abs/1990MNRAS.245..733A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% Abramowicz & Fragile 2013, LRR, Foundations of Black Hole Accretion Disk Theory
% %%2013LRR....16....1A,
@ARTICLE{abramowiczFragileLRR,
   author = {{Abramowicz}, M.A. and {Fragile}, P.C.},
    title = "{Foundations of Black Hole Accretion Disk Theory}",
  journal = {Living Reviews in Relativity},
archivePrefix = "arXiv",
   eprint = {1104.5499},
 primaryClass = "astro-ph.HE",
 keywords = {black hole accretion disks},
     year = 2013,
    month = jan,
   volume = 16,
    pages = {1},
      doi = {10.12942/lrr-2013-1},
   adsurl = {http://adsabs.harvard.edu/abs/2013LRR....16....1A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% Abramowicz & Kluzniak 2005, Ap\&SS, Epicyclic Frequencies Derived From The Effective Potential: Simple And Practical Formulae
%%2005Ap&SS.300..127A,
@ARTICLE{abramowiczKluzniak2005ApSS,
   author = {{Abramowicz}, M.A. and {Klu{\'z}niak}, W.},
    title = "{Epicyclic Frequencies Derived From The Effective Potential: Simple And Practical Formulae}",
  journal = {\apss},
   eprint = {astro-ph/0411709},
 keywords = {black holes, neutron stars, orbital motion, epicyclic frequencies},
     year = 2005,
    month = nov,
   volume = 300,
    pages = {127-136},
      doi = {10.1007/s10509-005-1173-z},
   adsurl = {http://adsabs.harvard.edu/abs/2005Ap\%26SS.300..127A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Allen C et al. ======
%% ============================================================

% 1991RMxAA..22..255A,
@ARTICLE{allenSantillan1991RMxAA,
   author = {{Allen}, C. and {Santillan}, A.},
    title = "{An improved model of the galactic mass distribution for orbit computations}",
  journal = {\rmxaa},
 keywords = {Astronomical Models, Galactic Mass, Mass Distribution, Milky Way Galaxy, Stellar Motions, Dynamic Models, Galactic Rotation, Galactic Structure, Mathematical Models},
     year = 1991,
    month = oct,
   volume = 22,
    pages = {255-263},
   adsurl = {http://adsabs.harvard.edu/abs/1991RMxAA..22..255A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Ansorg M et al. ======
%% ============================================================

%
%%1998JMP....39.5984A,
@ARTICLE{ansorg1998JMP,
   author = {{Ansorg}, M.},
    title = "{Timelike geodesic motions within the general relativistic gravitational field of the rigidly rotating disk of dust}",
  journal = {Journal of Mathematical Physics},
 keywords = {Exact solutions, Einstein-Maxwell spacetimes spacetimes with fluids radiation or classical fields},
     year = 1998,
    month = nov,
   volume = 39,
    pages = {5984-6000},
      doi = {10.1063/1.532609},
   adsurl = {http://adsabs.harvard.edu/abs/1998JMP....39.5984A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Arnold VI et al. ======
%% ============================================================

%
@book{arnoldMmcm,
  author = {V. I. Arnol'd}, edition = {Second},
  title  = {Mathematical Methods of Classical Mechanics},
  publisher = {Springer-Verlag},
  year = {1989}, series = {Graduate Texts in Mathematics},  volume = 60,
  address = {New York, NY}	
}



%\bibitem[\protect\citeauthoryear{Arnold}{1978}]{arnold}
%Arnold V. I., 1978, Mathematical Methods of Classical
%Mechanics. Springer-Verlag, New York, NY

%% ============================================================
%% ====== Bardeen JM et al. ======
%% ============================================================


%%1970ApJ...161..103B,
@ARTICLE{bardeen1970ApJ,
   author = {{Bardeen}, J. M.},
    title = "{Stability of Circular Orbits in Stationary, Axisymmetric Space-Times}",
  journal = {\apj},
     year = 1970,
    month = jul,
   volume = 161,
    pages = {103},
      doi = {10.1086/150515},
   adsurl = {http://adsabs.harvard.edu/abs/1970ApJ...161..103B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== BarrabÃ¨s C et al. ======
%% ============================================================

%1989CQGra...6..581B,
@ARTICLE{barrabes1989CQGra,
   author = {{Barrab{\`e}s}, C.},
    title = "{Singular hypersurfaces in general relativity - A unified description}",
  journal = {Classical and Quantum Gravity},
 keywords = {Cosmology, Hyperspaces, Relativity, Shock Waves, Einstein Equations, Stress Tensors},
     year = 1989,
    month = may,
   volume = 6,
    pages = {581-588},
      doi = {10.1088/0264-9381/6/5/003},
   adsurl = {http://adsabs.harvard.edu/abs/1989CQGra...6..581B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Batsleer P et al. ======
%% ============================================================

% 1994A&A...287...43B,
@ARTICLE{batsleerDejonghe1994AA,
   author = {{Batsleer}, P. and {Dejonghe}, H.},
    title = "{The generation of Stackel potentials for galactic dynamical modeling}",
  journal = {\aap},
 keywords = {Astronomical Models, Dynamic Models, Galactic Structure, Milky Way Galaxy, Potential, Rotation, Galactic Halos, Measure And Integration, Rotating Disks},
     year = 1994,
    month = jul,
   volume = 287,
    pages = {43-54},
   adsurl = {http://adsabs.harvard.edu/abs/1994A\%26A...287...43B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Bayin ======
%% ============================================================

@article{PhysRevD.26.1262,
  title = {Anisotropic fluid spheres in general relativity},
  author = {Bayin, S.S.},
  journal = {Phys. Rev. D},
  volume = {26},
  issue = {6},
  pages = {1262--1274},
  numpages = {0},
  year = {1982},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.26.1262},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.26.1262}
}



%% ============================================================
%% ====== Bekenstein J et al. ======
%% ============================================================

% 1984ApJ...286....7B,
@ARTICLE{bekensteinMilgrom1984ApJ,
   author = {{Bekenstein}, J. and {Milgrom}, M.},
    title = "{Does the missing mass problem signal the breakdown of Newtonian gravity?}",
  journal = {\apj},
 keywords = {Galactic Rotation, Gravitation Theory, Mass Distribution, Missing Mass (Astrophysics), Newton Theory, Nonrelativistic Mechanics, Potential Theory, Computational Astrophysics, Cosmology, Equivalence, Poisson Equation},
     year = 1984,
    month = nov,
   volume = 286,
    pages = {7-14},
      doi = {10.1086/162570},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...286....7B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Bershady MA et al. ======
%% ============================================================

% 2010ApJ...716..198B,
@ARTICLE{bershadyEtal2010ApJ1,
   author = {{Bershady}, M.A. and {Verheijen}, M. A. W. and {Swaters}, R. A. and
	{Andersen}, D. R. and {Westfall}, K. B. and {Martinsson}, T.
	},
    title = "{The DiskMass Survey. I. Overview}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1004.4816},
 primaryClass = "astro-ph.CO",
 keywords = {dark matter, galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: halos, galaxies: kinematics and dynamics, galaxies: spiral, galaxies: stellar content, galaxies: structure},
     year = 2010,
    month = jun,
   volume = 716,
    pages = {198-233},
      doi = {10.1088/0004-637X/716/1/198},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...716..198B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2010ApJ...716..234B,
@ARTICLE{bershadyEtal2010ApJ2,
   author = {{Bershady}, M. A. and {Verheijen}, M. A. W. and {Westfall}, K. B. and
	{Andersen}, D. R. and {Swaters}, R. A. and {Martinsson}, T.},
    title = "{The DiskMass Survey. II. Error Budget}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1004.5043},
 primaryClass = "astro-ph.CO",
 keywords = {dark matter, galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: halos, galaxies: kinematics and dynamics, galaxies: spiral, galaxies: stellar content, galaxies: structure, methods: data analysis, techniques: spectroscopic},
     year = 2010,
    month = jun,
   volume = 716,
    pages = {234-268},
      doi = {10.1088/0004-637X/716/1/234},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...716..234B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Bertin G et al. ======
%% ============================================================

%
@book{bertin2014dynamics,
  title={Dynamics of galaxies},
  author={Bertin, Giuseppe},
  year={2014},
  publisher={Cambridge University Press}
}

%% ============================================================
%% ====== Bertschinger E et al. ======
%% ============================================================

%
@misc{bertschinger,
  author={Bertschinger, E.},
  title={General relativity notes, chap. 3: Hamiltonian dynamics of particle motion},
  howpublished={Lecture notes (online resource)},
  note={http://web.mit.edu/edbert/GR/gr3.pdf},
  year={1999}
}

% \bibitem{bertschinger}
% Bertschinger, E., \textit{General relativity notes, cap.3: Hamiltonian dynamics of particle motion},
% http://web.mit.edu/edbert/GR/gr3.pdf


%% ============================================================
%% ====== Bi\v{c}\'ak J et al. (Bicak) ======
%% ============================================================

%1993PhRvD..47.4334B,
@ARTICLE{bicakLyndenbellKatz1993PRD,
   author = {{Bi{\v c}{\'a}k}, J. and {Lynden-Bell}, D. and {Katz}, J.},
    title = "{Relativistic disks as sources of static vacuum spacetimes}",
  journal = {\prd},
 keywords = {Exact solutions},
     year = 1993,
    month = may,
   volume = 47,
    pages = {4334-4343},
      doi = {10.1103/PhysRevD.47.4334},
   adsurl = {http://adsabs.harvard.edu/abs/1993PhRvD..47.4334B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}	

%% ============================================================
%% ====== Bienayme O et al. ======
%% ============================================================

% 2013A&A...549A..89B,
@ARTICLE{bienaymeTraven2013AA,
   author = {{Bienaym{\'e}}, O. and {Traven}, G.},
    title = "{Approximate integrals of motion}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1211.6306},
 primaryClass = "astro-ph.GA",
 keywords = {gravitation, methods: numerical, galaxies: kinematics and dynamics},
     year = 2013,
    month = jan,
   volume = 549,
      eid = {A89},
    pages = {A89},
      doi = {10.1051/0004-6361/201220008},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...549A..89B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2009A&A...500..801B,
@ARTICLE{bienaymeEtal2009AA,
   author = {{Bienaym{\'e}}, O. and {Famaey}, B. and {Wu}, X. and {Zhao}, H. S. and
	{Aubert}, D.},
    title = "{Galactic kinematics with modified Newtonian dynamics}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0904.3893},
 primaryClass = "astro-ph.GA",
 keywords = {gravitation, stars: kinematics, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2009,
    month = jun,
   volume = 500,
    pages = {801-805},
      doi = {10.1051/0004-6361/200809978},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...500..801B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Binney J et al.  ======
%% ============================================================



%series = {Graduate Texts in Mathematics},  volume = 60,
@book{binneytremaineGD,
  author = {{Binney}, J. and {Tremaine}, S.}, edition = {Second},
  title  = {Galactic Dynamics},
  publisher = {Princeton Univ. Press},
  year = {2008},
  address = {Princeton, NJ}	
}

% 2010MNRAS.401.2318B,
@ARTICLE{binney2010MNRAS,
   author = {{Binney}, J.},
    title = "{Distribution functions for the Milky Way}",
  journal = {\mnras},
archivePrefix = "arXiv",
 primaryClass = "astro-ph.GA",
 keywords = {solar neighbourhood, Galaxy: disc, galaxies: kinematics and dynamics},
     year = 2010,
    month = feb,
   volume = 401,
    pages = {2318-2330},
      doi = {10.1111/j.1365-2966.2009.15845.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.401.2318B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
  %   eprint = {0910.1512},
}

% 2011MNRAS.413.1889B,
@ARTICLE{binneyMcmillan2011MNRAS,
   author = {{Binney}, J. and {McMillan}, P.},
    title = "{Models of our Galaxy - II}",
  journal = {\mnras},
archivePrefix = "arXiv",
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disc, Galaxy: kinematics and dynamics, Galaxy: structure, galaxies: kinematics and dynamics},
     year = 2011,
    month = may,
   volume = 413,
    pages = {1889-1898},
      doi = {10.1111/j.1365-2966.2011.18268.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.413.1889B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
    % eprint = {1101.0747},
}


% 2012MNRAS.426.1328B,
@ARTICLE{binney2012MNRAS,
   author = {{Binney}, J.},
    title = "{More dynamical models of our Galaxy}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1207.4917},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disc, solar neighbourhood, galaxies: kinematics and dynamics},
     year = 2012,
    month = oct,
   volume = 426,
    pages = {1328-1337},
      doi = {10.1111/j.1365-2966.2012.21692.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.426.1328B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2012MNRAS.426.1324B,
@ARTICLE{binney2012MNRASactions,
   author = {{Binney}, J.},
    title = "{Actions for axisymmetric potentials}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1207.4910},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: kinematics and dynamics, galaxies: kinematics and dynamics},
     year = 2012,
    month = oct,		
   volume = 426,
    pages = {1324-1327},
      doi = {10.1111/j.1365-2966.2012.21757.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.426.1324B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2014IAUS..298..117B,
@INPROCEEDINGS{binneySanders2014IAUS,
   author = {{Binney}, J. and {Sanders}, J. L.},
    title = "{Dynamical models and Galaxy surveys}",
 keywords = {stellar dynamics, surveys, stars: abundances, Galaxy: disk, Galaxy: kinematics and dynamics, Galaxy: stellar content},
booktitle = {IAU Symposium},
     year = 2014,
   series = {IAU Symposium},
   volume = 298,
archivePrefix = "arXiv",
   eprint = {1309.2790},
 primaryClass = "astro-ph.GA",
   editor = {{Feltzing}, S. and {Zhao}, G. and {Walton}, N. A. and {Whitelock}, P.
	},
    month = jan,
    pages = {117-129},
      doi = {10.1017/S1743921313006297},
   adsurl = {http://adsabs.harvard.edu/abs/2014IAUS..298..117B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Bocaletti D et al.  ======
%% ============================================================

% 1999thor.book.....B,
@BOOK{theoryoforbits2,
   author = {{Boccaletti}, D. and {Pucacco}, G.},
    title = "{Theory of Orbits Volume 2: Perturbative and Geometrical Methods}",
booktitle = {Volume 2: Perturbative and Geometrical Methods, XV, 423 pp. 81 figs..  Springer-Verlag Berlin Heidelberg New York.  Also Astronomy and Astrophysics Library, volume 2},
     year = 1999,
   adsurl = {http://adsabs.harvard.edu/abs/1999thor.book.....B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
  publisher = {Springer-Verlag},
  address = {Berlin}
}


%% ============================================================
%% ====== Bonnor WB et al.  ======
%% ============================================================


%1968CMaPh...8..338B,
@ARTICLE{bonnor1968CMaPh,
   author = {{Bonnor}, W. B. and {Sackfield}, A.},
    title = "{The interpretation of some spheroidal metrics}",
  journal = {Communications in Mathematical Physics},
     year = 1968,
    month = dec,
   volume = 8,
    pages = {338-344},
      doi = {10.1007/BF01646273},
   adsurl = {http://adsabs.harvard.edu/abs/1968CMaPh...8..338B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Bosma A et al.  ======
%% ============================================================

% 2002ASPC..273..223B,
@INPROCEEDINGS{bosma2002ASPconf,
   author = {{Bosma}, A.},
    title = "{HI and Dark Matter in Spiral Galaxies}",
booktitle = {The Dynamics, Structure {\amp} History of Galaxies: A Workshop in Honour of Professor Ken Freeman},
     year = 2002,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 273,
   eprint = {astro-ph/0112080},
   editor = {{Da Costa}, G. S. and {Sadler}, E. M. and {Jerjen}, H.},
    pages = {223},
   adsurl = {http://adsabs.harvard.edu/abs/2002ASPC..273..223B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%Buchdahl


@ARTICLE{1964ApJ...140.1512B,
   author = {{Buchdahl}, H. A.},
    title = "{A Relativistic Fluid Sphere Resembling the Emden Polytrope of Index 5.}",
  journal = {\apj},
     year = 1964,
    month = nov,
   volume = 140,
    pages = {1512},
      doi = {10.1086/148055},
   adsurl = {http://adsabs.harvard.edu/abs/1964ApJ...140.1512B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Bowers  ======
%% ============================================================

@ARTICLE{1974ApJ...188..657B,
   author = {{Bowers}, R. L. and {Liang}, E. P. T.},
    title = "{Anisotropic Spheres in General Relativity}",
  journal = {\apj},
     year = 1974,
    month = mar,
   volume = 188,
    pages = {657},
      doi = {10.1086/152760},
   adsurl = {http://adsabs.harvard.edu/abs/1974ApJ...188..657B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Buchdahl  ======
%% ============================================================


@ARTICLE{1964ApJ...140.1512B,
   author = {{Buchdahl}, H.~A.},
    title = "{A Relativistic Fluid Sphere Resembling the Emden Polytrope of Index 5.}",
  journal = {\apj},
     year = 1964,
    month = nov,
   volume = 140,
    pages = {1512},
      doi = {10.1086/148055},
   adsurl = {http://adsabs.harvard.edu/abs/1964ApJ...140.1512B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%% ============================================================
%% ====== Callen H et al.  ======
%% ============================================================

%
@book{callen1985thermodynamics,
  title={Thermodynamics and an Introduction to Thermostatistics},
  author={Callen, Herbert B},
  year={1985},
  publisher={John Wiley \& Sons},
  address={New York}
}

%% ============================================================
%% ====== Chudakova EM et al.  ======
%% ============================================================

% 2014ARep...58..281C,
@ARTICLE{chudakova2014ARep,
   author = {{Chudakova}, E. M. and {Sil'chenko}, O. K.},
    title = "{The thickness of stellar disks in early-type galaxies}",
  journal = {Astronomy Reports},
archivePrefix = "arXiv",
   eprint = {1410.6713},
     year = 2014,
    month = may,
   volume = 58,
    pages = {281-290},
      doi = {10.1134/S1063772914050023},
   adsurl = {http://adsabs.harvard.edu/abs/2014ARep...58..281C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Chicone C et al.  ======
%% ============================================================

% 2002CQGra..19.4231C,
@ARTICLE{chiconeMashoon2002CQGra,
   author = {{Chicone}, C. and {Mashhoon}, B.},
    title = "{The generalized Jacobi equation}",
  journal = {Classical and Quantum Gravity},
   eprint = {gr-qc/0203073},
     year = 2002,
    month = aug,
   volume = 19,
    pages = {4231-4248},
      doi = {10.1088/0264-9381/19/16/301},
   adsurl = {http://adsabs.harvard.edu/abs/2002CQGra..19.4231C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Coimbra-Araujo C et al.  ======
%% ============================================================

% PhysRevD.76.043522,
@article{coimbraLetelier2007PRD,
  title = {Thin disk in higher dimensional space-time and dark matter interpretation},
  author = {Coimbra-Ara\'ujo, Carlos H. and Letelier, Patricio S.},
  journal = {Phys. Rev. D},
  volume = {76},
  issue = {4},
  pages = {043522},
  numpages = {17},
  year = {2007},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.76.043522},
  adsurl = {http://link.aps.org/doi/10.1103/PhysRevD.76.043522}
}

%% ============================================================
%% ====== Coley  ======
%% ============================================================

@ARTICLE{1994CQGra..11.2553C,
   author = {{Coley}, A. A. and {Tupper}, B. O. J.},
    title = "{Spherically symmetric anisotropic fluid ICKV spacetimes}",
  journal = {Classical and Quantum Gravity},
     year = 1994,
    month = oct,
   volume = 11,
    pages = {2553-2574},
      doi = {10.1088/0264-9381/11/10/015},
   adsurl = {http://adsabs.harvard.edu/abs/1994CQGra..11.2553C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



%% ============================================================
%% ====== Contopoulos G et al.  ======
%% ============================================================


%
@article{contopoulos2001development,
  title={The development of nonlinear dynamics in astronomy},
  author={Contopoulos, G},
  journal={Foundations of Physics},
  volume={31},
  number={1},
  pages={89--114},
  year={2001},
  publisher={Springer}
}

% 2002ocda.book.....C,
@BOOK{contopoulosOCDA2002,
   author = {{Contopoulos}, G.},
    title = "{Order and chaos in dynamical astronomy}",
 keywords = {CELESTIAL MECHANICS, ASTRODYNAMICS, DYNAMICS, CHAOS},
  publisher = {Springer-Verlag},
booktitle = {Order and chaos in dynamical astronomy /George Contopoulos. Berlin : Springer, c2002.  (Astronomy and astrophys library) QB 351 .K58 2002},
     year = 2002,
   adsurl = {http://adsabs.harvard.edu/abs/2002ocda.book.....C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1960ZA.....49..273C,
@ARTICLE{contopoulos1960ZA,
   author = {{Contopoulos}, G.},
    title = "{A third Integral of Motion in a Galaxy}",
  journal = {\zap},
     year = 1960,
   volume = 49,
    pages = {273},
   adsurl = {http://adsabs.harvard.edu/abs/1960ZA.....49..273C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1963AJ.....68....1C,
@ARTICLE{contopoulos1963AJ,
   author = {{Contopoulos}, G.},
    title = "{On the existence of a third integral of motion}",
  journal = {\aj},
     year = 1963,
    month = feb,
   volume = 68,
    pages = {1},
      doi = {10.1086/108903},
   adsurl = {http://adsabs.harvard.edu/abs/1963AJ.....68....1C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Coperstook et al  ======
%% ============================================================

@article{doi:10.1142/S0217751X0703666X,
author = {Cooperstock, F. I. and Tieu, S.},
title = {GALACTIC DYNAMICS VIA GENERAL RELATIVITY: A COMPILATION AND NEW DEVELOPMENTS},
journal = {International Journal of Modern Physics A},
volume = {22},
number = {13},
pages = {2293-2325},
year = {2007},
doi = {10.1142/S0217751X0703666X},

%URL = {http://www.worldscientific.com/doi/abs/10.1142/S0217751X0703666X},
%eprint = {http://www.worldscientific.com/doi/pdf/10.1142/S0217751X0703666X}
}

@Article{Carrick2012,
author="Carrick, J. D.
and Cooperstock, F. I.",
title="General relativistic dynamics applied to the rotation curves of galaxies",
journal="Astrophysics and Space Science",
year="2012",
month="Jan",
day="01",
volume="337",
number="1",
pages="321--329",
abstract="We extend our general relativistic analysis of galactic rotation curves (see Cooperstock and Tieu in Int. J. Mod. Phys. A 22:2293, 2007) with galaxies NGC 2841, NGC 2903 and NGC 5033. As before, we employ the solution of the Einstein field equations of general relativity with an expansion in Bessel functions. As in our earlier studies, the fits to the data are found to be very precise and the calculated baryonic masses are lower than those based upon Newtonian gravity. Also as in our previous studies, the galactic radii at which the optical luminosities terminate are seen to correlate with densities near 10â21.75 kg{\thinspace}mâ3. This concordance lends further support to the correctness of the procedure as well as providing a potentially valuable piece of information in the understanding of galactic evolution.",
%issn="1572-946X",
%doi="10.1007/s10509-011-0854-z",
%url="http://dx.doi.org/10.1007/s10509-011-0854-z"
}




%% ============================================================
%% ====== Corchero  ======
%% ============================================================

@article{0264-9381-15-11-022,
  author={E S Corchero},
  title={Equilibrium of spheres with local anisotropy in post-Newtonian gravity. Application to supermassive stars},
  journal={Classical and Quantum Gravity},
  volume={15},
  number={11},
  pages={3645},
  year={1998},
  %url={http://stacks.iop.org/0264-9381/15/i=11/a=022},
  abstract={A generalization of the theory of stellar equilibrium is proposed which involves the possibility of local anisotropy (unequal principal stresses) even if the star is formed by an otherwise perfect fluid. Using this theory, supermassive stars are studied in the post-Newtonian approximation and it is shown that there are equilibrium configurations with local anisotropy having mass above, or entropy below, the standard limit with local isotropy.}
}


%% ============================================================
%% ====== Das  ======
%% ============================================================


@article{doi:10.1063/1.532002,
author = {A. Das and N. Tariq and D. Aruliah and T. Biech},
title = {Spherically symmetric collapse of an anisotropic fluid body into an exotic black hole},
journal = {Journal of Mathematical Physics},
volume = {38},
number = {8},
pages = {4202-4227},
year = {1997},
doi = {10.1063/1.532002},

%URL = {http://dx.doi.org/10.1063/1.532002

}

@article{doi:10.1063/1.1621056,
author = {A. Das and A. DeBenedictis and N. Tariq},
title = {General solutions of Einstein spherically symmetric gravitational equations with junction conditions},
journal = {Journal of Mathematical Physics},
volume = {44},
number = {12},
pages = {5637-5655},
year = {2003},
doi = {10.1063/1.1621056},

%URL = {http://aip.scitation.org/doi/abs/10.1063/1.1621056

}

@article{PhysRevD.62.104002,
  title = {Analytical solutions of a spherically symmetric collapse of an anisotropic fluid body into a regular black hole},
  author = {Das, A. and Kloster, S.},
  journal = {Phys. Rev. D},
  volume = {62},
  issue = {10},
  pages = {104002},
  numpages = {10},
  year = {2000},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.62.104002},
 % url = {https://link.aps.org/doi/10.1103/PhysRevD.62.104002}
}






%% ============================================================
%% ====== de Blok WJ et al.  ======
%% ============================================================

% 1997MNRAS.290..533D,
@ARTICLE{deblokMcgaugh1997MNRAS,
   author = {{de Blok}, W. J. G. and {McGaugh}, S. S.},
    title = "{The dark and visible matter content of low surface brightness disc galaxies}",
  journal = {\mnras},
   eprint = {astro-ph/9704274},
 keywords = {GALAXIES: FUNDAMENTAL PARAMETERS, GALAXIES: HALOES, GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: SPIRAL, DARK MATTER},
     year = 1997,
    month = sep,
   volume = 290,
    pages = {533-552},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.290..533D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Deg N et al.  ======
%% ============================================================

% 2013MNRAS.428..912D,
@ARTICLE{degWidrow2013MNRAS,
   author = {{Deg}, N. and {Widrow}, L.},
    title = "{The Sagittarius stream and halo triaxiality}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1209.6614},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2013,
    month = jan,
   volume = 428,
    pages = {912-922},
      doi = {10.1093/mnras/sts089},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.428..912D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Dejonghe H et al.  ======
%% ============================================================

% 1988ApJ...333...90D,
@ARTICLE{dejongheDezeeuw1988ApJ,
   author = {{Dejonghe}, H. and {de Zeeuw}, T.},
    title = "{Analytic axisymmetric galaxy models with three integrals of motion}",
  journal = {\apj},
 keywords = {Astronomical Models, Galactic Structure, Stellar Motions, Axisymmetric Flow, Cylindrical Coordinates},
     year = 1988,
    month = oct,
   volume = 333,
    pages = {90-129},
      doi = {10.1086/166727},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...333...90D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== de Zeeuw T et al.  ======
%% ============================================================

% 1985MNRAS.216..273D,
@ARTICLE{dezeeuw1985MNRAS,
   author = {{de Zeeuw}, T.},
    title = "{Elliptical galaxies with separable potentials}",
  journal = {\mnras},
 keywords = {Celestial Mechanics, Elliptical Galaxies, Equations Of Motion, Galactic Structure, Gravitational Fields, Stellar Orbits, Astronomical Models, Density Distribution, Many Body Problem, Mass Distribution},
     year = 1985,
    month = sep,
   volume = 216,
    pages = {273-334},
   adsurl = {http://adsabs.harvard.edu/abs/1985MNRAS.216..273D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1987IAUS..127..271D,
@INPROCEEDINGS{dezeeuw1987IAUS,
   author = {{de Zeeuw}, P. T.},
    title = "{Dynamical models for axisymmetric and triaxial galaxies}",
 keywords = {Astronomical Models, Dynamic Models, Elliptical Galaxies, Galactic Structure, Distribution Functions, Hydrodynamics, Integrals, Stellar Motions},
booktitle = {Structure and Dynamics of Elliptical Galaxies},
     year = 1987,
   series = {IAU Symposium},
   volume = 127,
   editor = {{de Zeeuw}, P. T.},
    pages = {271-289},
   adsurl = {http://adsabs.harvard.edu/abs/1987IAUS..127..271D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1988NYASA.536...15D,
@ARTICLE{dezeeuw1988NYASA,
   author = {{de Zeeuw}, T.},
    title = "{Integrable Models for Galaxies}",
  journal = {Annals of the New York Academy of Sciences},
     year = 1988,
    month = aug,
   volume = 536,
    pages = {15-24},
      doi = {10.1111/j.1749-6632.1988.tb51558.x},
   adsurl = {http://adsabs.harvard.edu/abs/1988NYASA.536...15D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1990ApJ...356..365D,
@ARTICLE{dezeeuwHunter1990ApJ,
   author = {{de Zeeuw}, P. T. and {Hunter}, C.},
    title = "{Oblate galaxy models with thin tube orbits}",
  journal = {\apj},
 keywords = {Astronomical Models, Galactic Structure, Distribution Functions, Integral Equations, Kinematics, Orbital Mechanics, Stellar Motions, Velocity Distribution},
     year = 1990,
    month = jun,
   volume = 356,
    pages = {365-388},
      doi = {10.1086/168846},
   adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...356..365D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ======Dev et al.  ======
%% ============================================================


@article{Dev:2000gt,
      author         = "Dev, Krsna and Gleiser, Marcelo",
      title          = "{Anisotropic stars: Exact solutions}",
      journal        = "Gen. Rel. Grav.",
      volume         = "34",
      year           = "2002",
      pages          = "1793-1818",
      doi            = "10.1023/A:1020707906543",
      %eprint         = "astro-ph/0012265",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0012265;%%"
}


%% ============================================================
%% ====== d'Inverno R et al.  ======
%% ============================================================

%
@book{dinverno,
  title={Introducing Einstein's Relativity},
  year={1992},
  author={d'Inverno, RA},
  publisher={Oxford University Press},
  address ={Oxford}
}

%% ============================================================
%% ====== Eddington  ======
%% ============================================================


@ARTICLE{1916MNRAS..76..572E,
   author = {{Eddington}, A. S.},
    title = "{The distribution of stars in globular clusters}",
  journal = {\mnras},
     year = 1916,
    month = may,
   volume = 76,
    pages = {572-585},
      doi = {10.1093/mnras/76.7.572},
   adsurl = {http://adsabs.harvard.edu/abs/1916MNRAS..76..572E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Efthymiopoulos C et al.  ======
%% ============================================================

% 2007LNP...729..297E,
@INPROCEEDINGS{efthymiopoulosEtal2007LNP,
   author = {{Efthymiopoulos}, C. and {Voglis}, N. and {Kalapotharakos}, C.
	},
    title = "{Special Features of Galactic Dynamics}",
 keywords = {Galactic dynamics, Celestial Mechanics, Dynamical Systems},
booktitle = {Topics in Gravitational Dynamics: Solar, Extra-Solar and Galactic Systems.},
     year = 2007,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 729,
   eprint = {astro-ph/0610246},
   editor = {{Benest}, D. and {Froeschle}, C. and {Lega}, E.},
    pages = {297-389},
      doi = {10.1007/978-3-540-72984-6\_11},
   adsurl = {http://adsabs.harvard.edu/abs/2007LNP...729..297E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2010EPJST.186...91E,
@ARTICLE{efthymiopoulos2010EPJST,
   author = {{Efthymiopoulos}, C.},
    title = "{Special features of galactic dynamics: Disc dynamics}",
  journal = {European Physical Journal Special Topics},
     year = 2010,
    month = sep,
   volume = 186,
    pages = {91-122},
      doi = {10.1140/epjst/e2010-01261-8},
   adsurl = {http://adsabs.harvard.edu/abs/2010EPJST.186...91E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Evans et al.  ======
%% ============================================================

@ARTICLE{2005MNRAS.360..492E,
   author = {{Evans}, N. W. and {An}, J.},
    title = "{Hypervirial models of stellar systems}",
  journal = {\mnras},
   eprint = {astro-ph/0501091},
 keywords = {stellar dynamics, celestial mechanics, galaxies: elliptical and lenticular, cD, galaxies: kinematics and dynamics, galaxies: structure},
     year = 2005,
    month = jun,
   volume = 360,
    pages = {492-498},
      doi = {10.1111/j.1365-2966.2005.09078.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.360..492E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Famaey B et al.  ======
%% ============================================================

% 2005MNRAS.363..603F,
@ARTICLE{famaeyBinney2005MNRAS,
   author = {{Famaey}, B. and {Binney}, J.},
    title = "{Modified Newtonian dynamics in the Milky Way}",
  journal = {\mnras},
   eprint = {astro-ph/0506723},
 keywords = {gravitation, Galaxy: kinematics and dynamics},
     year = 2005,
    month = oct,
   volume = 363,
    pages = {603-608},
      doi = {10.1111/j.1365-2966.2005.09474.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.363..603F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2012LRR....15...10F,
@ARTICLE{famaeyMcgaugh2012LRR,
   author = {{Famaey}, B. and {McGaugh}, S. S.},
    title = "{Modified Newtonian Dynamics (MOND): Observational Phenomenology and Relativistic Extensions}",
  journal = {Living Reviews in Relativity},
archivePrefix = "arXiv",
   eprint = {1112.3960},
 keywords = {astronomical observations, Newtonian limit, equations of motion, extragalactic astronomy, cosmology, theories of gravity, fundamental physics, astrophysics},
     year = 2012,
    month = sep,
   volume = 15,
    pages = {10},
      doi = {10.12942/lrr-2012-10},
   adsurl = {http://adsabs.harvard.edu/abs/2012LRR....15...10F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2012sf2a.conf...15F,
@INPROCEEDINGS{famaey2012SF2A,
   author = {{Famaey}, B.},
    title = "{Gaia and the dynamics of the Galaxy}",
 keywords = {Galaxy: kinematics and dynamics, Galaxy: evolution},
booktitle = {SF2A-2012: Proceedings of the Annual meeting of the French Society of Astronomy and Astrophysics},
     year = 2012,
archivePrefix = "arXiv",
   eprint = {1209.5753},
 primaryClass = "astro-ph.GA",
   editor = {{Boissier}, S. and {de Laverny}, P. and {Nardetto}, N. and {Samadi}, R. and
	{Valls-Gabaud}, D. and {Wozniak}, H.},
    month = dec,
    pages = {15-24},
   adsurl = {http://adsabs.harvard.edu/abs/2012sf2a.conf...15F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Freeman K et al.  ======
%% ============================================================

%1970ApJ...160..811F,
@ARTICLE{freeman1970ApJ,
   author = {{Freeman}, K. C.},
    title = "{On the Disks of Spiral and so Galaxies}",
  journal = {\apj},
     year = 1970,
    month = jun,
   volume = 160,
    pages = {811},
      doi = {10.1086/150474},
   adsurl = {http://adsabs.harvard.edu/abs/1970ApJ...160..811F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Garcia A et al.  ======
%% ============================================================

% 2013arXiv1306.2549G,
@ARTICLE{garciaHackmannEtal2013arxiv,
   author = {{Garcia}, A. and {Hackmann}, E. and {Kunz}, J. and {L{\"a}mmerzahl}, C. and
	{Macias}, A.},
    title = "{Motion of test particles in a regular black hole space--time}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1306.2549},
 primaryClass = "gr-qc",
 keywords = {General Relativity and Quantum Cosmology},
     year = 2013,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1306.2549G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Geroch R et al.  ======
%% ============================================================

% 1987PhRvD..36.1017G,
@ARTICLE{gerochTraschen1987PRD,
   author = {{Geroch}, R. and {Traschen}, J.},
    title = "{Strings and other distributional sources in general relativity}",
  journal = {\prd},
 keywords = {Fundamental problems and general formalism},
     year = 1987,
    month = aug,
   volume = 36,
    pages = {1017-1031},
      doi = {10.1103/PhysRevD.36.1017},
   adsurl = {http://adsabs.harvard.edu/abs/1987PhRvD..36.1017G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Gonzalez GA et al.  ======
%% ============================================================

%1999CQGra..16..479G,
@ARTICLE{gonzalezLetelier1999CQGra,
   author = {{Gonz{\'a}lez}, G. A. and {Letelier}, P. S.},
    title = "{Relativistic static thin discs with radial stress support}",
  journal = {Classical and Quantum Gravity},
   eprint = {gr-qc/9803071},
     year = 1999,
    month = feb,
   volume = 16,
    pages = {479-494},
      doi = {10.1088/0264-9381/16/2/012},
   adsurl = {http://adsabs.harvard.edu/abs/1999CQGra..16..479G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%2006MNRAS.371.1873G,
@ARTICLE{gonzalezReina2006MNRAS,
   author = {{Gonz{\'a}lez}, G. A. and {Reina}, J. I.},
    title = "{An infinite family of generalized Kalnajs discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0806.4266},
 keywords = {stellar dynamics: galaxies: kinematics and dynamics, stellar dynamics, galaxies: kinematics and dynamics},
     year = 2006,
    month = oct,
   volume = 371,
    pages = {1873-1876},
      doi = {10.1111/j.1365-2966.2006.10819.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.371.1873G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%2010MNRAS.404..468G,
@ARTICLE{gonzalezPlataplataRamoscaro2010MNRAS,
   author = {{Gonz{\'a}lez}, G. A. and {Plata-Plata}, S. M. and {Ramos-Caro}, J.},
    title = "{Finite thin disc models of four galaxies in the UrsaMajor cluster: NGC3877, NGC3917, NGC3949 and NGC4010}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0906.1355},
 primaryClass = "astro-ph.GA",
 keywords = {stellar dynamics, galaxies: kinematics and dynamics},
     year = 2010,
    month = may,
   volume = 404,
    pages = {468-474},
      doi = {10.1111/j.1365-2966.2010.16303.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.404..468G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% gonzalez2012stationary
@article{gonzalezGutierrez2012CQGra,
  title={Stationary axially symmetric relativistic thin discs with nonzero radial pressure},
  author={Gonz{\'a}lez, Guillermo A and Guti{\'e}rrez-Pi{\ n}eres, Antonio C},
  journal={Classical and Quantum Gravity},
  volume={29},
  number={13},
  pages={135001},
  year={2012},
  publisher={IOP Publishing}
}


%% ============================================================
%% ====== Håkan Andréasson  ======
%% ============================================================

@Article{Andreasson2011,

author="Andr{\'e}asson, H{\aa}kan",

title="The Einstein-Vlasov System/Kinetic Theory",

journal="Living Reviews in Relativity",
year="2011",
month="May",
day="27",
volume="14",
number="1",
pages="4",

abstract="The main purpose of this article is to provide a guide to theorems on global properties of solutions to the Einstein-Vlasov system. This system couples Einstein's equations to a kinetic matter model. Kinetic theory has been an important field of research during several decades in which the main focus has been on non-relativistic and special relativistic physics, i.e., to model the dynamics of neutral gases, plasmas, and Newtonian self-gravitating systems. In 1990, Rendall and Rein initiated a mathematical study of the Einstein-Vlasov system. Since then many theorems on global properties of solutions to this system have been established. This paper gives introductions to kinetic theory in non-curved spacetimes and then the Einstein-Vlasov system is introduced. We believe that a good understanding of kinetic theory in non-curved spacetimes is fundamental to a good comprehension of kinetic theory in general relativity.",

issn="1433-8351",

doi="10.12942/lrr-2011-4",

url="http://dx.doi.org/10.12942/lrr-2011-4"
}




%% ============================================================
%% ====== Hawking SW et al.  ======
%% ============================================================

%
@book{hawkingEllisLSS,
  author = {{Hawking}, S. W. and {Ellis}, G. F. R.},
  title  = {The Large-Scale Structure of Space-Time},
  publisher = {Cambridge Univ. Press},
  year = {2008},
  address = {Cambridge, UK}	
}

%% ============================================================
%% ====== Helmi A et al.  ======
%% ============================================================

% 2004MNRAS.351..643H,
@ARTICLE{helmi2004MNRAS,
   author = {{Helmi}, A.},
    title = "{Is the dark halo of our Galaxy spherical?}",
  journal = {\mnras},
   eprint = {astro-ph/0309579},
 keywords = {Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure, galaxies: haloes, dark matter},
     year = 2004,
    month = jun,
   volume = 351,
    pages = {643-648},
      doi = {10.1111/j.1365-2966.2004.07812.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.351..643H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Henon M et al.  ======
%% ============================================================

% 1964AJ.....69...73H,
@ARTICLE{henonheiles1964AJ,
   author = {{Henon}, M. and {Heiles}, C.},
    title = "{The applicability of the third integral of motion: Some numerical experiments}",
  journal = {\aj},
     year = 1964,
    month = feb,
   volume = 69,
    pages = {73},
      doi = {10.1086/109234},
   adsurl = {http://adsabs.harvard.edu/abs/1964AJ.....69...73H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Hernandez-Pastora JL et al.  ======
%% ============================================================	

% 2013PhRvD..88f4041H,
@ARTICLE{hernandezpastoraHerreraOspino2013PRD,
   author = {{Hern\'{a}ndez-Pastora}, J. L. and {Herrera}, L. and {Ospino}, J.
	},
    title = "{Geodesics in the linearized multipole solution: Distinguishing black holes from naked singularities}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1309.2455},
 primaryClass = "gr-qc",
 keywords = {Fundamental problems and general formalism, Singularities and cosmic censorship, Experimental tests of gravitational theories, Black holes},
     year = 2013,
    month = sep,
   volume = 88,
   number = 6,
      eid = {064041},
    pages = {064041},
      doi = {10.1103/PhysRevD.88.064041},
   adsurl = {http://adsabs.harvard.edu/abs/2013PhRvD..88f4041H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{doi:10.1139/p03-124,
author = {H. Hern\'{a}ndez and L. A. Nu\~{n}ez},
title = {Nonlocal equation of state in anisotropic static fluid spheres in general relativity},
journal = {Canadian Journal of Physics},
volume = {82},
number = {1},
pages = {29-51},
year = {2004},
doi = {10.1139/p03-124},

%URL = {https://doi.org/10.1139/p03-124

}

%% ============================================================
%% ====== Hernquist L et al.  ======
%% ============================================================	

% 1990ApJ...356..359H,
@ARTICLE{hernquist1990ApJ,
   author = {{Hernquist}, L.},
    title = "{An analytical model for spherical galaxies and bulges}",
  journal = {\apj},
 keywords = {Computational Astrophysics, Elliptical Galaxies, Galactic Bulge, Galactic Structure, Astronomical Models, Astronomical Photometry, Brightness Distribution, Distribution Functions},
     year = 1990,
    month = jun,
   volume = 356,
    pages = {359-364},
      doi = {10.1086/168845},
   adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...356..359H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


7%% ============================================================
%% ====== Herrera et al.  ======
%% ============================================================

@ARTICLE{1997PhR...286...53H,
   author = {{Herrera}, L. and {Santos}, N. O.},
    title = "{Local anisotropy in self-gravitating systems}",
  journal = {\physrep},
     year = 1997,
    month = jul,
   volume = 286,
    pages = {53-130},
      doi = {10.1016/S0370-1573(96)00042-7},
   adsurl = {http://adsabs.harvard.edu/abs/1997PhR...286...53H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{HERRERA1998113,
title = "On the role of density inhomogeneity and local anisotropy in the fate of spherical collapse",
journal = "Physics Letters A",
volume = "237",
number = "3",
pages = "113 - 118",
year = "1998",
note = "",
doi = "http://dx.doi.org/10.1016/S0375-9601(97)00874-8",
author = "L. Herrera and A. Di Prisco and J.L. Hern\'{a}ndez-Pastora and N.O Santos",
%issn = "0375-9601",
%url = "http://www.sciencedirect.com/science/article/pii/S0375960197008748",
}

@article{PhysRevD.69.084026,
  title = {Spherically symmetric dissipative anisotropic fluids: A general study},
  author = {Herrera, L. and Di Prisco, A. and Martin, J. and Ospino, J. and Santos, N. O. and Troconis, O.},
  journal = {Phys. Rev. D},
  volume = {69},
  issue = {8},
  pages = {084026},
  numpages = {12},
  year = {2004},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.69.084026},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.69.084026}
}

@article{PhysRevD.77.027502,
  title = {All static spherically symmetric anisotropic solutions of Einstein's equations},
  author = {Herrera, L. and Ospino, J. and Di Prisco, A.},
  journal = {Phys. Rev. D},
  volume = {77},
  issue = {2},
  pages = {027502},
  numpages = {3},
  year = {2008},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.77.027502},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.77.027502}
}

@article{PhysRevD.87.087303,
  title = {Newtonian polytropes for anisotropic matter: General framework and applications},
  author = {Herrera, L. and Barreto, W.},
  journal = {Phys. Rev. D},
  volume = {87},
  issue = {8},
  pages = {087303},
  numpages = {5},
  year = {2013},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.87.087303},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.87.087303}
}







%% ============================================================
%% ====== Hieratinta J et al.  ======
%% ============================================================

% 1987PhR...147...87H,
@ARTICLE{hieratinta1987PhR,
   author = {{Hietarinta}, J.},
    title = "{Direct methods for the search of the second invariant}",
  journal = {\physrep},
     year = 1987,
    month = mar,
   volume = 147,
    pages = {87-154},
      doi = {10.1016/0370-1573(87)90089-5},
   adsurl = {http://adsabs.harvard.edu/abs/1987PhR...147...87H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Hirata CM et al.  ======
%% ============================================================

% 2011MNRAS.414.3198H,
@ARTICLE{hirata2011MNRAS1,
   author = {{Hirata}, C. M.},
    title = "{Lindblad resonance torques in relativistic discs - I. Basic equations}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1010.0758},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, black hole physics, relativistic processes},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {3198-3211},
      doi = {10.1111/j.1365-2966.2011.18617.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.3198H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2011MNRAS.414.3212H,
@ARTICLE{hirata2011MNRAS2,
   author = {{Hirata}, C. M.},
    title = "{Lindblad resonance torques in relativistic discs - II. Computation of resonance strengths}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1010.0759},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, black hole physics, relativistic processes},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {3212-3230},
      doi = {10.1111/j.1365-2966.2011.18619.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.3212H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Holmberg J et al.  ======
%% ============================================================	

% 2004MNRAS.352..440H,
@ARTICLE{holmbergFlynn2004MNRAS,
   author = {{Holmberg}, J. and {Flynn}, C.},
    title = "{The local surface density of disc matter mapped by Hipparcos}",
  journal = {\mnras},
   eprint = {astro-ph/0405155},
 keywords = {Galaxy: kinematics and dynamics, Galaxy: structure, dark matter},
     year = 2004,
    month = aug,
   volume = 352,
    pages = {440-446},
      doi = {10.1111/j.1365-2966.2004.07931.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.352..440H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Hunter C et al.  ======
%% ============================================================	

% 1963MNRAS.126..299H,
@ARTICLE{hunter1963MNRAS,
   author = {{Hunter}, C.},
    title = "{The structure and stability of self-gravitating disks}",
  journal = {\mnras},
     year = 1963,
   volume = 126,
    pages = {299},
   adsurl = {http://adsabs.harvard.edu/abs/1963MNRAS.126..299H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2003LNP...626..137H,
@INPROCEEDINGS{hunter2003LNP,
   author = {{Hunter}, C.},
    title = "{Disk-Crossing Orbits}",
booktitle = {Galaxies and Chaos},
     year = 2003,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 626,
   editor = {{Contopoulos}, G. and {Voglis}, N.},
    pages = {137-153},
      doi = {10.1007/978-3-540-45040-5\_11},
   adsurl = {http://adsabs.harvard.edu/abs/2003LNP...626..137H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2005NYASA1045..120H,
@ARTICLE{hunter2005NYASA,
   author = {{Hunter}, C.},
    title = "{Chaos in Orbits Due to Disk Crossings}",
  journal = {Annals of the New York Academy of Sciences},
     year = 2005,
    month = jan,
   volume = 1045,
    pages = {120},
      doi = {10.1196/annals.1350.011},
   adsurl = {http://adsabs.harvard.edu/abs/2005NYASA1045..120H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Ibata RA et al.  ======
%% ============================================================	

% 2013ApJ...765L..15I,
@ARTICLE{ibataEtal2013ApJL,
   author = {{Ibata}, R. and {Lewis}, G. F. and {Martin}, N. F. and {Bellazzini}, M. and
	{Correnti}, M.},
    title = "{Does the Sagittarius Stream Constrain the Milky Way Halo to be Triaxial?}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1212.4958},
 primaryClass = "astro-ph.GA",
 keywords = {dark matter, galaxies: dwarf, Galaxy: halo },
     year = 2013,
    month = mar,
   volume = 765,
      eid = {L15},
    pages = {L15},
      doi = {10.1088/2041-8205/765/1/L15},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...765L..15I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Iorio L et al.  ======
%% ============================================================	

% 2012EM&P..108..189I,
@ARTICLE{iorio2012EMP,
   author = {{Iorio}, L.},
    title = "{Orbital Perturbations Due to Massive Rings}",
  journal = {Earth Moon and Planets},
archivePrefix = "arXiv",
   eprint = {1201.5307},
 primaryClass = "gr-qc",
 keywords = {Gravity, Asteroid belt, Interplanetary dust, Perturbation methods},
     year = 2012,
    month = jun,
   volume = 108,
    pages = {189-217},
      doi = {10.1007/s11038-012-9391-1},
   adsurl = {http://adsabs.harvard.edu/abs/2012EM%26P..108..189I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Irrgang A et al.  ======
%% ============================================================	

% 2013A&A...549A.137I,
@ARTICLE{irrgangEtal2013AA,
   author = {{Irrgang}, A. and {Wilcox}, B. and {Tucker}, E. and {Schiefelbein}, L.
	},
    title = "{Milky Way mass models for orbit calculations}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1211.4353},
 primaryClass = "astro-ph.GA",
 keywords = {dark matter, Galaxy: fundamental parameters, Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure, stars: kinematics and dynamics},
     year = 2013,
    month = jan,
   volume = 549,
      eid = {A137},
    pages = {A137},
      doi = {10.1051/0004-6361/201220540},
   adsurl = {http://adsabs.harvard.edu/abs/2013A\%26A...549A.137I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Jackson JD et al.  ======
%% ============================================================	

%
@book{jackson1962classical,
  title={Classical electrodynamics},
  author={Jackson, John David and Jackson, John D},
  volume={3},
  year={1962},
  publisher={Wiley New York etc.}
}


%% ============================================================
%% ====== Jaffe  ======
%% ============================================================	

@ARTICLE{1983MNRAS.202..995J,
   author = {{Jaffe}, W.},
    title = "{A simple model for the distribution of light in spherical galaxies}",
  journal = {\mnras},
 keywords = {Astronomical Models, Brightness Distribution, Galactic Radiation, Gravitational Fields, Light Emission, Surface Properties},
     year = 1983,
    month = mar,
   volume = 202,
    pages = {995-999},
      doi = {10.1093/mnras/202.4.995},
   adsurl = {http://adsabs.harvard.edu/abs/1983MNRAS.202..995J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%% ============================================================
%% ====== Johnston KV et al.  ======
%% ============================================================	

% 1995ApJ...451..598J,
@ARTICLE{johnstonEtal1995,
   author = {{Johnston}, K. V. and {Spergel}, D. N. and {Hernquist}, L.},
    title = "{The Disruption of the Sagittarius Dwarf Galaxy}",
  journal = {\apj},
   eprint = {astro-ph/9502005},
 keywords = {GALAXIES: EVOLUTION, GALAXIES: INDIVIDUAL NAME: SAGITTARIUS, GALAXIES: INTERACTIONS, GALAXY: STRUCTURE},
     year = 1995,
    month = oct,
   volume = 451,
    pages = {598},
      doi = {10.1086/176247},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...451..598J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Juric M et al.  ======
%% ============================================================	

% 2008ApJ...673..864J,
@ARTICLE{juricEtal2008ApJ,
   author = {{Juri{\'c}}, M. and {Ivezi{\'c}}, {\v Z}. and {Brooks}, A. and
	{Lupton}, R. H. and {Schlegel}, D. and {Finkbeiner}, D. and
	{Padmanabhan}, N. and {Bond}, N. and {Sesar}, B. and {Rockosi}, C. M. and
	{Knapp}, G. R. and {Gunn}, J. E. and {Sumi}, T. and {Schneider}, D. P. and
	{Barentine}, J. C. and {Brewington}, H. J. and {Brinkmann}, J. and
	{Fukugita}, M. and {Harvanek}, M. and {Kleinman}, S. J. and
	{Krzesinski}, J. and {Long}, D. and {Neilsen}, Jr., E. H. and
	{Nitta}, A. and {Snedden}, S. A. and {York}, D. G.},
    title = "{The Milky Way Tomography with SDSS. I. Stellar Number Density Distribution}",
  journal = {\apj},
   eprint = {astro-ph/0510520},
 keywords = {Galaxy: Disk, Galaxy: Fundamental Parameters, Galaxy: Halo, Galaxy: Structure},
     year = 2008,
    month = feb,
   volume = 673,
    pages = {864-914},
      doi = {10.1086/523619},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...673..864J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Semerak et al.  ======
%% ============================================================	

% 2004CQGra..21R...1K,
@ARTICLE{karasHureSemerak2004CQGra,
   author = {{Karas}, V. and {Hur{\'e}}, J.-M. and {Semer{\'a}k}, O.},
    title = "{TOPICAL REVIEW:  Gravitating discs around black holes}",
  journal = {Classical and Quantum Gravity},
   eprint = {astro-ph/0401345},
     year = 2004,
    month = apr,
   volume = 21,
    pages = {1},
      doi = {10.1088/0264-9381/21/7/R01},
   adsurl = {http://adsabs.harvard.edu/abs/2004CQGra..21R...1K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{0264-9381-17-7-303,
  author={O. Semer\'{a}k and M. Z\'{a}cek},
  title={Gravitating discs around a Schwarzschild black hole: I},
  journal={Classical and Quantum Gravity},
  volume={17},
  number={7},
  pages={1613},
  year={2000},
  abstract={We study the class of Lemos-Letelier annular discs (realistic gravitating static axisymmetric thin discs obtained by inversion of the first Morgan-Morgan solution) around Schwarzschild black holes. For each value of the inner radius, the range of masses is found when all of the disc can be interpreted by counter-rotating streams of particles on stable timelike geodesics. One can then consider a sequence of stable physical discs with different masses and inner rims at the corresponding least possible radii. The basic properties of this sequence are shown on positions of the inner rims and of important circular orbits, on positions of the horizon and on density and Keplerian-velocity profiles within the discs, plotted in terms of the Schwarzschild radial coordinate, circumferential radius and proper distance from the horizon.}
% url={http://stacks.iop.org/0264-9381/17/i=7/a=303},
}

@article{0264-9381-19-14-321,
  author={O Semer\'{a}k},
  title={Thin disc around a rotating black hole, but with support in-between},
  journal={Classical and Quantum Gravity},
  volume={19},
  number={14},
  pages={3829},
  year={2002},
  abstract={In the previous paper, we presented the metric obtained from a general Weyl seed using the BelinskiiâZakharov inverse-scattering technique with two real solitons. It describes the field of a stationary black hole surrounded by a source inherited from the seed. In the present paper, we study the solution in further detail with the inverted first MorganâMorgan counter-rotating disc employed as a seed. In particular, the properties of the horizon, the static limit, the equatorial plane, the extreme limit of the solution and the resulting external disc are analysed and illustrated. It turns out that there is a jump in derivatives of the metric in the equatorial plane even below the seed disc, indicating the presence of a 'suspension layer' that confines the system against gravitational collapse or decay. Hence, the solution cannot represent a realistic axisymmetric accretion disc around a rotating black hole.}
%  url={http://stacks.iop.org/0264-9381/19/i=14/a=321},
}

@Article{semerak2002,
author="{\v{Z}}{\'a}{\v{c}}ek, M.
and Semer{\'a}k, O.",
title="Gravitating discs around a Schwarzschild black hole II",
journal="Czechoslovak Journal of Physics",
year="2002",
month="Jan",
day="01",
volume="52",
number="1",
pages="19--27",
abstract="A sequence of exact spacetimes is obtained describing the fields of a Schwarzschild black hole surrounded by stable static axisymmetric thin discs having their inner rim at the least possible radius. In the previous paper we only required stability with respect to perturbations in the disc plane, while it turns out that for discs with relative mass >0.23 the perturbations in perpendicular direction are more dangerous. The discs of the resulting sequence have their inner rims just on, or very close to, circular geodesics marginally stable with respect to either of the perturbations. Redshift from static and Keplerian observers in the disc is computed. The inverted first Morgan-Morgan counter-rotating disc, used in superpositions, has a number of satisfactory physical properties, but it has turned out to have a curvature singularity at the inner rim. However, this is only a consequence of a too steep radial start of density, not present in (inverted) ``higher'' Morgan-Morgan solutions.",
%issn="1572-9486",
%doi="10.1023/A:1013957512339",
%url="http://dx.doi.org/10.1023/A:1013957512339"
}

%% ============================================================
%% ====== Kehagias A et al.  ======
%% ============================================================	

% 2009PhLB..678..123K,
@ARTICLE{kehagiasSfetsos2009PhLB,
   author = {{Kehagias}, A. and {Sfetsos}, K.},
    title = "{The black hole and FRW geometries of non-relativistic gravity}",
  journal = {Physics Letters B},
archivePrefix = "arXiv",
   eprint = {0905.0477},
 primaryClass = "hep-th",
     year = 2009,
    month = jul,
   volume = 678,
    pages = {123-126},
      doi = {10.1016/j.physletb.2009.06.019},
   adsurl = {http://adsabs.harvard.edu/abs/2009PhLB..678..123K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Kent SM et al.  ======
%% ============================================================	

% 1986AJ.....91.1301K,
@ARTICLE{kent1986AJ,
   author = {{Kent}, S. M.},
    title = "{Dark matter in spiral galaxies. I - Galaxies with optical rotation curves}",
  journal = {\aj},
 keywords = {Brightness Distribution, Galactic Structure, Missing Mass (Astrophysics), Spectral Energy Distribution, Spiral Galaxies, Visible Spectrum, Astronomical Models, Charge Coupled Devices, Mass Distribution, Mass To Light Ratios, Tables (Data)},
     year = 1986,
    month = jun,
   volume = 91,
    pages = {1301-1327},
      doi = {10.1086/114106},
   adsurl = {http://adsabs.harvard.edu/abs/1986AJ.....91.1301K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1987AJ.....93..816K,
@ARTICLE{kent1987AJ,
   author = {{Kent}, S. M.},
    title = "{Dark matter in spiral galaxies. II - Galaxies with H I rotation curves}",
  journal = {\aj},
 keywords = {Angular Velocity, Brightness Distribution, Dark Matter, Hydrogen Clouds, Mass Distribution, Spiral Galaxies, Astronomical Models, Galactic Structure, Mass To Light Ratios, Star Distribution},
     year = 1987,
    month = apr,
   volume = 93,
    pages = {816-832},
      doi = {10.1086/114366},
   adsurl = {http://adsabs.harvard.edu/abs/1987AJ.....93..816K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Kluzniak W et al.  ======
%% ============================================================	

% 2013MNRAS.434.2825K,
@ARTICLE{kluzniakRosinska2013MNRAS,
   author = {{Klu{\'z}niak}, W. and {Rosi{\'n}ska}, D.},
    title = "{Orbital and epicyclic frequencies of Maclaurin spheroids}",
  journal = {\mnras},
 keywords = {black hole physics, dense matter, gravitation, instabilities, stars: neutron},
     year = 2013,
    month = oct,
   volume = 434,
    pages = {2825-2829},
      doi = {10.1093/mnras/stt1185},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.434.2825K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Landau LD et al.  ======
%% ============================================================	

%
@book{landauLifshitzFM,
  author = {{Landau}, L. D. and {Lifshitz}, E. M.}, edition = {Second},
  title  = {Fluid Mechanics},
  publisher = {Elsevier},
  year = {2007},
  address = {Oxford, UK},	
  series = {Course of Theoretical Physics},  volume = {VI},
}

%% ============================================================
%% ====== Law DR et al.  ======
%% ============================================================	

% 2009ApJ...703L..67L,
@ARTICLE{lawEtal2009ApJL,
   author = {{Law}, D. R. and {Majewski}, S. R. and {Johnston}, K. V.},
    title = "{Evidence for a Triaxial Milky Way Dark Matter Halo from the Sagittarius Stellar Tidal Stream}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0908.3187},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2009,
    month = sep,
   volume = 703,
    pages = {L67-L71},
      doi = {10.1088/0004-637X/703/1/L67},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...703L..67L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Lee JM et al.  ======
%% ============================================================	

%
@book{lee2012smooth,
  title={Introduction to smooth manifolds},
  author={Lee, John},
  volume={218},
  year={2012},
  publisher={Springer}
}

%% ============================================================
%% ====== Lemos JPS et al.  ======
%% ============================================================	

% 1994PhRvD..49.5135L,
@ARTICLE{lemosLetelier1994PRD,
   author = {{Lemos}, J. P. S. and {Letelier}, P. S.},
    title = "{Exact general relativistic thin disks around black holes}",
  journal = {\prd},
 keywords = {Exact solutions, Black holes},
     year = 1994,
    month = may,
   volume = 49,
    pages = {5135-5143},
      doi = {10.1103/PhysRevD.49.5135},
   adsurl = {http://adsabs.harvard.edu/abs/1994PhRvD..49.5135L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{0264-9381-10-6-003,
  author={J P S Lemos and P S Letelier},
  title={Superposition of Morgan and Morgan discs with a Schwarzschild black hole},
  journal={Classical and Quantum Gravity},
  volume={10},
  number={6},
  pages={L75},
  year={1993},
  abstract={The exact superposition of a black hole and a thin disc is considered. The disc is made of counter-rotating particles and belongs to the Morgan and Morgan family (1969). There are three parameters to play with, the black hole mass, and the disc mass and radius. The superposed exact solution comprehends several configurations, some yield mass ratios in conformity with the usual accretion discs. There is also a remarkable configuration of a black hole surrounded by a disc made of pure superluminal matter up to the edge, which is at the photonic orbit.}
%url={http://stacks.iop.org/0264-9381/10/i=6/a=003},
}




%% ============================================================
%% ====== Letelier PS et al.  ======
%% ============================================================	

% 2003PhRvD..68j4002L,
@ARTICLE{letelier2003PRD,
   author = {{Letelier}, P. S.},
    title = "{Stability of circular orbits of particles moving around black holes surrounded by axially symmetric structures}",
  journal = {\prd},
   eprint = {gr-qc/0309033},
 keywords = {Classical black holes, Orbit determination and improvement, Infall and accretion, Infall accretion and accretion disks},
     year = 2003,
    month = nov,
   volume = 68,
   number = 10,
      eid = {104002},
    pages = {104002},
      doi = {10.1103/PhysRevD.68.104002},
   adsurl = {http://adsabs.harvard.edu/abs/2003PhRvD..68j4002L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%1987JMP....28..165L,
@ARTICLE{letelierOliveira1987JMP,
   author = {{Letelier}, P. S. and {Oliveira}, S. R.},
    title = "{Exact self-gravitating disks and rings: A solitonic approach}",
  journal = {Journal of Mathematical Physics},
     year = 1987,
    month = jan,
   volume = 28,
    pages = {165-170},
      doi = {10.1063/1.527800},
   adsurl = {http://adsabs.harvard.edu/abs/1987JMP....28..165L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%
@article{letelier2005RBEF,
  title={Solu{\c{c}}{\~o}es exatas das equa{\c{c}}{\~o}es de Einstein com simetria axial},
  author={Letelier, Patricio S},
  journal={Revista Brasileira de Ensino de F{\'\i}sica},
  volume={27},
  number={1},
  pages={121--136},
  year={2005},
  publisher={SciELO Brasil}
}

% 2007MNRAS.381.1031L,
@ARTICLE{letelier2007MNRAS,
   author = {{Letelier}, P. S.},
    title = "{Simple potential-density pairs for flat rings}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0706.2802},
 keywords = {instabilities, planets: rings},
     year = 2007,
    month = nov,
   volume = 381,
    pages = {1031-1034},
      doi = {10.1111/j.1365-2966.2007.12128.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.381.1031L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{PhysRevD.62.064025,
  title = {Rotating relativistic thin disks},
  author = {Gonz\'alez, Guillermo A. and Letelier, Patricio S.},
  journal = {Phys. Rev. D},
  volume = {62},
  issue = {6},
  pages = {064025},
  numpages = {8},
  year = {2000},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.62.064025},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.62.064025}
}


%% ============================================================
%% ====== Lichtenberg AJ et al.  ======
%% ============================================================	

%
@book{lichtenbergLieberman1992,
  title={Regular and Chaotic Dynamics},
  author={Lichtenberg, AJ and Lieberman, M},
  publisher={Springer, New York},
  series={Applied Mathematical Sciences},
  volume={38},
  year={1992}
}

%% ============================================================
%% ====== Lynden-Bell  ======
%% ============================================================	


@ARTICLE{1962MNRAS.123..447L,
   author = {{Lynden-Bell}, D.},
    title = "{Stellar dynamics: Exact solution of the self-gravitation equation}",
  journal = {\mnras},
     year = 1962,
   volume = 123,
    pages = {447},
      doi = {10.1093/mnras/123.5.447},
   adsurl = {http://adsabs.harvard.edu/abs/1962MNRAS.123..447L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%% ============================================================
%% ====== Lora-Clavijo FD et al.  ======
%% ============================================================	

% 2010PhRvD..82h4005L,
@ARTICLE{loraclavijo-ospinahenao-pedraza2010PRD,
   author = {{Lora-Clavijo}, F. D. and {Ospina-Henao}, P. A. and {Pedraza}, J. F.
	},
    title = "{Charged annular disks and Reissner-Nordstr{\"o}m type black holes from extremal dust}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1009.1005},
 primaryClass = "gr-qc",
 keywords = {Exact solutions, Einstein-Maxwell spacetimes spacetimes with fluids radiation or classical fields, Galactic nuclei circumnuclear matter and bulges},
     year = 2010,
    month = oct,
   volume = 82,
   number = 8,
      eid = {084005},
    pages = {084005},
      doi = {10.1103/PhysRevD.82.084005},
   adsurl = {http://adsabs.harvard.edu/abs/2010PhRvD..82h4005L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Maharaj et al.  ======
%% ============================================================

@Article{Maharaj2006,
author="Maharaj, S. D.
and Chaisi, M.",
title="Equation of state for anisotropic spheres",
journal="General Relativity and Gravitation",
year="2006",
month="Nov",
day="01",
volume="38",
number="11",
pages="1723--1726",
abstract="We present a new class of exact interior solutions for anisotropic spheres to the Einstein field equations with a prescribed energy density. This category of solutions has similar energy density profiles to the models of Chaisi and Maharaj (Gen. Rel. Grav. 37, 1177--1189, 2005) whose approach we follow in the integration process. A distinguishing feature of the solutions presented is that they satisfy a barotropic equation of state linearly relating the radial pressure to the energy density.",
%issn="1572-9532",
%doi="10.1007/s10714-006-0353-7",
%url="http://dx.doi.org/10.1007/s10714-006-0353-7"
}

@article {MMA:MMA665,
author = {Maharaj, S. D. and Chaisi, M.},
title = {New anisotropic models from isotropic solutions},
journal = {Mathematical Methods in the Applied Sciences},
volume = {29},
number = {1},
publisher = {John Wiley & Sons, Ltd.},
doi = {10.1002/mma.665},
pages = {67--83},
keywords = {astrophysics, Einstein equations, dense stars},
year = {2006},
%issn = {1099-1476},
%url = {http://dx.doi.org/10.1002/mma.665},
}




%% ============================================================
%% ====== Mak et al.  ======
%% ============================================================	

@article {Mak393,
	author = {Mak, M.K. and Harko, T.},
	title = {Anisotropic stars in general relativity},
	volume = {459},
	number = {2030},
	pages = {393--408},
	year = {2003},
	doi = {10.1098/rspa.2002.1014},
	publisher = {The Royal Society},
	abstract = {We present a class of exact solutions of Einstein{\textquoteright}s gravitational{\textendash}field equations describing spherically symmetric and static anisotropic stellar{\textendash}type configurations. The solutions are obtained by assuming a particular form of the anisotropy factor. The energy density and both radial and tangential pressures are finite and positive inside the anisotropic star. Numerical results show that the basic physical parameters (mass and radius) of the model can describe realistic astrophysical objects such as neutron stars.},
	%issn = {1364-5021},
%	URL = {http://rspa.royalsocietypublishing.org/content/459/2030/393},
%	eprint = {http://rspa.royalsocietypublishing.org/content/459/2030/393.full.pdf},
	journal = {Proceedings of the Royal Society of London A: Mathematical, Physical and Engineering Sciences}
}

%% ============================================================
%% ====== McMillan PJ et al.  ======
%% ============================================================	

% 2008MNRAS.390..429M,
@ARTICLE{mcmillanBinney2008MNRAS,
   author = {{McMillan}, P. J. and {Binney}, J. J.},
    title = "{Disassembling the Galaxy with angle-action coordinates}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0806.0319},
 keywords = {methods: numerical , Galaxy: kinematics and dynamics , solar neighbourhood , Galaxy: structure},
     year = 2008,
    month = oct,
   volume = 390,
    pages = {429-437},
      doi = {10.1111/j.1365-2966.2008.13767.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.390..429M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2011MNRAS.414.2446M,
@ARTICLE{mcmillan2011MNRAS,
   author = {{McMillan}, P. J.},
    title = "{Mass models of the Milky Way}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1102.4340},
 primaryClass = "astro-ph.GA",
 keywords = {methods: statistical, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {2446-2457},
      doi = {10.1111/j.1365-2966.2011.18564.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.2446M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Milgrom M et al.  ======
%% ============================================================	

% 1983ApJ...270..365M,
@ARTICLE{milgrom1983ApJ,
   author = {{Milgrom}, M.},
    title = "{A modification of the Newtonian dynamics as a possible alternative to the hidden mass hypothesis}",
  journal = {\apj},
 keywords = {Cosmology, Galactic Structure, Nonrelativistic Mechanics, Stellar Motions, Particle Acceleration, Solar System},
     year = 1983,
    month = jul,
   volume = 270,
    pages = {365-370},
      doi = {10.1086/161130},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...270..365M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1983ApJ...270..371M,
@ARTICLE{milgrom1983ApJgalaxies,
   author = {{Milgrom}, M.},
    title = "{A modification of the Newtonian dynamics - Implications for galaxies}",
  journal = {\apj},
 keywords = {Galactic Structure, Newton Theory, Stellar Motions, Angular Velocity, Disk Galaxies, Elliptical Galaxies, Galactic Rotation, Mass Distribution, Milky Way Galaxy, Oort Cloud},
     year = 1983,
    month = jul,
   volume = 270,
    pages = {371-389},
      doi = {10.1086/161131},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...270..371M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1983ApJ...270..384M,
@ARTICLE{milgrom1983ApJgalaxysystems,
   author = {{Milgrom}, M.},
    title = "{A Modification of the Newtonian Dynamics - Implications for Galaxy Systems}",
  journal = {\apj},
     year = 1983,
    month = jul,
   volume = 270,
    pages = {384},
      doi = {10.1086/161132},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...270..384M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% 2010MNRAS.403..886M,
@ARTICLE{milgrom2010MNRAS,
   author = {{Milgrom}, M.},
    title = "{Quasi-linear formulation of MOND}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0911.5464},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: kinematics and dynamics, cosmology: theory, dark matter},
     year = 2010,
    month = apr,
   volume = 403,
    pages = {886-895},
      doi = {10.1111/j.1365-2966.2009.16184.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403..886M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% 2014MNRAS.437.2531M,
@ARTICLE{milgrom2014MNRAS,
   author = {{Milgrom}, M.},
    title = "{MOND laws of galactic dynamics}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1212.2568},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: general, galaxies: kinematics and dynamics, dark matter},
     year = 2014,
    month = jan,
   volume = 437,
    pages = {2531-2541},
      doi = {10.1093/mnras/stt2066},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.437.2531M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Mimoso et al. ======
%% ============================================================	

@article{PhysRevD.88.027301,
  title = {Separating expansion and collapse in general fluid models with heat flux},
  author = {Le Delliou, Morgan and Mimoso, Jos\'e P. and Mena, Filipe C. and Fontanini, Michele and Guariento, Daniel C. and Abdalla, Elcio},
  journal = {Phys. Rev. D},
  volume = {88},
  issue = {2},
  pages = {027301},
  numpages = {5},
  year = {2013},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.88.027301},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.88.027301}
}


%% ============================================================
%% ====== Misner CW et al. ======
%% ============================================================	

%
@book{misner1973gravitation,
  title={Gravitation},
  author={Misner, Charles W and Thorne, Kip S and Wheeler, John Archibald},
  year={1973},
  publisher={W. H. Freeman and Company},
  address={San Francisco}
}

%% ============================================================
%% ====== Miyamoto-Nagai  ======
%% ============================================================	

% 1975PASJ...27..533M,
@ARTICLE{miyamotoNagai1975PASJ,
   author = {{Miyamoto}, M. and {Nagai}, R.},
    title = "{Three-dimensional models for the distribution of mass in galaxies}",
  journal = {\pasj},
 keywords = {Astronomical Models, Density Distribution, Galactic Structure, Mass Distribution, Potential Theory, Three Dimensional Models, Functions (Mathematics), Globular Clusters, Gravitational Effects, Mathematical Models, Milky Way Galaxy},
     year = 1975,
   volume = 27,
    pages = {533-543},
   adsurl = {http://adsabs.harvard.edu/abs/1975PASJ...27..533M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Morgan & Morgan  ======
%% ============================================================	

% 1969PhRv..183.1097M,
@ARTICLE{morganMorgan1969PR,
   author = {{Morgan}, T. and {Morgan}, L.},
    title = "{The Gravitational Field of a Disk}",
  journal = {Physical Review},
     year = 1969,
    month = jul,
   volume = 183,
    pages = {1097-1101},
      doi = {10.1103/PhysRev.183.1097},
   adsurl = {http://adsabs.harvard.edu/abs/1969PhRv..183.1097M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1970PhRvD...2.2756M,
@ARTICLE{morganMorgan1970PRD,
   author = {{Morgan}, L. and {Morgan}, T.},
    title = "{Gravitational Field of Shells and Disks in General Relativity}",
  journal = {\prd},
     year = 1970,
    month = dec,
   volume = 2,
    pages = {2756-2761},
      doi = {10.1103/PhysRevD.2.2756},
   adsurl = {http://adsabs.harvard.edu/abs/1970PhRvD...2.2756M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Ollongren A et al.  ======
%% ============================================================	

% 1962BAN....16..241O,
@ARTICLE{ollongren1962BAIN,
   author = {{Ollongren}, A.},
    title = "{Three-dimensional galactic stellar orbits}",
  journal = {\bain},
     year = 1962,
    month = oct,
   volume = 16,
    pages = {241},
   adsurl = {http://adsabs.harvard.edu/abs/1962BAN....16..241O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Nucamendi et al.  ======
%% ============================================================	


@article{1742-6596-545-1-012006,
  author={A Herrera-Aguilar and U Nucamendi},
  title={A relativistic axisymmetric approach to the galactic rotation curves problem},
  journal={Journal of Physics: Conference Series},
  volume={545},
  number={1},
  pages={012006},
  year={2014},
  abstract={It is known that galactic potentials can be kinematically linked to the observed red/blue shifts of the corresponding galactic rotation curves under a minimal set of assumptions (see [1] and [2] for details): i ) that emitted photons come to us from stable timelike circular geodesic orbits of stars in a static spherically symmetric gravitational field, and ii ) that these photons propagate to us along null geodesics. This relation can be established without appealing at all to a concrete theory of gravitational interaction. This kinematical spherically symmetric approach to the galactic rotation curves problem can be generalized to the stationary axisymmetric realm, which is precisely the symmetry that spiral galaxies possess [3]. Here we review the relativistic results obtained in the latter work. Namely, by making use of the most general stationary axisymmetric metric, we consider stable circular orbits of stars that emit signals which travel to a distant observer along null geodesics and express the galactic red/blue shifts in terms of three arbitrary metric functions, clarifying the contribution of the rotation as well as the dragging of the gravitational field. This stationary axisymmetric approach distinguishes between red and blue shifts emitted by circularly orbiting receding and approaching stars, respectively, even when they are considered with respect to the center of a spiral galaxy, indicating the need of precise measurements in order to confront predictions with observations. We also point out the difficulties one encounters in the attempt of determining the metric functions from observations and list some potential strategies to overcome them.}
 % url={http://stacks.iop.org/1742-6596/545/i=1/a=012006},
}



%% ============================================================
%% ====== Papapetrou A et al.  ======
%% ============================================================	


@article{papapetrou1966,
author = {Papapetrou, A.},
journal = {Annales de l'institut Henri Poincar{\'e} (A) Physique th{\'e}orique},
language = {fre},
number = {2},
pages = {83-105},
publisher = {Gauthier-villars},
title = {Champs gravitationnels stationnaires {\`a} sym{\'e}trie axiale},
adsurl = {http://eudml.org/doc/75527},
volume = {4},
year = {1966},
}

%% ============================================================
%% ====== Pauli EM et al.  ======
%% ============================================================	

% 2003A&A...400..877P,
@ARTICLE{pauliEtal2003AA,
   author = {{Pauli}, E.-M. and {Napiwotzki}, R. and {Altmann}, M. and {Heber}, U. and
	{Odenkirchen}, M. and {Kerber}, F.},
    title = "{3D kinematics of white dwarfs from the SPY project}",
  journal = {\aap},
   eprint = {astro-ph/0301467},
 keywords = {stars: white dwarfs, stars: kinematics and dynamics, Galaxy: halo, Galaxy: disk, Galaxy: kinematics and dynamics},
     year = 2003,
    month = mar,
   volume = 400,
    pages = {877-890},
      doi = {10.1051/0004-6361:20030012},
   adsurl = {http://adsabs.harvard.edu/abs/2003A\%26A...400..877P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Pedraza JF et al.  ======
%% ============================================================	

% 2008MNRAS.390.1587P,
@ARTICLE{pedrazaRamoscaroGonzalez2008MNRAS,
   author = {{Pedraza}, J. F. and {Ramos-Caro}, J. and {Gonz{\'a}lez}, G. A.},
    title = "{An infinite family of self-consistent models for axisymmetric flat galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
 keywords = {stellar dynamics , galaxies: kinematics and dynamics},
     year = 2008,
    month = nov,
   volume = 390,
    pages = {1587-1597},
      doi = {10.1111/j.1365-2966.2008.13846.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.390.1587P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
  %  eprint = {0806.4277},
}

@article{PhysRevD.88.064020,
  title = {Anisotropic models for globular clusters, Galactic bulges, and dark halos},
  author = {Nguyen, P. H. and Pedraza, J. F.},
  journal = {Phys. Rev. D},
  volume = {88},
  issue = {6},
  pages = {064020},
  numpages = {27},
  year = {2013},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.88.064020},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.88.064020}
}


@article{PhysRevD.82.084005,
  title = {Charged annular disks and Reissner-Nordstr\"om type black holes from extremal dust},
  author = {Lora-Clavijo, F. D. and Ospina-Henao, P. A. and Pedraza, J. F.},
  journal = {Phys. Rev. D},
  volume = {82},
  issue = {8},
  pages = {084005},
  numpages = {13},
  year = {2010},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.82.084005},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.82.084005}
}






%% ============================================================
%% ====== Persic M et al.  ======
%% ============================================================	

% 1996MNRAS.281...27P,
@ARTICLE{persicSalucci1996MNRAS,
   author = {{Persic}, M. and {Salucci}, P. and {Stel}, F.},
    title = "{The universal rotation curve of spiral galaxies - I. The dark matter connection}",
  journal = {\mnras},
   eprint = {astro-ph/9506004},
 keywords = {GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: SPIRAL, GALAXIES: STRUCTURE, DARK MATTER},
     year = 1996,
    month = jul,
   volume = 281,
    pages = {27-47},
   adsurl = {http://adsabs.harvard.edu/abs/1996MNRAS.281...27P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Plummer  ======
%% ============================================================	

@ARTICLE{1911MNRAS..71..460P,
   author = {{Plummer}, H. C.},
    title = "{On the problem of distribution in globular star clusters}",
  journal = {\mnras},
     year = 1911,
    month = mar,
   volume = 71,
    pages = {460-470},
      doi = {10.1093/mnras/71.5.460},
   adsurl = {http://adsabs.harvard.edu/abs/1911MNRAS..71..460P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





%% ============================================================
%% ====== Pugliese D et al.  ======
%% ============================================================	

% 2011PhRvD..83b4021P,
@ARTICLE{puglieseQuevedoRuffini2011PRD,
   author = {{Pugliese}, D. and {Quevedo}, H. and {Ruffini}, R.},
    title = "{Circular motion of neutral test particles in Reissner-Nordstr{\"o}m spacetime}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1012.5411},
 primaryClass = "astro-ph.HE",
 keywords = {Classical general relativity, Relativistic stars: structure stability and oscillations, Classical black holes},
     year = 2011,
    month = jan,
   volume = 83,
   number = 2,
      eid = {024021},
    pages = {024021},
      doi = {10.1103/PhysRevD.83.024021},
   adsurl = {http://adsabs.harvard.edu/abs/2011PhRvD..83b4021P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Ramos-Caro J et al.  ======
%% ============================================================	

% 2008MNRAS.386..440R,
@ARTICLE{ramoscaroLopezsuspesGonzalez2008MNRAS,
   author = {{Ramos-Caro}, J. and {L{\'o}pez-Suspes}, F. and {Gonz{\'a}lez}, G. A.
	},
    title = "{Chaotic and regular motion around generalized Kalnajs discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0806.4272},
 keywords = {stellar dynamics, galaxies: kinematics and dynamics},
     year = 2008,
    month = may,
   volume = 386,
    pages = {440-446},
      doi = {10.1111/j.1365-2966.2008.13047.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386..440R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2011MNRAS.414.3105R,
@ARTICLE{ramoscaroPedrazaLetelier2011MNRAS,
   author = {{Ramos-Caro}, J. and {Pedraza}, J. F. and {Letelier}, P. S.},
    title = "{Motion around a monopole + ring system - I. Stability of equatorial circular orbits versus regularity of three-dimensional motion}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1103.4616},
 primaryClass = "astro-ph.EP",
 keywords = {chaos, celestial mechanics, planets and satellites: rings},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {3105-3116},
      doi = {10.1111/j.1365-2966.2011.18618.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.3105R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{PhysRevD.86.043008,
  title = {Kinetic theory of collisionless self-gravitating gases. II. Relativistic corrections in galactic dynamics},
  author = {Ramos-Caro, J. and Ag\'on, C. A. and Pedraza, J. F.},
  journal = {Phys. Rev. D},
  volume = {86},
  issue = {4},
  pages = {043008},
  numpages = {15},
  year = {2012},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.86.043008},
  %url = {https://link.aps.org/doi/10.1103/PhysRevD.86.043008}
}

@article{0264-9381-25-4-045011,
  author={Javier Ramos-Caro and Guillermo A Gonz\'{a}lez},
  title={FokkerâPlanckâRosenbluth-type equations for self-gravitating systems in the 1PN approximation},
  journal={Classical and Quantum Gravity},
  volume={25},
  number={4},
  pages={045011},
  year={2008},
  abstract={We present two formulations of FokkerâPlanckâRosenbluth-type (FPR) equations for many-particle self-gravitating systems, with first-order relativistic corrections in the post-Newtonian approach (1PN). The first starts from a covariant FokkerâPlanck equation for a simple gas, introduced recently by ChacÃ³n-Acosta and Kremer (2007 Phys. Rev. E 76 021201). The second derivation is based on the establishment of an 1PN-BBGKY hierarchy, developed systematically from the 1PN microscopic law of force and using the KlimontovichâDupree (KD) method. We close the hierarchy by the introduction of a two-point correlation function that describes adequately the relaxation process. This picture reveals an aspect that is not considered in the first formulation: the contribution of ternary correlation patterns to the diffusion coefficients, as a consequence of the nature of 1PN interaction. Both formulations can be considered as a generalization of the equation derived by Rezania and Sobouti (2000 Astron. Astrophys. 354 1110), to stellar systems where the relativistic effects of gravitation play a significant role.}
%  url={http://stacks.iop.org/0264-9381/25/i=4/a=045011},
}

%% ============================================================
%% ====== Rodrigues DC et al.  ======
%% ============================================================	

% 2010JCAP...04..020R,
@ARTICLE{rodriguesShapiroLetelier2010JCAP,
   author = {{Rodrigues}, D. C. and {Letelier}, P. S. and {Shapiro}, I. L.
	},
    title = "{Galaxy rotation curves from general relativity with renormalization group corrections}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {0911.4967},
 primaryClass = "astro-ph.CO",
     year = 2010,
    month = apr,
   volume = 4,
      eid = {020},
    pages = {20},
      doi = {10.1088/1475-7516/2010/04/020},
   adsurl = {http://adsabs.harvard.edu/abs/2010JCAP...04..020R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{1475-7516-2012-09-031,
  author={Davi C. Rodrigues},
  title={Elliptical galaxies kinematics within general relativity with renormalization group effects},
  journal={Journal of Cosmology and Astroparticle Physics},
  volume={2012},
  number={09},
  pages={031},
  year={2012},
  abstract={The renormalization group framework can be applied to Quantum Field Theory on curved space-time, but there is no proof whether the beta-function of the gravitational coupling indeed goes to zero in the far infrared or not. In a recent paper [ 1 [http://dx.doi.org/10.1088/1475-7516/2010/04/020] ] we have shown that the amount of dark matter inside spiral galaxies may be negligible if a small running of the General Relativity coupling G is present (Î´ G / G 0 ##IMG## [http://ej.iop.org/icons/Entities/lesssim.gif] {lesssim} 10 â7 across a galaxy). Here we extend the proposed model to elliptical galaxies and present a detailed analysis on the modeling of NGC 4494 (an ordinary elliptical) and NGC 4374 (a giant elliptical). In order to compare our results to a well known alternative model to the standard dark matter picture, we also evaluate NGC 4374 with MOND. In this galaxy MOND leads to a significative discrepancy with the observed velocity dispersion curve and has a significative tendency towards tangential anisotropy. On the other hand, the approach based on the renormalization group and general relativity (RGGR) could be applied with good results to these elliptical galaxies and is compatible with lower mass-to-light ratios (of about the Kroupa IMF type).}
%url={http://stacks.iop.org/1475-7516/2012/i=09/a=031},
}

%% ============================================================
%% ====== Rosa VM et al.  ======
%% ============================================================	

% 2007GReGr..39.1419R,
@ARTICLE{rosaLetelier2007GRG,
   author = {{Rosa}, V. M. and {Letelier}, P. S.},
    title = "{Stability of closed timelike curves in the G{\"o}del universe}",
  journal = {General Relativity and Gravitation},
   eprint = {gr-qc/0703100},
     year = 2007,
    month = sep,
   volume = 39,
    pages = {1419-1435},
      doi = {10.1007/s10714-007-0464-9},
   adsurl = {http://adsabs.harvard.edu/abs/2007GReGr..39.1419R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2007PhLA..370...99R,
@ARTICLE{rosaletelier2007PhLA,
   author = {{Rosa}, V. M. and {Letelier}, P. S.},
    title = "{Stability of closed timelike geodesics}",
  journal = {Physics Letters A},
   eprint = {gr-qc/0703148},
 keywords = {Spacetime topology causal structure spinor structure, Exact solutions},
     year = 2007,
    month = oct,
   volume = 370,
    pages = {99-103},
      doi = {10.1016/j.physleta.2007.05.041},
   adsurl = {http://adsabs.harvard.edu/abs/2007PhLA..370...99R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Saa A et al.  ======
%% ============================================================	

% 1999PhLA..259..201S,
@ARTICLE{saaVenegeroles1999PhLA,
   author = {{Saa}, A. and {Venegeroles}, R.},
    title = "{Chaos around the superposition of a black-hole and a thin disk}",
  journal = {Physics Letters A},
   eprint = {gr-qc/9906028},
     year = 1999,
    month = aug,
   volume = 259,
    pages = {201-206},
      doi = {10.1016/S0375-9601(99)00447-8},
   adsurl = {http://adsabs.harvard.edu/abs/1999PhLA..259..201S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Sanders J et al.  ======
%% ============================================================

% 2012MNRAS.426..128S,
@ARTICLE{sanders2012MNRAS,
   author = {{Sanders}, J.},
    title = "{Angle-action estimation in a general axisymmetric potential}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1208.2813},
 keywords = {methods: numerical, Galaxy: kinematics and dynamics, solar neighbourhood, Galaxy: structure, galaxies: kinematics and dynamics },
     year = 2012,
    month = oct,
   volume = 426,
    pages = {128-139},
      doi = {10.1111/j.1365-2966.2012.21698.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.426..128S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2014MNRAS.441.3284S,
@ARTICLE{sandersBinney2014MNRAS,
   author = {{Sanders}, J. L. and {Binney}, J.},
    title = "{Actions, angles and frequencies for numerically integrated orbits}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1401.3600},
 keywords = {methods: numerical, Galaxy: kinematics and dynamics, galaxies: kinematics and dynamics},
     year = 2014,
    month = jul,
   volume = 441,
    pages = {3284-3295},
      doi = {10.1093/mnras/stu796},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.441.3284S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Sanders RH et al.  ======
%% ============================================================

% 2002ARA&A..40..263S,
@ARTICLE{sandersMcgaughARAA2002,
   author = {{Sanders}, R. H. and {McGaugh}, S. S.},
    title = "{Modified Newtonian Dynamics as an Alternative to Dark Matter}",
  journal = {\araa},
   eprint = {astro-ph/0204521},
 keywords = {dark matter, galaxy dynamics, gravitational theory, cosmology},
     year = 2002,
   volume = 40,
    pages = {263-317},
      doi = {10.1146/annurev.astro.40.060401.093923},
   adsurl = {http://adsabs.harvard.edu/abs/2002ARA\%26A..40..263S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== SemerÃ¡k O et al.  ======
%% ============================================================	

% 1999MNRAS.308..691S,
@ARTICLE{semerakZellerinZacek1999MNRAS,
   author = {{Semer{\'a}k}, O. and {Zellerin}, T. and {{\v Z}{\'a}{\v c}ek}, M.
	},
    title = "{The structure of superposed Weyl fields}",
  journal = {\mnras},
     year = 1999,
    month = sep,
   volume = 308,
    pages = {691-704},
      doi = {10.1046/j.1365-8711.1999.02748.x},
   adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.308..691S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1999MNRAS.308..705S,
@ARTICLE{semerakZacekZellerin1999MNRAS,
   author = {{Semer{\'a}k}, O. and {{\v Z}{\'a}{\v c}ek}, M. and {Zellerin}, T.
	},
    title = "{Test-particle motion in superposed Weyl fields}",
  journal = {\mnras},
     year = 1999,
    month = sep,
   volume = 308,
    pages = {705-717},
      doi = {10.1046/j.1365-8711.1999.02749.x},
   adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.308..705S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2000PASJ...52.1067S,
@ARTICLE{semerakZacek2000PASJ,
   author = {{Semer{\'a}k}, O. and {{\v Z}{\'a}{\v c}ek}, M.},
    title = "{Oscillations of Static Discs around Schwarzschild Black Holes: Effect of Self-Gravitation}",
  journal = {\pasj},
 keywords = {ACCRETION DISCS, BLACK-HOLE PHYSICS, RELATIVITY},
     year = 2000,
    month = dec,
   volume = 52,
    pages = {1067-},
      doi = {10.1093/pasj/52.6.1067},
   adsurl = {http://adsabs.harvard.edu/abs/2000PASJ...52.1067S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2000CQGra..17.1613S,
@ARTICLE{semerakZacek2000CQGra,
   author = {{Semer{\'a}k}, O. and {Z{\'a}{\v c}ek}, M.},
    title = "{Gravitating discs around a Schwarzschild black hole: I}",
  journal = {Classical and Quantum Gravity},
     year = 2000,
    month = apr,
   volume = 17,
    pages = {1613-1626},
      doi = {10.1088/0264-9381/17/7/303},
   adsurl = {http://adsabs.harvard.edu/abs/2000CQGra..17.1613S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2002gfpi.conf..111S,
@INPROCEEDINGS{semerak2002review,
   author = {{Semer{\'a}k}, O.},
    title = "{Towards gravitating discs around stationary black holes}",
booktitle = {Gravitation: Following the Prague Inspiration},
     year = 2002,
   eprint = {gr-qc/0204025},
   editor = {{Semer{\'a}k}, O. and {Podolsk{\'y}}, J. and {Zofka}, M.},
    pages = {111},
   adsurl = {http://adsabs.harvard.edu/abs/2002gfpi.conf..111S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2010MNRAS.404..545S,
@ARTICLE{semerakSukova2010MNRAS,
   author = {{Semer{\'a}k}, O. and {Sukov{\'a}}, P.},
    title = "{Free motion around black holes with discs or rings: between integrability and chaos - I}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1211.4106},
 primaryClass = "gr-qc",
 keywords = {black hole physics, gravitation, relativity},
     year = 2010,
    month = may,
   volume = 404,
    pages = {545-574},
      doi = {10.1111/j.1365-2966.2009.16003.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.404..545S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2012MNRAS.425.2455S,
@ARTICLE{semerakSukova2012MNRAS,
   author = {{Semer{\'a}k}, O. and {Sukov{\'a}}, P.},
    title = "{Free motion around black holes with discs or rings: between integrability and chaos - II}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1211.4107},
 primaryClass = "gr-qc",
 keywords = {black hole physics, chaos, gravitation},
     year = 2012,
    month = oct,
   volume = 425,
    pages = {2455-2476},
      doi = {10.1111/j.1365-2966.2012.21630.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.425.2455S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Sgro et al.  ======
%% ============================================================	

@article{doi:10.1093/mnras/stt773,
author = {Sgr\'{o}, Mario A. and Paz, Dante J. and Merch\'{a}n, Manuel},
title = {Anisotropic halo model: implementation and numerical results},
journal = {Monthly Notices of the Royal Astronomical Society},
volume = {433},
number = {1},
pages = {787},
year = {2013},
doi = {10.1093/mnras/stt773},
%URL = { + http://dx.doi.org/10.1093/mnras/stt773},
%eprint = {/oup/backfile/content_public/journal/mnras/433/1/10.1093/mnras/stt773/3/stt773.pdf}
}



%% ============================================================
%% ====== Shrama et al.  ======
%% ============================================================	

@Article{Sharma2012,
author="Sharma, Ranjan
and Tikekar, Ramesh",
title="Space--time inhomogeneity, anisotropy and gravitational collapse",
journal="General Relativity and Gravitation",
year="2012",
month="Oct",
day="01",
volume="44",
number="10",
pages="2503--2520",
abstract="We investigate the evolution of non-adiabatic collapse of a shear-free spherically symmetric stellar configuration with anisotropic stresses accompanied with radial heat flux. The collapse begins from a curvature singularity with infinite mass and size on an inhomogeneous space--time background. The collapse is found to proceed without formation of an even horizon to singularity when the collapsing configuration radiates all its mass energy. The impact of inhomogeneity on various parameters of the collapsing stellar configuration is examined in some specific space--time backgrounds.",
%issn="1572-9532",
%doi="10.1007/s10714-012-1406-8",
%url="http://dx.doi.org/10.1007/s10714-012-1406-8"
}




%% ============================================================
%% ====== Shirokov MF et al.  ======
%% ============================================================	

% 1973GReGr...4..131S,
@ARTICLE{shirokov1973GRG,
   author = {{Shirokov}, M.F.},
    title = "{On one new effect of the Einsteinian theory of gravitation}",
  journal = {General Relativity and Gravitation},
     year = 1973,
    month = mar,
   volume = 4,
    pages = {131-136},
      doi = {10.1007/BF00762799},
   adsurl = {http://adsabs.harvard.edu/abs/1973GReGr...4..131S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Sing et al  ======
%% ============================================================


@ARTICLE{1992IJTP...31..545S,
   author = {{Singh}, T. and {Singh}, G. P. and {Srivastava}, R. S.},
    title = "{Static anisotropic fluid spheres in general relativity with nonuniform density}",
  journal = {International Journal of Theoretical Physics},
     year = 1992,
    month = mar,
   volume = 31,
    pages = {545-551},
      doi = {10.1007/BF00740004},
   adsurl = {http://adsabs.harvard.edu/abs/1992IJTP...31..545S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%% ============================================================
%% ====== Sofue Y et al.  ======
%% ============================================================

% 2001ARA&A..39..137S,
@ARTICLE{sofueRubin2001ARAA,
   author = {{Sofue}, Y. and {Rubin}, V.},
    title = "{Rotation Curves of Spiral Galaxies}",
  journal = {\araa},
   eprint = {astro-ph/0010594},
     year = 2001,
   volume = 39,
    pages = {137-174},
      doi = {10.1146/annurev.astro.39.1.137},
   adsurl = {http://adsabs.harvard.edu/abs/2001ARA%26A..39..137S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 1999ApJ...523..136S,
@ARTICLE{sofueEtal1999ApJ,
   author = {{Sofue}, Y. and {Tutui}, Y. and {Honma}, M. and {Tomita}, A. and
	{Takamiya}, T. and {Koda}, J. and {Takeda}, Y.},
    title = "{Central Rotation Curves of Spiral Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/9905056},
 keywords = {GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: NUCLEI, GALAXIES: SPIRAL, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Galaxies: Spiral},
     year = 1999,
    month = sep,
   volume = 523,
    pages = {136-146},
      doi = {10.1086/307731},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...523..136S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2009PASJ...61..227S,
@ARTICLE{sofueHonmaOmodaka2009PASJ,
   author = {{Sofue}, Y. and {Honma}, M. and {Omodaka}, T.},
    title = "{Unified Rotation Curve of the Galaxy -- Decomposition into de Vaucouleurs Bulge, Disk, Dark Halo, and the 9-kpc Rotation Dip --}",
  journal = {\pasj},
archivePrefix = "arXiv",
   eprint = {	},
 keywords = {Galaxy: bulge, Galaxy: disk, Galaxy: rotation curve, Galaxy: structure},
     year = 2009,
    month = feb,
   volume = 61,
    pages = {227-},
      doi = {10.1093/pasj/61.2.227},
   adsurl = {http://adsabs.harvard.edu/abs/2009PASJ...61..227S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Sotomayor J et al.  ======
%% ============================================================

%
@book{sotomayor1979li,
  title={Li\c{c}\~oes de equa\c{c}\~oes diferenciais ordin{\'a}rias},
  author={Sotomayor, Jorge},
  volume={11},
  year={1979},
  publisher={Instituto de Matem{\'a}tica Pura e Aplicada, CNPq}
}

%% ============================================================
%% ====== Stephani H et al.  ======
%% ============================================================

%
@book{stephani2003exact,
  title={Exact solutions of Einstein's field equations},
  author={Stephani, Hans and Kramer, Dietrich and MacCallum, Malcolm and Hoenselaers, Cornelius and Herlt, Eduard},
  year={2003},
  publisher={Cambridge University Press}
}

%% ============================================================
%% ====== Steinmetz M et al.  ======
%% ============================================================

% 2012AN....333..523S,
@ARTICLE{steinmetz2012AN,
   author = {{Steinmetz}, M.},
    title = "{The Galactic thin and thick disk}",
  journal = {Astronomische Nachrichten},
archivePrefix = "arXiv",
   eprint = {1205.6098},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: abundances, Galaxy: evolution, Galaxy: formation, Galaxy: kinematics and dynamics, Galaxy: stellar content, Galaxy: structure, surveys},
     year = 2012,
    month = jun,
   volume = 333,
    pages = {523},
      doi = {10.1002/asna.201211698},
   adsurl = {http://adsabs.harvard.edu/abs/2012AN....333..523S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Stuchlik Z et al.  ======
%% ============================================================

%
@ARTICLE{stuchlikHedlik2002AcPSl,
   author = {{Stuchl{\'i}k}, Z. and {Hled{\'i}k}, S.},
    title = "{Properties of the Reissner-Nordstr{\"o}m spacetimes with a nonzero cosmological constant}",
  journal = {Acta Physica Slovaca},
     year = 2002,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1311.5820V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== SukovÃ¡ P et al.  ======
%% ============================================================

% 2013MNRAS.436..978S,
@ARTICLE{sukovaSemerak2013MNRAS,
   author = {{Sukov{\'a}}, P. and {Semer{\'a}k}, O.},
    title = "{Free motion around black holes with discs or rings: between integrability and chaos - III}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1308.4306},
 primaryClass = "gr-qc",
 keywords = {black hole physics, chaos, gravitation, Galaxy: centre},
     year = 2013,
    month = dec,
   volume = 436,
    pages = {978-996},
      doi = {10.1093/mnras/stt1587},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.436..978S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Tabor M et al.  ======
%% ============================================================

%
@book{tabor1989chaos,
  title={Chaos and integrability in nonlinear dynamics},
  author={Tabor, Michael},
  year={1989},
  publisher={Wiley}
}

%% ============================================================
%% ====== Taub AH et al.  ======
%% ============================================================

% 1980JMP....21.1423T,
@ARTICLE{taub1980JMP,
   author = {{Taub}, A. H.},
    title = "{Space-times with distribution valued curvature tensors.}",
  journal = {Journal of Mathematical Physics},
 keywords = {Relativity:Space-Time},
     year = 1980,
   volume = 21,
    pages = {1423-1431},
      doi = {10.1063/1.524568},
   adsurl = {http://adsabs.harvard.edu/abs/1980JMP....21.1423T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Ujevic M et al.  ======
%% ============================================================

% 2004PhRvD..70h4015U,
@ARTICLE{ujevicLetelier2004PRD,
   author = {{Ujevic}, M. and {Letelier}, P. S.},
    title = "{Stability of general relativistic geometric thin disks}",
  journal = {\prd},
   eprint = {gr-qc/0409110},
 keywords = {Relativistic stars: structure stability and oscillations, Exact solutions, Spiral arms and bars, galactic disks},
     year = 2004,
    month = oct,
   volume = 70,
   number = 8,
      eid = {084015},
    pages = {084015},
      doi = {10.1103/PhysRevD.70.084015},
   adsurl = {http://adsabs.harvard.edu/abs/2004PhRvD..70h4015U},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== van der Kruit PC et al.  ======
%% ============================================================

% 1988A&A...192..117V,
@ARTICLE{vanderkruit1988AA,
   author = {{van der Kruit}, P. C.},
    title = "{The three-dimensional distribution of light and mass in disks of spiral galaxies}",
  journal = {\aap},
 keywords = {Gas Dynamics, Mass To Light Ratios, Spiral Galaxies, Star Distribution, Astronomical Models, Density Distribution, Mass Distribution, Radial Velocity, Velocity Distribution, Vertical Distribution},
     year = 1988,
    month = mar,
   volume = 192,
    pages = {117-127},
   adsurl = {http://adsabs.harvard.edu/abs/1988A\%26A...192..117V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2011ARA&A..49..301V,
@ARTICLE{vanderkruitFreeman2011ARAA,
   author = {{van der Kruit}, P. C. and {Freeman}, K. C.},
    title = "{Galaxy Disks}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1101.1771},
 primaryClass = "astro-ph.GA",
     year = 2011,
    month = sep,
   volume = 49,
    pages = {301-371},
      doi = {10.1146/annurev-astro-083109-153241},
   adsurl = {http://adsabs.harvard.edu/abs/2011ARA\%26A..49..301V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Veltz L et al.  ======
%% ============================================================

% 2008A&A...480..753V,
@ARTICLE{veltzEtal2008AA,
   author = {{Veltz}, L. and {Bienaym{\'e}}, O. and {Freeman}, K. C. and
	{Binney}, J. and {Bland-Hawthorn}, J. and {Gibson}, B. K. and
	{Gilmore}, G. and {Grebel}, E. K. and {Helmi}, A. and {Munari}, U. and
	{Navarro}, J. F. and {Parker}, Q. A. and {Seabroke}, G. M. and
	{Siebert}, A. and {Steinmetz}, M. and {Watson}, F. G. and {Williams}, M. and
	{Wyse}, R. F. G. and {Zwitter}, T.},
    title = "{Galactic kinematics with RAVE data. I. The distribution of stars towards the Galactic poles}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0801.2120},
 keywords = {stars: kinematics, Galaxy: disk, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2008,
    month = mar,
   volume = 480,
    pages = {753-765},
      doi = {10.1051/0004-6361:20066948},
   adsurl = {http://adsabs.harvard.edu/abs/2008A\%26A...480..753V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Vieira RSS et al.  ======
%% ============================================================

% 2014GReGr..46.1641V,
@ARTICLE{vieiraLetelier2014GRG,
   author = {{Vieira}, R. S. S. and {Letelier}, P. S.},
    title = "{Thin-disk models in an integrable Weyl-Dirac theory}",
  journal = {General Relativity and Gravitation},
archivePrefix = "arXiv",
   eprint = {1305.2662},
 primaryClass = "gr-qc",
 keywords = {Weyl-Dirac theory, Exact solutions, Galaxy astrophysics, Modified gravity},
     year = 2014,
    month = jan,
   volume = 46,
    pages = {1641},
      doi = {10.1007/s10714-013-1641-7},
   adsurl = {http://adsabs.harvard.edu/abs/2014GReGr..46.1641V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2014ApJ...786...27V,
@ARTICLE{vieiraRamoscaro2014ApJ,
   author = {{Vieira}, R. S. S. and {Ramos-Caro}, J.},
    title = "{A Simple Formula for the Third Integral of Motion of Disk-crossing Stars in the Galaxy}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1305.7078},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: spiral, Galaxy: disk, Galaxy: kinematics and dynamics },
     year = 2014,
    month = may,
   volume = 786,
      eid = {27},
    pages = {27},
      doi = {10.1088/0004-637X/786/1/27},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...786...27V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2014PhRvD..90b4035V,
@ARTICLE{vieiraMarekEtal2014PRD,
   author = {{Vieira}, R. S. S. and {Schee}, J. and {Klu{\'z}niak}, W. and
	{Stuchl{\'{\i}}k}, Z. and {Abramowicz}, M.},
    title = "{Circular geodesics of naked singularities in the Kehagias-Sfetsos metric of Ho{\v r}ava's gravity}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1311.5820},
 primaryClass = "gr-qc",
 keywords = {Modified theories of gravity, Classical black holes, Relativistic stars: structure stability and oscillations, Orbit determination and improvement},
     year = 2014,
    month = jul,
   volume = 90,
   number = 2,
      eid = {024035},
    pages = {024035},
      doi = {10.1103/PhysRevD.90.024035},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..90b4035V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% 2016CeMDA.tmp...40V
@ARTICLE{vieiraRamoscaro2016CeMDA,
   author = {{Vieira}, R. S. S. and {Ramos-Caro}, J.},
    title = "{Integrability of motion around galactic razor-thin disks}",
  journal = {Celestial Mechanics and Dynamical Astronomy},
archivePrefix = "arXiv",
   eprint = {1606.06349},
 keywords = {Dynamics of galaxies, Razor-thin disks, Disk-crossing orbits, Vertical stability, Third integral, Adiabatic approximation},
     year = 2016,
    month = jun,
     note = {(published online, doi:10.1007/s10569-016-9705-0)},
      doi = {10.1007/s10569-016-9705-0},
   adsurl = {http://adsabs.harvard.edu/abs/2016CeMDA.tmp...40V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% doi:10.1142/9789814623995_0438
@inproceedings{vieiraRamoscaro2015MG13,
author = {{Vieira}, R. S. S. and {Ramos-Caro}, J.},
title = {On the Stability of Circular Orbits in Galactic Dynamics: Newtonian Thin Disks},
booktitle = {The Thirteenth Marcel Grossmann Meeting},
editor = {Kjell Rosquist and Robert T. Jantzen and Remo Ruffini},
chapter = {438},
pages = {2346-2348},
year={2015},
publisher= {World Scientific},
doi = {10.1142/9789814623995_0438}
}



% 1PN razor thin disks
@article{PhysRevD.86.043008,
  title = {Kinetic theory of collisionless self-gravitating gases. II. Relativistic corrections in galactic dynamics},
  author = {Ramos-Caro, J. and Ag\'on, C. A. and Pedraza, J. F.},
  journal = {Phys. Rev. D},
  volume = {86},
  issue = {4},
  pages = {043008},
  numpages = {15},
  year = {2012},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.86.043008},
  adsurl = {http://link.aps.org/doi/10.1103/PhysRevD.86.043008}
}


%% ============================================================
%% ====== Vogt D et al.  ======
%% ============================================================

% 2003PhRvD..68h4010V,
@ARTICLE{vogtLetelier2003PRD,
   author = {{Vogt}, D. and {Letelier}, P. S.},
    title = "{Exact general relativistic perfect fluid disks with halos}",
  journal = {\prd},
   eprint = {gr-qc/0308031},
 keywords = {Exact solutions, Self-gravitating systems, continuous media and classical fields in curved spacetime, Accretion and accretion disks},
     year = 2003,
    month = oct,
   volume = 68,
   number = 8,
      eid = {084010},
    pages = {084010},
      doi = {10.1103/PhysRevD.68.084010},
   adsurl = {http://adsabs.harvard.edu/abs/2003PhRvD..68h4010V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2005MNRAS.363..268V,
@ARTICLE{vogtLetelier2005MNRAS,
   author = {{Vogt}, D. and {Letelier}, P. S.},
    title = "{Relativistic models of galaxies}",
  journal = {\mnras},
   eprint = {astro-ph/0507406},
 keywords = {relativity, stellar dynamics, celestial mechanics, galaxies: kinematics and dynamics},
     year = 2005,
    month = oct,
   volume = 363,
    pages = {268-284},
      doi = {10.1111/j.1365-2966.2005.09436.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.363..268V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% 2009MNRAS.396.1487V,
@ARTICLE{vogtLetelier2009MNRAS,
   author = {{Vogt}, D. and {Letelier}, P. S.},
    title = "{Analytical potential-density pairs for flat rings and toroidal structures}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0906.0919},
 primaryClass = "astro-ph.GA",
 keywords = {planets: rings , galaxies: kinematics and dynamics},
     year = 2009,
    month = jul,
   volume = 396,
    pages = {1487-1498},
      doi = {10.1111/j.1365-2966.2009.14803.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.396.1487V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{doi:10.1111/j.1365-2966.2009.15967.x,
author = {Vogt, D. and Letelier, P. S.},
title = {Newtonian and General Relativistic models of spherical shells},
journal = {Monthly Notices of the Royal Astronomical Society},
volume = {402},
number = {2},
pages = {1313},
year = {2010},
doi = {10.1111/j.1365-2966.2009.15967.x},
%URL = { + http://dx.doi.org/10.1111/j.1365-2966.2009.15967.x},
%eprint = {/oup/backfile/content_public/journal/mnras/402/2/10.1111/j.1365-2966.2009.15967.x/2/mnras0402-1313.pdf}
}

@article{doi:10.1111/j.1365-2966.2010.16863.x,
author = {Vogt, D. and Letelier, P. S.},
title = {Newtonian and General Relativistic models of spherical shells â II},
journal = {Monthly Notices of the Royal Astronomical Society},
volume = {406},
number = {4},
pages = {2689},
year = {2010},
doi = {10.1111/j.1365-2966.2010.16863.x},
%URL = { + http://dx.doi.org/10.1111/j.1365-2966.2010.16863.x},
%eprint = {/oup/backfile/content_public/journal/mnras/406/4/10.1111/j.1365-2966.2010.16863.x/2/mnras0406-2689.pdf}
}


%
@phdthesis{vogtthesis,
  author={Vogt, Daniel},
  title={Modelos de discos e outras estruturas auto-gravitantes em relatividade geral},
  school={Universidade Estadual de Campinas, Instituto de Fisica Gleb Wataghin},
  year={2006}
}



%% ============================================================
%% ====== Voorhees BH et al.  ======
%% ============================================================

% 1972PhRvD...5.2413V,
@ARTICLE{voorhees1972PRD,
   author = {{Voorhees}, B. H.},
    title = "{Relativistic Disks. I. Background Models}",
  journal = {\prd},
     year = 1972,
    month = may,
   volume = 5,
    pages = {2413-2418},
      doi = {10.1103/PhysRevD.5.2413},
   adsurl = {http://adsabs.harvard.edu/abs/1972PhRvD...5.2413V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%% ============================================================
%% ====== Wald R et al.  ======
%% ============================================================

%
@book{waldGR,	
  author = {R. Wald},
  title  = {General Relativity},
  publisher = {The University of Chicago Press},
  year = {1984},
  address = {Chicago, IL}	
}

%% ============================================================
%% ====== Witzany V et al.  ======
%% ============================================================

% 2015MNRAS.451.1770W
@ARTICLE{witzanySemerakSukova2015MNRAS,
   author = {{Witzany}, V. and {Semer{\'a}k}, O. and {Sukov{\'a}}, P.},
    title = "{Free motion around black holes with discs or rings: between integrability and chaos - IV}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1503.09077},
 primaryClass = "astro-ph.HE",
 keywords = {black hole physics, chaos, gravitation},
     year = 2015,
    month = aug,
   volume = 451,
    pages = {1770-1794},
      doi = {10.1093/mnras/stv1148},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.451.1770W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%% ============================================================
%% ====== Zacek M et al.  ======
%% ============================================================

% 2002CzJPh..52...19Z,
@ARTICLE{zacekSemerak2002CzJP,
   author = {{{\v Z}{\'a}{\v c}ek}, M. and {Semer{\'a}k}, O.},
    title = "{Gravitating Discs Around a Schwarzschild Black Hole II}",
  journal = {Czechoslovak Journal of Physics},
 keywords = {general relativity - black holes - exact solutions of Einstein equations},
     year = 2002,
    month = jan,
   volume = 52,
    pages = {19-27},
      doi = {10.1023/A:1013957512339},
   adsurl = {http://adsabs.harvard.edu/abs/2002CzJPh..52...19Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



%% ============================================================
%% ====== Zharnitsky V et al.  ======
%% ============================================================

% 2000CMaPh.211..289Z,
@ARTICLE{zharnitsky2000CMaPh,
   author = {{Zharnitsky}, V.},
    title = "{Invariant Tori in Hamiltonian Systems with Impacts}",
  journal = {Communications in Mathematical Physics},
     year = 2000,
   volume = 211,
    pages = {289-302},
      doi = {10.1007/s002200050813},
   adsurl = {http://adsabs.harvard.edu/abs/2000CMaPh.211..289Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{Nguyen,
  author    = {Nguyen, Phuc H. and Lingam, Manasvi},
  title     = {Analytical families of two-component anisotropic polytropes and their relativistic extensions},
  journal   = {Monthly Notices of the Royal Astronomical Society},
  year      = {2013},
  volume    = {436},
  number    = {3},
  pages     = {2014},
  month     = {oct},
  doi       = {10.1093/mnras/stt1719},
  keywords  = {rank5},
  publisher = {Oxford University Press ({OUP})},
  %url       = {http://dx.doi.org/10.1093/mnras/stt1719},
}

@Book{poissontoolkit,
  title     = {A Relativist's Toolkit},
  publisher = {Cambridge University Press},
  year      = {2007},
  author    = {Eric Poisson},
  date      = {2007-11-05},
  ean       = {9780521537803},
  isbn      = {0521537800},
  pagetotal = {252},
}

@Book{Weinberg,
  title     = {Gravitation and Cosmology},
  publisher = {John Wiley and Sons Ltd},
  year      = {1972},
  author    = {Steven Weinberg},
  date      = {1972-01-01},
  ean       = {9780471925675},
  pagetotal = {688},
   % isbn      = {0471925675},

   @Book{Kremer,
  title     = {The Relativistic Boltzmann Equation: Theory and Applications},
  publisher = {Birkhäuser Basel},
  year      = {2002},
  author    = {Carlo Cercignani and Gilberto M. Kremer},
  date      = {2002-01-01},
  ean       = {},
  pagetotal = {384},
   % isbn      = {978-3-7643-6693-3},
}
@article{Fackerell_1968,
	doi = {10.1086/149693},
	year = 1968,
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {153},
	pages = {643},
	author = {Edward D. Fackerell},
	title = {Relativistic Stellar Dynamics},
	journal = {The Astrophysical Journal}
	%url = {https://doi.org/10.1086%2F149693},
}

@Book{Polyanin,
  title     = {Handbook of Integral Equations},
  publisher = {Chapman and Hall/CRC},
  year      = {2008},
  author    = {Andrei D. Polyanin and Alexander V. Manzhirov},
  edition   = {Second Edition},
  keywords  = {rank5},
}

@Book{Straumann,
  title     = {General Relativity},
  publisher = {Springer Netherlands},
  year      = {2013},
  author    = {Norbert Straumann},
  edition   = {Second Edition},
}

@Comment{jabref-meta: databaseType:bibtex;}

